Stealing Hyperparameters in Machine Learning

Hyperparameters are critical in machine learning, as different hyperparameters often result in models with significantly different performance. Hyperparameters may be deemed confidential because of their commercial value and the confidentiality of the proprietary algorithms that the learner uses to learn them. In this work, we propose attacks on stealing the hyperparameters that are learned by a learner. We call our attacks hyperparameter stealing attacks. Our attacks are applicable to a variety of popular machine learning algorithms such as ridge regression, logistic regression, support vector machine, and neural network. We evaluate the effectiveness of our attacks both theoretically and empirically. For instance, we evaluate our attacks on Amazon Machine Learning. Our results demonstrate that our attacks can accurately steal hyperparameters. We also study countermeasures. Our results highlight the need for new defenses against our hyperparameter stealing attacks for certain machine learning algorithms.

==> analysis.tex <==
\section{Sensitivity Analysis}

In this section, we will analyze the sensitivity of different regularizations and loss functions of regression and classification methods. Specifically, \emph{we quantify the sensitivity as the variation of estimated $\hat{\lambda}$ or $\hat{C}$ with respect to the variation of weight vector $\mathbf{w}$ in the original space or $\bm{\alpha}$ in the kernel-mapped space}. 
%Formally, we denote the variation of $w_i$, $\alpha_i$, $\hat{\lambda}^{i}$, and $\hat{C}^{i}$ as $\Delta w_i$, $\Delta \alpha_i$, $\Delta \hat{\lambda}^{i}$, and $\Delta \hat{C}^i$ respectively. 
%To perform sensitivity analysis, we treat each $\Delta \hat{\lambda}^{(i)}$ or $\hat{C}^{(j)}$ as the function of $w_i$ (or $\alpha_j$), while fixing the remaining $\mathbf{w}_{-i}$ (or $\bm{\alpha}_{-i}$). Furthermore, we assume that the fixed $\mathbf{w}_{-i}$ (or $\bm{\alpha}_{-i}$) are the same when comparing two methods.  

To perform sensitivity analysis, we treat each $\hat{\lambda}^{(i})$ or $\hat{C}^{(i)}$ as the function of $w_i$ (or $\alpha_i$), while fixing the remaining $\mathbf{w}_{-i}$ (or $\bm{\alpha}_{-i}$). Furthermore, for a fair comparison, we assume that the fixed $\mathbf{w}_{-i}$ (or $\bm{\alpha}_{-i}$) are the same when we contrast two methods.  
Formally, we define $\hat{\lambda}^{(i)} = \hat{\lambda}^{(i)}(w_i) $ (or $\hat{\lambda}^{(i)} = \hat{\lambda}^{(i)}(\alpha_i))$ and $\hat{C}^{(i)} = \hat{C}^{(i)}(w_i)$ (or $\hat{C}^{(i)} = \hat{C}^{(i)}(\alpha_i)$). 
We denote the variation of $w_i$, $\alpha_i$, $\hat{\lambda}^{(i)}$, and $\hat{C}^{(i)}$ as $\Delta w_i$, $\Delta \alpha_i$, $\Delta \hat{\lambda}^{(i)}$, and $\Delta \hat{C}^{(i)}$ respectively. In doing so, the sensitivity, e.g, $\hat{\lambda}$ with respect to $\hat{w}_i$, can be formulated as $|\frac{\Delta \hat{\lambda}^{(i)}}{\Delta w_i}|$.

\subsection{Regression: Compare $l_1$ with $l_2$ Regularization}

In this part, we compare four aforementioned regression methods, i.e., Ridge regression, LASSO, Elastic Net, and Kernel Ridge regression.

%We compare $l_2$-regularized Ridge regression with $l_1$-regularized LASSO in this part. 

For Ridge regression, 
\begin{align}
\begin{split}
\Bigg| \frac{\Delta \hat{\lambda}_{Ridge}^{(i)}}{\Delta w_i} \Bigg| & = \Bigg|\frac{\hat{\lambda}_{Ridge}^{(i)}(w_i + \Delta w_i) - \hat{\lambda}_{Ridge}^{(i)}(w_i)}{\Delta w_i}\Bigg| \\
& = \Bigg|\frac{1}{\Delta w_i} \bigg( \frac{\langle \mathbf{x}_i, \mathbf{r}_i \rangle}{w_i + \Delta w_i} - \frac{\langle \mathbf{x}_i, \mathbf{r}_i \rangle}{w_i} \bigg)\Bigg| \\ 
& = \Bigg|\frac{1}{(w_i + \Delta w_i) w_i} \langle \mathbf{x}_i, \mathbf{r}_i \rangle \Bigg|.
\end{split}
\end{align}

For LASSO, if $w_i > 0$
\begin{align}
\Bigg| \frac{\Delta \hat{\lambda}_{LASSO}^{(i)}}{\Delta w_i} \Bigg| = \Bigg| \frac{-2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle (w_i + \Delta w_i) + 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i }{\Delta w_i} \Bigg| = \big| 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle \big|.
\end{align}
%Similarly, $\frac{\Delta \hat{\lambda}_{LASSO}^{(i)}}{\Delta w_i} = 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle $ if $w_i < 0$.

Note that the variation of Ridge regression depends on both the true $w_i$ and the changed $w_i + \Delta w_i$; While for LASSO, it is independent of both $w_i$ and $\Delta w_i$ and is constant. As a consequence, the estimated $\hat{\lambda}_{LASSO}^{(i)}$ of LASSO will be almost not affected if the length of $\mathbf{x}_i$ is small, which can be obtained through preprocessing the raw data; However, $\hat{\lambda}_{Ridge}^{(i)}$ of Ridge regression can be changed dramatically once $w_i$ is much smaller than 1, or/and the absolute value of $\Delta w_i$ is comparable with $w_i$ (We mention in advance that $\Delta w_i$ and $w_i$ always have the opposite sign in our experiments, and thus when $|\Delta w_i| \rightarrow |w_i|, w_i + \Delta w_i \rightarrow 0$). 
%, which is often the case. For instance, $l_2$ norm of $\mathbf{w}$ is required to be less than or equal 1, i.e., $\| \mathbf{w} \|_2 \leq 1$.  

For Elastic Net, since it incorporates both $l_2$ and $l_1$ regularizations, the sensitivity of $\hat{\lambda_2}^{(i)}$ and $\hat{\lambda_1}^{(i)}$ share the same property with $\hat{\lambda}_{Ridge}^{(i)}$ in Ridge regression and $\hat{\lambda}_{LASSO}^{(i)}$ in LASSO. Specifically,


For Kernel Ridge regression, the sensitivity is 
\begin{align}
\label{KernelRidge_sensi}
\begin{split}
\Bigg| \frac{\Delta \hat{\lambda}_{KernelRidge}^{(j)}}{\Delta \alpha_j} \Bigg| & = \Bigg| \frac{1}{\Delta \alpha_j} \bigg( \frac{y_j}{\alpha_j + \Delta \alpha_j} - \frac{y_j}{\alpha_j} \bigg) \Bigg| \\
& = \Bigg| -\frac{1}{(\alpha_j + \Delta \alpha_j) \alpha_j} y_j \Bigg|,   
\end{split}
\end{align}
which has a similar form with Ridge regression. Thus, the far smaller $\alpha_j$ is than 1, or the much closer $\Delta \alpha_j$ is to $\alpha_j$, the more sensitive Kernel Ridge regression is.  

\subsection{Logistic Regression: Compare $l_1$ with $l_2$ Regularization}

First, we consider $L_2$-BLR and $L_1$-BLR.

For $L_2$-BLR, 
$\hat{\lambda}_{L_2-BLR}^{(i)} (w_i + \Delta w_i) = - \frac{\langle \mathbf{x}_i, h_{\mathbf{w}+\Delta w_i}(\mathbf{X}) - \mathbf{y} \rangle}{ 2 (w_i + \Delta w_i)}$, 
where $h_{\mathbf{w}+\Delta w_i}(\mathbf{X}) = \left[ h_{\mathbf{w}+\Delta w_i}(\mathbf{x}^1_T), h_{\mathbf{w}+\Delta w_i}(\mathbf{x}^2_T), \cdots, h_{\mathbf{w}+\Delta w_i}(\mathbf{x}^n_T) \right]^T $ and $h_{\mathbf{w}+\Delta w_i} (\mathbf{x}^i_T) = \frac{1}{1 + \exp(\sum_{j \neq i} w_j x_{i,j}) + (w_i + \Delta w_i) x_{i,i}}$ (One should notice that the notation $\mathbf{w}+\Delta w_i$ here is not so ``formal", as $\Delta w_i$ is not added to all elements of $\mathbf{w}$, but to its $i$-th entry. We use such notation for ease of writing).
Therefore, 
\begin{align}
\label{L2_BLR_sensi}
\begin{split}
& \Bigg| \frac{\Delta \hat{\lambda}_{L_2-BLR}^{(i)}}{\Delta w_i} \Bigg| = \Bigg| \frac{\hat{\lambda}_{L_2-BLR}^{(i)} (w_i + \Delta w_i) - \hat{\lambda}_{L_2-BLR}^{(i)} (w_i)}{\Delta w_i} \Bigg| \\
& = \Bigg| \frac{1}{\Delta w_i} \bigg( -\frac{1}{2(w_i + \Delta w_i)} \langle \mathbf{x}_i, h_{\mathbf{w}+\Delta w_i}(\mathbf{X}) - \mathbf{y} \rangle + \frac{1}{2 w_i} \langle \mathbf{x}_i, h_{\mathbf{w}}(\mathbf{X}) - \mathbf{y} \rangle \bigg) \Bigg| \\
& = \Bigg| \frac{1}{\Delta w_i} \bigg( - \frac{1}{2(w_i + \Delta w_i)} \langle \mathbf{x}_i, h_{\mathbf{w}+\Delta w_i}(\mathbf{X}) - \mathbf{y} \rangle + \frac{1}{2(w_i + \Delta w_i)} \langle \mathbf{x}_i, h_{\mathbf{w}}(\mathbf{X}) - \mathbf{y} \rangle \bigg) \\ 
& \quad + \frac{1}{\Delta w_i} \bigg( - \frac{1}{2(w_i + \Delta w_i)} \langle \mathbf{x}_i, h_{\mathbf{w}}(\mathbf{X}) - y \rangle + \frac{1}{2 w_i} \langle \mathbf{x}_i, h_{\mathbf{w}}(\mathbf{X}) - \mathbf{y} \rangle \bigg) \Bigg| \\
& = \Bigg| - \frac{1}{2(w_i + \Delta w_i) \Delta w_i} \langle \mathbf{x}_i, h_{\mathbf{w}+\Delta w_i}(\mathbf{X}) - h_{\mathbf{w}}(\mathbf{X}) \rangle \\
& \quad + \frac{1}{2 w_i (w_i + \Delta w_i)} \langle \mathbf{x}_i, h_{\mathbf{w}}(\mathbf{X}) - \mathbf{y} \rangle \Bigg|. 
\end{split}
\end{align}

For $L_1$-BLR, 
\begin{align}
\label{L1_BLR_sensi}
\begin{split}
\Bigg| \frac{\Delta \hat{\lambda}_{L_1-BLR}^{(i)}}{\Delta w_i} \Bigg| & = \Bigg| \frac{1}{\Delta w_i} \big( \langle \mathbf{x}_i, h_{\mathbf{w} + \Delta w_i}(\mathbf{X}) - \mathbf{y} \rangle - \langle \mathbf{x}_i, h_{\mathbf{w}}(\mathbf{X}) - \mathbf{y} \rangle \big) \Bigg| \\
& = \Bigg| \frac{1}{\Delta w_i} \langle \mathbf{x}_i, h_{\mathbf{w} + \Delta w_i}(\mathbf{X}) - h_{\mathbf{w}}(\mathbf{X}) \rangle \Bigg|.
\end{split}
\end{align}
%Similarly, if $w_i <0$, $\frac{\Delta \hat{\lambda}_{L_1-BLR}^{(i)}}{\Delta w_i} = - \frac{1}{\Delta w_i} \langle \mathbf{x}_i, h_{\mathbf{w} + \Delta w_i}(\mathbf{X}) - h_{\mathbf{w}}(\mathbf{X}) \rangle $.

Comparing Eqn~\ref{L2_BLR_sensi} with Eqn~\ref{L1_BLR_sensi} and reusing the aforementioned analysis, we observe that once the absolute value of $w_i$ is one or two orders of magnitude smaller than 1 or $\Delta w_i$ is comparable with $w_i$, then $L_2$-BLR is more sensitive than $L_1$-BLR in terms of the variation of $w_i$. 

Then, we consider $L_2$-BKLR and $L_1$-BKLR.

For $L_2$-BKLR,
\begin{align}
\begin{split}
& \Bigg| \frac{\Delta \hat{\lambda}_{L_2-BKLR}^{(j)}}{\Delta \alpha_j} \Bigg| = \Bigg| \frac{1}{\Delta \alpha_j} \bigg( \frac{y_j - h_{\bm{\alpha} + \Delta \alpha_j}(\mathbf{k}_j)}{2(\alpha_j + \Delta \alpha_j)} - \frac{y_j - h_{\bm{\alpha}} (\mathbf{k}_j)}{2 \alpha_j} \bigg) \Bigg| \\
& = \Bigg| - \frac{h_{\bm{\alpha}+\Delta \alpha_j}(\mathbf{k}_j) - h_{\bm{\alpha}}(\mathbf{k}_j)}{2(\alpha_j + \Delta \alpha_j) \Delta \alpha_j} + \frac{h_{\bm{\alpha}}(\mathbf{k}_j) - y_j}{2(\alpha_j + \Delta \alpha_j) \alpha_j} \Bigg|,
\end{split}
\end{align}
where $h_{\bm{\alpha}+\Delta \alpha_j} (\mathbf{k}_j) = \frac{1}{1+ \exp(\langle \bm{\alpha}, \mathbf{k}_j \rangle + \Delta \alpha_j k_{j,j})}$.

For $L_1$-BKLR, %if $\mathbf{k}^j \bm{\alpha} < 0$,
\begin{align}
\Bigg| \frac{\Delta \hat{\lambda}_{L_1-BKLR}^{(j)}}{\Delta \alpha_j} \Bigg| = \Bigg| \frac{1}{\Delta \alpha_j} \big( h_{\bm{\alpha}+\Delta \alpha_j}(\mathbf{k}_j) - h_{\bm{\alpha}}(\mathbf{k}_j) \big) \Bigg|.
\end{align}
%and $\frac{\Delta \hat{\lambda}_{L_1-BKLR}^{(j)}}{\Delta \alpha_j} = \frac{1}{\Delta \alpha_j} \big( - h_{\bm{\alpha}+\Delta \alpha_j}(\mathbf{k}_j) + h_{\bm{\alpha}}(\mathbf{k}_j) \big)$ if $\mathbf{k}^j \bm{\alpha} > 0$. 

We can perform similar sensitivity analysis of $L_2$-BKLR and $L_1$-BKLR as that of $L_2$-BLR and $L_1$-BLR. Namely, if the absolute value of $\alpha_j$ is one or two orders of magnitude smaller than 1 or $\Delta \alpha_j$ is comprable with $\alpha_j$, then L2-BKLR is more sensitive than L1-BKLR.

\subsection{Support Vector Classification: Compare $l_1$ with $l_2$ constrained Loss Function}

First, we consider BLSVC-RHL and BLSVC-SHL.

For BLSVC-RHL, 
\begin{align}
\label{BLSVC_RHL_sensi}
\begin{split}
& \Bigg| \frac{\Delta \hat{C}_{BLSVC-RHL}^{(i)}}{\Delta w_i} \Bigg| = \\
& \Bigg| \frac{1}{\Delta w_i} \Bigg( \frac{w_i + \Delta w_i}{\sum\limits_{j, y_j \big( \langle \mathbf{w}, \mathbf{x}_T^j \rangle + \Delta w_i x_{j,i} \big) < 1} y_j x_{j,i}} - \frac{w_i}{\sum\limits_{j, y_j \langle \mathbf{w}, \mathbf{x}_T^j \rangle <1} y_j x_{j,i} } \Bigg) \Bigg|. 
\end{split}
\end{align}

For BLSVC-SHL, 
\begin{align}
\label{BLSVC_SHL_sensi}
\begin{split}
& \Bigg| \frac{\Delta \hat{C}_{BLSVC-SHL}^{(i)}}{\Delta w_i} \Bigg| = \\
&  \Bigg| \frac{1}{\Delta w_i} \Bigg( \frac{w_i + \Delta w_i}{\sum\limits_{j, y_j \big( \langle \mathbf{w}, \mathbf{x}_T^j \rangle + \Delta w_i x_{j,i} \big) < 1} 2 y_j x_{j,i} \big(1 - y_j \big( \langle \mathbf{w}, \mathbf{x}_T^j \rangle + \Delta w_i x_{j,i} \big) \big) } \\
& \quad - \frac{w_i}{\sum\limits_{j, y_j \langle \mathbf{w}, \mathbf{x}_T^j \rangle <1} 2 y_j x_{j,i} \big(1 - y_j \langle \mathbf{w}, \mathbf{x}_T^j \rangle \big) } \Bigg) \Bigg| .
\end{split}
\end{align}

Comparing Eqn~\ref{BLSVC_RHL_sensi} and Eqn~\ref{BLSVC_SHL_sensi}, we notice that their difference is between the factor $2\big(1 - y_j \big( \langle \mathbf{w}, \mathbf{x}_T^j \rangle + \Delta w_i x_{i,i} \big) \big)$ and 1. Taking into account the property of SVC, we know that when the training set $\mathbf{X}$ can be (approximately) linearly separable, then $y_j \langle \mathbf{w}, \mathbf{x}_T^j \rangle $ is close to 1, i.e., $1-y_j \langle \mathbf{w}, \mathbf{x}_T^j \rangle $ is a small positive number. Therefore, by adding $\Delta w_i$ such that the sign of $1- y_j \big( \langle \mathbf{w}, \mathbf{x}_T^j \rangle + \Delta w_i x_{i,i} \big) \big)$ is still positive, we conclude that $ 1- y_j \big( \langle \mathbf{w}, \mathbf{x}_T^j \rangle + \Delta w_i x_{i,i} \big) \big) < \frac{1}{2}$, and thus $\hat{C}_{BLSVC-SHL}^{(i)}$ is more sensitive than $\hat{C}_{BLSVC-RHL}^{(i)}$. 


Then, we consider BKSVC-RHL and BKSVC-SHL.

For BKSVC-RHL, 
\begin{align}
\label{BKSVC_RHL_sensi}
\begin{split}
& \Bigg| \frac{\Delta \hat{C}_{BKSVC-RHL}^{(i)}}{\Delta \alpha_i} \Bigg|  = \\ 
& \Bigg| \frac{1}{\Delta \alpha_i} \Bigg( \frac{\mathbf{k}^i \bm{\alpha} + k_{ii} \Delta \alpha_i}{\sum\limits_{j, y_j (\langle \bm{\alpha}, \mathbf{k}_j \rangle + \Delta \alpha_i k_{i,j}) <1} y_j k_{j,i}} - \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j, y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle <1} y_j k_{j,i} } \Bigg) \Bigg|.
\end{split}
\end{align}

For BKSVC-SHL
\begin{align}
\label{BKSVC_SHL_sensi}
\begin{split}
& \Bigg| \frac{\Delta \hat{C}_{BKSVC-SHL}^{(i)}}{\Delta \alpha_i} \Bigg| = \\
& \Bigg| \frac{1}{\Delta \alpha_i} \Bigg( \frac{\mathbf{k}^i \bm{\alpha} + k_{ii} \Delta \alpha_i}{\sum\limits_{j, y_j (\langle \bm{\alpha}, \mathbf{k}_j \rangle + \Delta \alpha_i k_{i,j}) <1} 2 y_j k_{j,i} \big( 1 - y_j (\langle \bm{\alpha}, \mathbf{k}_j \rangle + \Delta \alpha_i k_{i,j}) \big)} \\
& \quad -  \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j, y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle <1} 2 y_j k_{j,i} \big( 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle \big)} \Bigg) \Bigg|.
\end{split}
\end{align}

Similar results can be obtained, i.e., $\hat{C}_{BKSVC-SHL}^{(i)}$ is more sensitive than $\hat{C}_{BKSVC-RHL}^{(i)}$,  as $1 - y_j (\langle \bm{\alpha}, \mathbf{k}_j \rangle + \Delta \alpha_i k_{i,j}) < \frac{1}{2}$ is often satisfied. 





==> attack.tex <==
\section{Hyperparameter Stealing Attack}
\label{hyper_attack}

% \begin{sidewaystable*}
% \small
% \centering
% \caption{Summarization of all ML models.}
% \label{sum_ml}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
%   Category                &       \multicolumn{2}{c|}{ML Model}            & Obj. Func. & Loss Func. & Regression  & Est. Hyper. & 	\\ \hline
% \multirow{4}{*}{Regression} & \multirow{3}{*}{Linear} & RR & $\mathcal{L}_{RR}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X} \mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_2^2 $
%  & Least Square & $L_2$ & $\hat{\lambda}^{(i)}_{RR} = \frac{-\langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle}{w_i}$ &  \\ \cline{3-8} 
%                   &                   &  LASSO & $\mathcal{L}_{LASSO}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_1.
% $ & Least Square & $L_1$ & $\hat{\lambda}^{(i)}_{LASSO} =  
% \begin{cases}
% 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if }  w_i < 0 \\
% -2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if } w_i > 0 
% \end{cases} $ &  \\ \cline{3-8} 
%                   &                   & ENet & $ \mathcal{L}_{ENet}(\lambda_2, \lambda_1, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda_2 \| \mathbf{w} \|_2^2 + \lambda_1 \| \mathbf{w} \|_1 $ & Least Square & $L_2 + L_1$ & $\hat{\bm{\lambda}}_{ENet} = \left( \mathbf{A}^T \mathbf{A} \right)^{-1} \mathbf{A}^T \mathbf{b} $ &  \\ \cline{2-8} 
%                   &     Nonlinear       & KRR       & $\mathcal{L}_{KRR}(\lambda, \mathbf{w}^\prime) = \| \mathbf{y}-\Phi(\mathbf{X}) \mathbf{w}^\prime \|_2^2 + \lambda \| \mathbf{w}^\prime \|_2^2$ &  Least Square & $L_2$ & $\hat{\lambda}^{(j)}_{KRR} = \frac{y_j - \mathbf{k}^{j} \alpha_j}{\alpha_j}. 
% $ & \\ \hline

           
% \multirow{4}{*}{BLR Classification} & \multirow{2}{*}{Linear}  & L2-BLR & $\mathcal{L}_{L2-BLR}(\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};\mathbf{x}_i,y_j) + \lambda \| \mathbf{w} \|_2^2 $
%  & Cross Ent. & $L_2$ & $\hat{\lambda}^{(i)}_{L2-BLR} = - \frac{\langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle}{2 w_i} $  & \\ \cline{3-8} 
%                   &                    & L1-BLR & $\mathcal{L}_{L1-BLR}(\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};\mathbf{x}_i,y_j) + \lambda \| \mathbf{w} \|_1 $ & Cross Ent. & $L_1$ & $\hat{\lambda}^{(i)}_{L1-BLR} = \begin{cases}
% - \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i > 0 \\
%  \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i < 0 \end{cases} $  & \\ \cline{2-8} 
                  
%                   & \multirow{2}{*}{Nonlinear}  & L2-BKLR & $\mathcal{L}_{L2-BKLR}(\lambda, \bm{\alpha}) = \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & Cross Ent. & $L_2$ & $\hat{\lambda}^{(j)}_{L2-BKLR} = - \frac{h_{\bm{\alpha}}(\mathbf{k}_j) - y_j} {2 \alpha_j}$ &  \\ \cline{3-8} 
                  
%                   &                    &  L1-BKLR & $\mathcal{L}_{L1-BKLR}(\lambda, \bm{\alpha}) = \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + \lambda \| \mathbf{K} \bm{\alpha} \|_1 $ & Cross Ent. & $L_1$ & $\hat{\lambda}^{(j)}_{L1-BKLR} = \begin{cases} y_j - h_{\bm{\alpha}}(\mathbf{k}_j)  & \text{if } \mathbf{k}^j \bm{\alpha} > 0 \\
%  h_{\bm{\alpha}}(\mathbf{k}_j) - y_j  & \text{if } \mathbf{k}^j \bm{\alpha} < 0 \end{cases} $ & \\ \hline

% \multirow{2}{*}{MLR Classification} & Linear & L2-MLR & $\mathcal{L}_{L2-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}_i, \mathbf{y}^j) + \lambda \sum_{c=1}^C \| \mathbf{w}_c \|_2^2 $  & Max. Ent. & $L_2$ & $\hat{
% \lambda}^{(i,c)}_{L2-MLR} = - \frac{\langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle }{2 w_{i,c}} $ & \\ \cline{2-3} 
% % 						  & Nonlinear & L1-MLR & $\mathcal{L}_{L2-MKLR}(
% \lambda, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + 
% \lambda \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c $ & Max. Ent. & $L_1$ & $\mathcal{L}_{L2-MKLR}(
% \lambda, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + 
% \lambda \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c $ & \\ \hline

% % \multirow{4}{*}{SVC Classification} & \multirow{2}{*}{Linear}  & BLSVC-RHL & $\mathcal{L}_{BLSVC-RHL}(T, \mathbf{w}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \mathbf{w}, 
% \mathbf{x}_i \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2 $  & RHL & $L_2$ & $\hat{T}^{(i)}_{BLSVC-RHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, 
% \mathbf{x}_i \rangle < 1} y_j {x}_{j,i}}$ &  \\ \cline{3-8} 
% %                   &                    & BLSVC-SHL & $\mathcal{L}_{BLSVC-SHL}(T, \mathbf{w}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \mathbf{w}, 
% \mathbf{x}_i \rangle)^2 + \frac{1}{2} \| \mathbf{w} \|_2^2 $ & SHL & $L_2$ & $\hat{T}^{(i)}_{BLSVC-SHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, 
% \mathbf{x}_i \rangle \leq 1} 2y_j {x}_{j,i} (1 - y_j \langle \mathbf{w}, 
% \mathbf{x}_i \rangle) }$ &  \\ \cline{2-8} 
% %                   & \multirow{2}{*}{Nonlinear}  & BKSVC-RHL & $\mathcal{L}_{BKSVC-RHL}(T, \bm{\alpha}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle ) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & RHL & $L_2$ & $\hat{T}^{(i)}_{BKSVC-RHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j, y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle <1} y_j k_{j,i}}$ &  \\ \cline{3-8} 
%                   &                    & BKSVC-SHL & $\mathcal{L}_{BKSVC-SHL}(T, \bm{\alpha}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )^2 + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & SHL & $L_2$ & $\hat{T}^{(i)}_{BKSVC-SHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle \leq 1} 2y_j {k}_{j,i} (1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle)}$ & \\ \hline

% \end{tabular}
% \end{sidewaystable*}

\begin{sidewaystable*}
\small
\centering
\caption{Summarization of all ML models.}
\label{sum_ml}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
  Category                &       \multicolumn{2}{c|}{ML Model}       & Objective Function & Loss Function & Regularization \\ \hline
\multirow{4}{*}{Regression} & \multirow{3}{*}{Linear} & RR & $\mathcal{L}_{RR}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X} \mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_2^2 $	& Least Square & $L_2$ \\ \cline{3-6} 
                  &                   &  LASSO & $\mathcal{L}_{LASSO}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_1. $ & Least Square & $L_1$ \\ \cline{3-6} 
                  &                   & ENet & $ \mathcal{L}_{ENet}(\lambda_2, \lambda_1, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda_2 \| \mathbf{w} \|_2^2 + \lambda_1 \| \mathbf{w} \|_1 $ & Least Square & $L_2 + L_1$ \\ \cline{2-6} 
                  &     Nonlinear       & KRR       & $\mathcal{L}_{KRR}(\lambda, \bm{\alpha}) = \| \mathbf{y} - \mathbf{K} \bm{\alpha} \|_2^2 + \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha}$ &  Least Square & $L_2$ \\ \hline

           
\multirow{4}{*}{BLR Classification} & \multirow{2}{*}{Linear}  & L2-BLR & $\mathcal{L}_{L2-BLR}(
\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};
\mathbf{x}_i,y_j) + 
\lambda \| \mathbf{w} \|_2^2 $
 & Cross Ent. & $L_2$ \\ \cline{3-6} 
                  &                    & L1-BLR & $\mathcal{L}_{L1-BLR}(
\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};
\mathbf{x}_i,y_j) + 
\lambda \| \mathbf{w} \|_1 $ & Cross Ent. & $L_1$ \\ \cline{2-6} 
                  
                  & \multirow{2}{*}{Nonlinear}  & L2-BKLR & $\mathcal{L}_{L2-BKLR}(
\lambda, \bm{\alpha}) = \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + 
\lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & Cross Ent. & $L_2$ \\ \cline{3-6} 
                  
                  &                    &  L1-BKLR & $\mathcal{L}_{L1-BKLR}(
\lambda, \bm{\alpha}) = \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + 
\lambda \| \mathbf{K} \bm{\alpha} \|_1 $ & Cross Ent. & $L_1$ \\ \hline

\multirow{2}{*}{MLR Classification} & Linear & L2-MLR & $\mathcal{L}_{L2-MLR}(
\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};
\mathbf{x}_i, \mathbf{y}^j) + 
\lambda \sum_{c=1}^C \| \mathbf{w}_c \|_2^2 $  & Max. Ent. & $L_2$ \\ \cline{2-3} 
						  & Nonlinear & L1-MLR & $\mathcal{L}_{L2-MKLR}(
\lambda, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + 
\lambda \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c $ & Max. Ent. & $L_1$ \\ \hline

\multirow{4}{*}{SVC Classification} & \multirow{2}{*}{Linear}  & BLSVC-RHL & $\mathcal{L}_{BLSVC-RHL}(T, \mathbf{w}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2 $  & RHL & $L_2$ \\ \cline{3-6} 
                  &                    & BLSVC-SHL & $\mathcal{L}_{BLSVC-SHL}(T, \mathbf{w}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle)^2 + \frac{1}{2} \| \mathbf{w} \|_2^2 $ & SHL & $L_2$ \\ \cline{2-6} 
                  & \multirow{2}{*}{Nonlinear}  & BKSVC-RHL & $\mathcal{L}_{BKSVC-RHL}(T, \bm{\alpha}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle ) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & RHL & $L_2$ \\ \cline{3-6} 
                  &                    & BKSVC-SHL & $\mathcal{L}_{BKSVC-SHL}(T, \bm{\alpha}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )^2 + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & SHL & $L_2$ \\ \hline

\hline
  Category                &       \multicolumn{2}{c|}{ML Model}            & Stealed Hyperparameter & Optimization Algorithm & Solution Type \\ \hline
            
\multirow{4}{*}{Regression} & \multirow{3}{*}{Linear} & RR & $\hat{\lambda}^{(i)}_{RR} = \frac{-\langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle}{w_i}$ & SVD~\cite{weisstein2002singular} & I \\ \cline{3-6}

                  &                   &  LASSO & $\hat{\lambda}^{(i)}_{LASSO} =  \begin{cases}
2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if }  w_i < 0 \\
-2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if } w_i > 0 
\end{cases} $ & CD~\cite{friedman2010regularization} & II \\ \cline{3-6} 
                  &                   & ENet & $\hat{\bm{\lambda}}_{ENet} = \left( \mathbf{A}^T \mathbf{A} \right)^{-1} \mathbf{A}^T \mathbf{b} $ & CD & II \\ \cline{2-6} 
                  &     Nonlinear       & KRR       & $\hat{\lambda}^{(j)}_{KRR} = \frac{y_j - \mathbf{k}^{j} \alpha_j}{\alpha_j} $ & SVD & I \\ \hline

\multirow{4}{*}{BLR Classification} & \multirow{2}{*}{Linear}  & L2-BLR & $\hat{
\lambda}^{(i)}_{L2-BLR} = - \frac{\langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle}{2 w_i} $  & \multirow{4}*{LBFGS~\cite{liu1989limited}}  & \multirow{4}*{II} \\ \cline{3-4}

                  &                    & L1-BLR & $\hat{
\lambda}^{(i)}_{L1-BLR} = \begin{cases}
- \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i > 0 \\
 \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i < 0 \end{cases} $  & & \\ \cline{2-4} 
                  
                  & \multirow{2}{*}{Nonlinear}  & L2-BKLR & $\hat{
\lambda}^{(j)}_{L2-BKLR} = - \frac{h_{\bm{\alpha}}(\mathbf{k}_j) - y_j} {2 \alpha_j}$ &  & \\ \cline{3-4} 
                  
                  &                    &  L1-BKLR & $\hat{
\lambda}^{(j)}_{L1-BKLR} = \begin{cases} y_j - h_{\bm{\alpha}}(\mathbf{k}_j)  & \text{if } \mathbf{k}^j \bm{\alpha} > 0 \\ h_{\bm{\alpha}}(\mathbf{k}_j) - y_j  & \text{if } \mathbf{k}^j \bm{\alpha} < 0 \end{cases} $ &  & \\ \hline

\multirow{2}{*}{MLR Classification} & Linear & L2-MLR & $\hat{
\lambda}^{(i,c)}_{L2-MLR} = - \frac{\langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle }{2 w_{i,c}} $ & \multirow{2}{*}{Newton-CG~\cite{wright1999numerical}} & \multirow{2}{*}{II} \\ \cline{2-4} 
						  & Nonlinear & L1-MLR & $\mathcal{L}_{L2-MKLR}(
\lambda, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + 
\lambda \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c $ & & \\ \hline

\multirow{4}{*}{SVC Classification} & \multirow{2}{*}{Linear}  & BLSVC-RHL & $\hat{T}^{(i)}_{BLSVC-RHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle < 1} y_j {x}_{j,i}}$ & SMO~\cite{platt1998sequential} & \multirow{4}*{III} \\ \cline{3-5} 
                  &                    & BLSVC-SHL & $\hat{T}^{(i)}_{BLSVC-SHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle \leq 1} 2y_j {x}_{j,i} (1 - y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle) }$ & SGD~\cite{bottou2010large} & \\ \cline{2-5} 
                  & \multirow{2}{*}{Nonlinear}  & BKSVC-RHL & $\hat{T}^{(i)}_{BKSVC-RHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j, y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle <1} y_j k_{j,i}}$ & SMO & \\ \cline{3-5} 
                  &                    & BKSVC-SHL & $\hat{T}^{(i)}_{BKSVC-SHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle \leq 1} 2y_j {k}_{j,i} (1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle)}$ & SGD & \\ \hline

\end{tabular} \\
\small
%Note: Obj. Func. is short for ``Objective Function". Similarly, Loss Func., Regu., Regression, Classification, Linear, Nonlinear, Est. Hyper., Opt. Alg., and Sol. Type are short for ``Loss Function", ``Regularization", ``Regression", ``Classification", ``Linear", ``Nonlinear", ``Estimated Hyperparameter", ``Optimization Algorithm", and ``Solution Type"; 
Note: SVD is Singular Value Decomposition; CD is Coordinate Descent; CG is Conjugate Gradient; SMO is Sequential Minimal Optimization; SGD is Stochastic Gradient Descent.
\end{sidewaystable*}

\subsection{Our Attack Framework}

From optimization's perspective, we know that the optimal parameters and optimal hyperparameter of a ML algorithm are learnt via minimizing its objective function. In other words, once the minimal value of a convex objective function is acheived, the model parameters and hyperparameter should be optimal. 
%However, the \emph{global minimal} value can be guaranteed if and only if the objective function is \emph{convex}, as shown in Definition~\ref{app:cvx_prop}. 
Therefore, from an attacker's view, if he knows the convex objective function (of a ML algorithm) and the optimal parameters, then he can steal the hyperparamete
%another way to understand is that if the objective function is convex and the optimal parameters are given, then the optimal hyperparameters can be achieved 
by setting the subgradient of the objective function with respect to the parameters to be zero. %if the objective function is \emph{smooth} (or \emph{nonsmooth}). 
With such an intuition, our attack framework is defined as  
\begin{align}
%\label{attack_frame}
&\text{\bf For linear models:} \nonumber \\
& \frac{\mathcal{L}(\mathbf{w})}{\partial \mathbf{w}} = \sum_{i=1}^n \frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial \mathbf{w}} + \lambda \frac{\partial \text{R}(\mathbf{w})}{\partial \mathbf{w}}. \label{attack_frame_lin}\\
%&\mathcal{L}(\mathbf{w}) = \sum_{i=1}^n \text{L}(\mathbf{x}_i, y_i, \mathbf{w}) +  \lambda \text{R}(\mathbf{w}) \\
%& \qquad = \sum_{i=1}^n \text{Loss}(\mathbf{w}; \mathbf{x}_i, y_i) + \sum_{j} h_j \text{Reg}_j(\mathbf{w}),   
&\text{\bf For kernel models:} \nonumber \\
& \frac{\mathcal{L}(\bm{\alpha})}{\partial \bm{\alpha}} = \sum_{i=1}^n \frac{\partial \text{L}(\bm{\alpha}; \phi(\mathbf{x}_i), y_i)}{\partial \bm{\alpha}} + \lambda \frac{\partial \text{R}(\bm{\alpha})}{\partial \bm{\alpha}}, \label{attack_frame_kernel}
\end{align}
where $\frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial \mathbf{w}} = \left[\frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial w_1}; \frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial w_2}; \cdots; \frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial w_m} \right]$ and other terms have a similar form.
%More specifically, we can leverage \emph{gradient-based} method if the objective function is \emph{smooth} or \emph{subgradient-based} method if it is \emph{nonsmooth}. 
%Mathematically, if the data samples are drawn from the original space, then
% \begin{small} 
% \begin{align}
% \label{attack_frame}
% \begin{split}
% \frac{\mathcal{L}(\mathbf{w}, \mathbf{h})}{\partial \mathbf{w}} & = \sum_{i=1}^n \frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial \mathbf{w}} + \lambda \frac{\partial \text{R}(\mathbf{w})}{\partial \mathbf{w}}. 
% \end{split}
% \end{align}
% \end{small}
%Note that Eqn~\ref{attack_frame} a $m$-dim vector-based derivative. 

Setting Eqns~\ref{attack_frame_lin} and~\ref{attack_frame_kernel} to be $\mathbf{0}$, we then have a system of $m$ equations for linear models and a system of $n$ equations for kernel models to estimate a single $\lambda$. 
Specifically, for linear models, we denote 
%For linear models, we denote $\hat{\lambda}^{(i)}$ as the estimate for $i$-th equation (the subgradient with respect to $w_i$), and denote 
\begin{small} 
\begin{align*}
\mathbf{a} = \left[
\begin{array}{c}
\frac{\partial \text{R}(\mathbf{w})}{\partial w_1} \\
\frac{\partial \text{R}(\mathbf{w})}{\partial w_2} \\
\vdots \\
\frac{\partial \text{R}(\mathbf{w})}{\partial w_m} \\
\end{array}
\right], \, 
% \mathbf{A} = \left[
% \begin{array}{cccc} 
% \frac{\partial \text{R}(\mathbf{w})}{\partial w_1} & 0 & \cdots & 0 \\
% 0 & \frac{\partial \text{R}(\mathbf{w})}{\partial w_1} & \cdots & 0 \\
% \vdots & \vdots \\
% 0 & \cdots & 0 & \frac{\partial \text{R}(\mathbf{w})}{\partial w_m} \\
% \end{array}
% \right], \\
\mathbf{b} = \left[ 
\begin{array}{c}
\sum_{i=1}^n \frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial {w}_1} \\
\sum_{i=1}^n \frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial {w}_2} \\
\vdots \\
\sum_{i=1}^n \frac{ \partial \text{L}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial {w}_m} \\
\end{array}
\right]. 
\end{align*}
\end{small}
Then, Eqn~\ref{attack_frame_lin} becomes 
\begin{align}
\label{attack_lin_soln}
\lambda \mathbf{a} + \mathbf{b} = 0.
\end{align}

Usually, Eqn.~\ref{attack_lin_soln} has no solution. To address the issue, we resort to \emph{least square regression} and then Eqn.~\ref{attack_lin_soln} can be written into the normal equation~\cite{montgomery2015introduction}:
\begin{align}
\label{norm_eqn}
 \mathbf{a}^T \mathbf{a} \lambda + \mathbf{a}^T \mathbf{b} = 0.
\end{align}
Hence, $\lambda$ can be estimated as 
\begin{align}
\label{fianl_est}
\hat{\lambda} = -(\mathbf{a}^T \mathbf{a})^{-1}(\mathbf{a}^T \mathbf{b}).
%\hat{\lambda} = -\frac{\mathbf{a}^T \mathbf{b}}{\mathbf{a}^T \mathbf{a}}.
\end{align}
% \begin{align}
% \hat{\bm{\lambda}} = - \mathbf{A}^{-1} \mathbf{b},  
% \end{align}
%and we take the average of elements of $\hat{\bm{\lambda}}$, i.e., $\hat{\lambda} = \frac{1}{m} \sum_{j=1}^m \hat{\lambda}^{(j)}$, as the final estimate of $\lambda$.
For kernel models, we can derivate a similar form by just replacing $\mathbf{w}$ with $\bm{\alpha}$, $\mathbf{x}_i$ with $\phi(\mathbf{x}_i)$, and $m$ with $n$.

%in the kernel-mapped feature space) and thus can estimate each hyperparameter $h_j$. 
In the paper, we call this hyperparameter stealing as \textbf{subgradient-based attack}.

%In practice, for different regression and classification algorithms, loss functions and regularizations are different. For instance, loss functions can be \emph{cross entropy}~\cite{hosmer2013applied}, \emph{maximum entropy}~\cite{hosmer2013applied}, \emph{regular hinge loss (RHL)}~\cite{fan2008liblinear}, and \emph{square hinge loss (SHL)}~\cite{fan2008liblinear}, etc. Regularizations can be \emph{$L_1$-norm}, \emph{$L_2$-norm}, and the combination of $L_1$-norm and $L_2$-norm, etc. 
%Throughout this paper, we only focus on well-known convex ML models. For regression, we take ridge regression, LASSO, ElasticNet as examples; For classification, we choose LR and SVC. 

In the following, we will provide the detail as how to steal the hyperparameter of well-known convex-inducing regression and classification algorithm listed in Table~\ref{}. 
%For simplicity, we use the same notation for the same type model for simplicity. For instance, for regression models, we adopt $\bm{\lambda}$; for Logistic Regression (LR)-based models, we adopt $\lambda$; for Support Vector Classification (SVC)-based models, we adopt $T$.

\subsection{Attack on Convex-Induced Regression Models} 
\label{attack_cvx_reg}

We consider attacks on both convex linear and kernel regression models.

\subsubsection{Linear Regression Models} 
\label{cvx_reg_lin}

We aim at stealing the hyperparameter of Ridge Regression (RR)~\cite{hoerl1970ridge}, LASSO~\cite{tibshirani1996regression}, and Elastic Net (ENet)~\cite{zou2005regularization}. 
Due to space limitation, we only show the detail as how to steal the hyperparameter of RR. The results of LASSO and ENet are list in Table~\ref{sum_ml} and their derivation are provided in Appendix~\ref{app:cvx_reg}.
%For simplicity, we only show the objective function and the stealed hyperparameter(s) of each model. The derivation details are provided in Appendix~\ref{app:cvx_reg}.

\myparatight{Ridge Regression (RR)} The objective function of RR is 
\begin{align}
\label{ridge_reg}
\mathcal{L}(\mathbf{w}) = \| \mathbf{y}-\mathbf{X}^T \mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_2^2,
\end{align}
where it uses least square loss function and $L_2$ regularization. In general, the optimal $\mathbf{w}$ is analytically solved via SVD algorithm~\cite{weisstein2002singular}.

Taking its derivative with respect to $\mathbf{w}$ yields
\begin{align*}
\frac{\partial \mathcal{L}(\mathbf{w})}{\partial \mathbf{w}} = -2 \mathbf{X y} + 2 \mathbf{X}\mathbf{X}^T\mathbf{w} + 2 \lambda \mathbf{w}. 
\end{align*}

% Rewriting Eqn.~\ref{ridge_reg} in terms of each $w_j$ and taking its derivative with respect to $w_j$ yields
% \begin{align*}
% %\label{ridge_reg_grad}
% \begin{split}
% \frac{\partial \mathcal{L}(\mathbf{w})}{\partial w_j} & = 2 \langle \mathbf{x}_T^j, \mathbf{x}_T^j \rangle w_j - 2 \left\langle \mathbf{x}_T^j, \mathbf{r}_j \right \rangle + 2 \lambda w_j,
% \end{split}
% \end{align*}
% where $\mathbf{r}_j = \mathbf{y}-\mathbf{X}^T_{:,-j} \mathbf{w}_{-j}$ is the residual that all features are used except the $i$-th feature to approximate $\mathbf{y}$.
Setting it to be $\mathbf{0}$ and comparing it with Eqn.~\ref{norm_eqn}, we have 
$\mathbf{a} = \mathbf{w}$ and $\mathbf{b} = \mathbf{X} (\mathbf{X}^T\mathbf{w} - \mathbf{y})$. 

% In this case, $\mathbf{a} = \left[ ;\right]$
% Setting it to be 0, we can estimate $\lambda$ as
% \begin{align}
% \label{ridge_reg_soln}
% \hat{\lambda} = \frac{1}{m} \sum_{j=1}^m \frac{-\langle \mathbf{x}_T^j, \mathbf{x}_T^j \rangle w_j + \left\langle \mathbf{x}_T^j, \mathbf{r}_j \right\rangle}{w_j}. 
% \end{align}
%where $\mathbf{r}_i = \mathbf{y}-\mathbf{X}_{:,-i} \mathbf{w}_{-i}$ is the residual that all features are used except the $i$-th feature to approximate $\mathbf{y}$. 

%Eqn~\ref{ridge_reg_soln} implies that if we are provided $\mathbf{w}$ by machine learning service provider (who achieves it using some training dataset and certain model selection (e.g., cross validataion, AIC, BIC) technique). Then, we can ``steal" the true hyperparameter $\lambda$, denoted as $\hat{\lambda}_1$. 

%Theoretically, each estimated $\hat{\lambda}^{(i)}_{RR}$ should be the exact $\lambda$. We demonstrate that our estimates are indeed accurate from the experimental results. 

% \myparatight{LASSO} The objective function is 
% \begin{align}
% \label{lasso}
% \mathcal{L}_{LASSO}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_1.
% \end{align}

% Notice that $\| \mathbf{w} \|_1$ is \emph{not differentiable} when $w_i=0$. To handle such a nonsmooth function, we need to extend the notion of gradient to \emph{subgradient}, as defined above. Setting the \emph{subgradient} of $\mathcal{L}_{LASSO}$ with respect to $w_i$ to be 0 yields 
% \begin{align}
% \label{lasso_soln}
% \hat{\lambda}^{(i)}_{LASSO} =  
% \begin{cases}
% 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if }  w_i < 0 \\
% -2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if } w_i > 0 
% \end{cases}
% \end{align}
 
% Setting $\frac{\partial \mathcal{L}_{LASSO}}{\partial w_i} = 0$, we have three cases of values of $w_i$, which depends on the value of $\lambda$ and $\left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle$, as follows: 
% \begin{align}
% w_i = 
% \begin{case}
% (2 \left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle + \lambda) / (2 \| \mathbf{x}_i \|_2^2) \quad \text{if} \, c_j < -\lambda \\
% 0 \quad \text{if} \, c_j \in [-\lambda, \lambda] \\
% (2 \left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle - \lambda) / (2 \| \mathbf{x}_i \|_2^2) \quad \text{if} \, c_j > \lambda 
% \end{case}
% \end{align}

% Note that if $\lambda \geq \lambda_{\max} = \| \mathbf{X}^T \mathbf{y} \|_{\infty} = \max_i |\langle \mathbf{y}, \mathbf{x}_i \rangle|$, then $\mathbf{w} = \mathbf{0}$. It is because $\mathbf{0}$ is optimal if $(\mathbf{X}^T \mathbf{y})_j \in [-\lambda, \lambda]$, for any $j$. Therefore, $\hat{\lambda}^{(i)}_{LASSO} < \max_i |\langle \mathbf{y}, \mathbf{x}_i \rangle|$.

%The value is obtained by using the fact that $\mathbf{0}$ is optimal if $(\mathbf{X}^T \mathbf{y})_j \in [-\lambda, \lambda]$, for any j. Therefore, we have $\hat{\lambda}^{(i)}_{LASSO} < \max_i |\langle \mathbf{y}, \mathbf{x}_i \rangle|$.

% \subsubsection{Support Vector Regression}

% \begin{align}
% \label{svr}
% \mathcal{L}_{SVR}(T, \mathbf{w}) = T \sum_{j=1}^n L_{\epsilon}(y_j, \langle \mathbf{w}, \mathbf{x}_i \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2,
% \end{align}
% where 
% \begin{align}
% L_{\epsilon}(y_j, \langle \mathbf{w}, \mathbf{x}_i \rangle) = 
% \begin{cases}
% 0 & \text{if } |y_j - \langle \mathbf{w}, \mathbf{x}_i \rangle| \leq \epsilon \\
% |y_j - \langle \mathbf{w}, \mathbf{x}_i \rangle | - \epsilon  & \text{if } |y_j - \langle \mathbf{w}, \mathbf{x}_i \rangle| > \epsilon
% \end{cases}
% \end{align}
% is the so called $\epsilon$-\textbf{insensitive loss function}. It indicates that any point lying insider an $\epsilon$-tube around the prediction is not penalized. 
% %$\hat{y}_j = \langle \mathbf{w}, \mathbf{x}_i \rangle$ and $T = 1 / \lambda$ is a regularization constant.
% Note that the objective is convex, but is not differentiable at the points $y_j = \langle \mathbf{w}, \mathbf{x}_i \rangle + \epsilon$ and $y_j = \langle \mathbf{w}, \mathbf{x}_i \rangle - \epsilon$ due to the absolute value function in the loss term. 

% % One popular approach is to formulate the problem as a constrained optimization problem by introducing \textbf{slack parameters} to represent the degree to which each sample lies outside the $\epsilon$-tube. Specifically, we rewrite the objective as 
% % \begin{align}
% % \begin{split}
% % & \mathcal{L}_{SVR}(\mathbf{w},\bm{\xi}_+, \bm{\xi}_+, T) = T \sum_{j=1}^n ( \xi^j_+ + \xi^j_- ) + \frac{1}{2} \| \mathbf{w} \|_2^2 \\
% % & \text{s.t. } \langle \mathbf{w} \mathbf{x}^j \rangle - \epsilon - \xi^j_- \leq y_j \leq \langle \mathbf{w} \mathbf{x}^j \rangle + \epsilon + \xi^j_+, \xi^j_+, \xi^j_- \geq 0, \forall j.
% % \end{split}
% % \end{align}

% % The subgradient of $L_{\epsilon}$ with respect to $\mathbf{w}$ is then given by 
% % \begin{align}
% % \frac{\partial L_{\epsilon}(y_j, \langle \mathbf{w}, 
% \mathbf{x}_i \rangle)}{\partial \mathbf{w}} = 
% % \begin{cases}
% % -
% \mathbf{x}_i & \text{if } \langle \mathbf{w}, 
% \mathbf{x}_i \rangle < y_j - \epsilon \\
% % \left[ -
% \mathbf{x}_i, \mathbf{0} \right] & \text{if } \langle \mathbf{w}, 
% \mathbf{x}_i \rangle = y_j - \epsilon \\
% % \mathbf{0} & \text{if } y_j - \epsilon < \langle \mathbf{w}, 
% \mathbf{x}_i \rangle < y_j + \epsilon \\
% % \left[ \mathbf{0}, 
% \mathbf{x}_i \right] & \text{if } \langle \mathbf{w}, 
% \mathbf{x}_i \rangle = y_j + \epsilon \\
% % 
% \mathbf{x}_i & \text{if } \langle \mathbf{w}, 
% \mathbf{x}_i \rangle > y_j + \epsilon
% % \end{cases}
% % \end{align}


% %Here, we consider the case when $\epsilon=0$.

% In practice, for two non-differential points, the subgradient is set to be 0.
% Finally, setting the derivative of $\mathcal{L}_{SVR}$ with respect to $\mathbf{w}$ to zero, we estimate $T$ as  
% \begin{align}
% \hat{T}^{(i)} = \frac{w_i}{\sum\limits_{j,\langle \mathbf{w}, 
% \mathbf{x}_i \rangle < y_j - \epsilon} x_{j,i} - \sum\limits_{j,\langle \mathbf{w}, 
% \mathbf{x}_i \rangle > y_j + \epsilon} x_{j,i} }
% % \end{align}

% It is critical here, as in any regularization scheme, that a proper value is chosen for $C$, the penalty factor. If it is too large, we have a high penalty for nonseparable points and we may store many support vectors and overfit. If it is too small, we may have underfitting." 
% Alpaydin (2004), page 224
% \begin{align}
% \hat{T}^{(i)} = 
% \begin{cases}
% \frac{w_i}{x_{j,i}} & \text{if } \langle \mathbf{w}, 
%\mathbf{x}_i \rangle < y_j \\
% -\frac{w_i}{x_{j,i}} & \text{if } \langle \mathbf{w}, 
%\mathbf{x}_i \rangle > y_j
% \end{cases}
% \end{align}

\subsubsection{Kernel Regression Models}
\label{cvx_reg_nonlin}
%\subsubsection{Nonlinear Model}

% So far, we have noticed that linear models represent each data sample in a \emph{fixed, explicit, and finite dimensional feature space},. However, for certain types of data, it is not clear how they can be best represented using a fixed dimensional vector. 
% For instance, how can we represent a text document, which can be of variable length? 
% To tackle such problems, one popular way is to leverage a \textbf{nonlinear kernel function} $\kappa$ that measures the similarity between data samples in an \emph{implicit, abstract, even infinite dimensional feature space}. $\kappa$ is nonnegative and symmetric (See  Definition~\ref{app:kernel} in Appendix). As a results, linear regression models that uses a nonlinear kernel function becomes \emph{nonlinear regression models}. 

%In the paper, we only deal with Kernel RR (KRR)~\cite{vovk2013kernel}, as the kernel version of LASSO and ENet are seldom used in practice. 


For kernel regression models, we only deal with Kernel RR (KRR)~\cite{vovk2013kernel}, as the kernel version of LASSO and ENet are seldom used in practice. 

We use \textbf{Gaussian kernel}, a Mercer kernel (See Definition~\ref{app:kernel} in Appendix), as the kernel function.  It is defined as 
%$\kappa(\mathbf{x}, \mathbf{x}^{\prime}) = \exp ( \| \mathbf{x} - \mathbf{x}^\prime \|_2^2 ／ 2 \sigma^2 )$,
\begin{small}
\begin{align}
\label{gaussian_kernel}
%\kappa(\mathbf{x}, \mathbf{x}^\prime) = \exp \big( \| \mathbf{x} - \mathbf{x}^\prime \|_2^2 ／ 2 \sigma^2} \big), 
\kappa(\mathbf{x}, \mathbf{x}^\prime) = \phi(\mathbf{x}) \phi(\mathbf{x}^\prime) = \exp \bigg( -\frac{1}{2\sigma^2} \| \mathbf{x} - \mathbf{x}^\prime \|_2^2 \bigg), 
\end{align}
\end{small}
where $\sigma^2$ is the bandwidth. 
% \begin{itemize}
% \item Gaussian kernel: $\kappa(\mathbf{x}, \mathbf{x}^\prime) = \exp \big( \frac{\| \mathbf{x} - \mathbf{x}^\prime \|_2^2}{2 \sigma^2} \big)$, where $\sigma^2$ is the bandwidth.
% \item Polynomial kernel: $\kappa(\mathbf{x}, \mathbf{x}^\prime) = (\langle \mathbf{x}, \mathbf{x}^\prime \rangle)^d$, where $d$ is the degree of the polynomial. 
% \end{itemize}      
%Note that aforementioned linear models use the simplest linear kernel, i.e.,  $\kappa(\mathbf{x}, \mathbf{x}^\prime) = \langle \mathbf{x}, \mathbf{x}^\prime \rangle $.

% In general, if the kernel is Mercer kernel (positive definite kernel), then there exists a function $\phi$ mapping $\mathbf{x} \in \mathbb{R}^m$ to $\phi(\mathbf{x}) \in \mathbb{R}^M $ such that 
% \begin{align}
% \kappa(\mathbf{x}, \mathbf{x}^\prime) = \langle \phi(\mathbf{x}), \phi(\mathbf{x}^\prime) \rangle,
% \end{align}
% is an inner product of some feature vectors that are implicitly defined by $\phi$, which depends on the eigen functions of $\kappa$.  Hence, $M$ can be potentially infinite dimension.     

%For nonlinear regression, we only focus on kernel ridge regression (KLR)~\cite{welling2013kernel}, as the kernel version of LASSO and Elastic Net is seldom used in practice. 

\myparatight{Kernel RR (KRR)} 
%Given kernel mapping $\Phi : \mathbb{R}^m \rightarrow \mathbb{R}^M$, where $M$ is the dimension of the feature space. Then, the objective function of KRR is 
%\subsubsection{Kernel Ridge Regression}
% \begin{small}
% \begin{align}
% \label{kernel_ridge_primal} 
% \mathcal{L}_{KRR}(\lambda, \mathbf{w}^\prime) = \| \mathbf{y}-\Phi(\mathbf{X}) \mathbf{w}^\prime \|_2^2 + \lambda \| \mathbf{w}^\prime \|_2^2,
% \end{align}
% \end{small}
% where $\Phi(\mathbf{X}) = \left[ \phi(\mathbf{x}^1_T); \phi(\mathbf{x}^2_T); \cdots; \phi(\mathbf{x}^n_T) \right] \in \mathbb{R}^{n \times M}$. 

% However, we point out that $\lambda$ cannot be solved using Eqn~\ref{kernel_ridge_primal}, as the exact form of each mapped sample $\phi(\mathbf{x}_i)$ is unknown. Fortunately, we can leverage \emph{Dual Representer Theorem}~\cite{scholkopf2001generalized}, with which $\mathbf{w}^\prime$ can be rewritten as a linear combination of $\phi(\mathbf{x}_i)$ with an associated coefficient $\alpha_j$. Specifically, 
% \begin{small}
% \begin{align}
% \mathbf{w}^\prime = \sum_{j=1}^n \alpha_j \phi(\mathbf{x}_i) = \Phi(\mathbf{X})^T \bm{\alpha}.
% \end{align} 
% \end{small}
% Note that $\bm{\alpha}$ is an $n$-dim vector, same size as the number of samples. 
% Accordingly, $\mathbf{w}^\prime$ and $ \bm{\alpha}$ are called \textbf{primal parameters} and \textbf{dual parameters}.

% In doing so, we can solve $\lambda$ using $n$-dim $\bm{\alpha}$ instead of $M$-dim $\mathbf{w}^\prime$. 
%Speficically, substituting $\mathbf{w}^\prime$ with $\Phi(\mathbf{X})^T \bm{\alpha}$, Eqn~\ref{kernel_ridge_primal} becomes 
%For ease of computation, kernalized methods often optimize $\bm{\alpha}$ with size $n$ instead of (infinite) $M$-dim $\mathbf{w}^\prime$. Therefore, by substituting $\mathbf{w}^\prime$ with $\Phi(\mathbf{X})^T \bm{\alpha}$, Eqn~\ref{kernel_ridge_primal} becomes 
The objective function of KRR is 
\begin{small}
\begin{align}
\label{kernel_ridge_dual}
\begin{split}
%\mathcal{L}_{KRR}(\lambda, \bm{\alpha}) 
\mathcal{L}(\bm{\alpha})
%& = \| \mathbf{y}-\Phi(\mathbf{X}) \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 + \lambda \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
& = \| \mathbf{y} - \mathbf{K} \bm{\alpha} \|_2^2 + \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha},
\end{split}
\end{align}
\end{small}
where $\mathbf{K}=\Phi(\mathbf{X})^T \Phi(\mathbf{X})=\{ \langle \phi(\mathbf{x}_i), \phi(\mathbf{x}_j) \rangle_{i,j} \}$ is an $n \times n$ Gram matrix. 
%inner product matrix, also called \textbf{Gram matrix}, defined in the feature space.
It uses least square loss function and $L_2$ regularization. In general, the optimal $\bm{\alpha}$ is analytically solved via SVD~\cite{weisstein2002singular}.


Then, taking the derivative of $\mathcal{L}_{KRR}$ with respect to $\bm{\alpha}$ and setting it to be \textbf{0}, we have
\begin{small}
\begin{align*}
\mathbf{K}(\lambda \bm{\alpha} + \mathbf{K} \bm{\alpha} - \mathbf{y}) = \mathbf{0}.
\end{align*}
\end{small} 
As $\mathbf{K}$ is positive definite and thus invertible, we multiply both sides with $\mathbf{K}^{-1}$. Then,
$\mathbf{a} = \bm{\alpha}$ and $\mathbf{b} = \mathbf{K} \bm{\alpha} - \mathbf{y}$. 
%and estimate $\lambda$ as
%for each $\alpha_j$ as
% \begin{small}
% \begin{align}
% \hat{\lambda} = \frac{1}{n} \sum_{i=1}^n \frac{y_i - \mathbf{k}^{i} \alpha_i}{\alpha_i}. 
% \end{align}
% \end{small}

%\vspace{-5mm}
%As the kernel version of LASSO and Elastic Net is seldom used in real-world problems, we thus do not provide the analysis. 
 
% \subsubsection{Kernel Support Vector Regression}

% The problem with kernel ridge regression is that the $\mathbf{w}^\prime$ depends on all the training samples. We now seek a method to produce a sparse estimate of $\mathbf{w}^\prime$.

% Leveraging the similar idea as kernel ridge regression, we rewrite primal parameters $\mathbf{w}^{\prime}$ using its dual $\bm{\alpha}$ and have 
% \begin{align}
% \label{kernel_svr}
% \begin{split}
% \mathcal{L}_{KernelSVR}(T, \bm{\alpha}) & = T \sum_{j=1}^n L_{\epsilon}(y_j, \langle \Phi(\mathbf{X})^T \bm{\alpha}, \phi(\mathbf{x}_i) \rangle) + \frac{1}{2} \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
% & = T \sum_{j=1}^n L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha}, 
% \end{split}
% \end{align}
% where 
% \begin{align}
% L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = 
% \begin{cases}
% 0 & \text{if } |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle| \leq \epsilon \\
% |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle | - \epsilon  & \text{if } |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle| > \epsilon
% \end{cases}
% \end{align}
% and $\mathbf{k}_j = \Phi(\mathbf{X}) \phi(\mathbf{x}_i)$.

% Note again that the objective function is convex but not differentiable at the points $y_j = \langle \bm{\alpha}, \mathbf{k}_j \rangle \pm \epsilon$. Then, the subgradient of $L_{\epsilon}$ with respect to $\bm{\alpha}$ is 
% \begin{align}
% \frac{\partial L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle)}{\partial \bm{\alpha}} = 
% \begin{cases}
% - \mathbf{k}_j & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j - \epsilon \\
% \left[ -\mathbf{k}_j, \mathbf{0} \right] & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle = y_j - \epsilon \\
% \mathbf{0} & \text{if } y_j - \epsilon < \langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j + \epsilon \\
% \left[ \mathbf{0}, \mathbf{k}_j \right] & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle = y_j + \epsilon \\
% \mathbf{k}_j & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle > y_j + \epsilon
% \end{cases}
% \end{align}

% Finally, we set the subgradient of non-differential points as 0 and the derivative of $\mathcal{L}_{KernelSVR}$ with respect to $\bm{\alpha}$ to zero. With it, $T$ is estimated as  
% \begin{align}
% \hat{T}^{(i)} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,\langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j - \epsilon} k_{j,i} - \sum\limits_{j,\langle \bm{\alpha}, \mathbf{k}_j \rangle > y_j + \epsilon} k_{j,i} }
% \end{align}

\subsection{Attack on Convex-Induced Classification Models}
\label{attack_cvx_clf}

%We consider attacks on both convex linear and kernel-based nonlinear classification models.
We consider attacks on both convex linear and kernel classification models.

\subsubsection{Linear Classification Models}
\label{cvx_clf_lin}

In this part, we focus on stealing the hyperparameter of two well-known linear classification models, i.e., LR~\cite{hosmer2013applied} and linear SVC (LSVC)~\cite{cortes1995support}. 
For LR, we consider its both binary and multi-class classification, and denote them as binary LR (BLR) and multi-class LR (MLR), respectively.  In addition, we consider $L_2$ and $L_1$ regularizations.
For LSVC, we consider its two different loss functions, i.e., Regular Hinge Loss (RHL) and Square Hinge Loss (SHL).
%For LR, we consider both its binary case and multi-class case, and denote them as binary LR (BLR) and multi-class LR (MLR), respectively. 
Due to space limitation, we only show hyperparameter stealing of $L_2$-regularized BLR (L2-BLR). The results of other models are listed in Table~\ref{sum_ml} and their derivation are provided in Appendix~\ref{app:cvx_clf}.

%\myparatight{$L_2$-regularized Binary LR (L2-BLR)} 
%The objective function of L2-BLR is 
% Taking a single sample $\{\mathbf{x},y\}$ for example, BLR aims at maximizing the following conditional probability with $y \in \{0,1\}$,
% %binary classification model with label $y \in {0,1}$: 
% \begin{small}
% \begin{align}
% \label{lr_eqn}
% Pr(y|\mathbf{x}, \mathbf{w}) = \text{Ber}(y|h_\mathbf{w}(\mathbf{x})) = h_\mathbf{w}(\mathbf{x})^y (1-h_\mathbf{w}(\mathbf{x}))^{1-y},
% %Pr(y|\mathbf{x}, \mathbf{w}) = \text{Ber}(y|\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) = \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)^y (1-\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle))^{1-y},
% \end{align}
% \end{small}
% where \textbf{Ber} is bernoulli distribution with $\text{Ber}(k|p)=p$ if $k=1$, and $\text{Ber}(k|p)=1-p$ if $k=0$; $h_\mathbf{w}(\mathbf{x})=\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) $, where \textbf{sigm} refers to the sigmoid (logistic, or logit) function, defined as $\text{sigm}(z)=\frac{1}{1+\exp{(-z)}}$.

% In practice, the maximization of Eqn~\ref{lr_eqn} is often transformed to the minimization of nonnegative log-likelihood (NLL), which is given by
% \begin{small}
% \begin{align}
% \label{lr_nll}
% \begin{split}
% & \text{NLL}_{BLR}(\mathbf{w};\mathbf{x},y) = - \log Pr(y|\mathbf{x}, \mathbf{w}) \\
% & \qquad = - \big( y \, \log h_\mathbf{w}(\mathbf{x}) + (1-y) \log (1- h_\mathbf{w}(\mathbf{x})) \big). 
% %\text{NLL}(\mathbf{w};\mathbf{x},y) = - \log Pr(y|\mathbf{x}, \mathbf{w}) = - \big( y \, \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) + (1-y) (1- \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) \big). 
% \end{split}
% \end{align}
% \end{small}
% This is also called \textbf{cross entropy} error function. 

% To tackle real-world problems, BLR is often added an $L_2$ or $L_1$ regularization. Here, we simply take $L_2$-regularized BLR (L2-BLR) as an example. 
%Its objective function is 
%\paragraph{$L_2$-regularized BLR (L2-BLR)} Its objective function  is
\myparatight{$L_2$-regularized Binary LR (L2-BLR)} The objective function of L2-BLR is 
\begin{small}
\begin{align}
\label{l2lr}
\mathcal{L}(\mathbf{w}) = \sum_{i=1}^n \text{NLL}(\mathbf{w};\mathbf{x}_i,y_i) + \lambda \| \mathbf{w} \|_2^2,
\end{align}
\end{small}
where $\text{NLL}(\mathbf{w};\mathbf{x},y) = - \big( y \, \log h_\mathbf{w}(\mathbf{x}) + (1-y) \log (1- h_\mathbf{w}(\mathbf{x})) \big)$ is called \textbf{cross entropy} loss function and $h_\mathbf{w}(\mathbf{x}) = \frac{1}{1+\exp{(-\langle \mathbf{w}, \mathbf{x} \rangle)}} $. Generally, coordinate descent algorithm~\cite{friedman2010regularization} is leveraged to approximately solve for $\mathbf{w}$.  
%\mathcal{L}_{L2-BLR}(
% \lambda, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}_i) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}_i)) \right] + 
% \lambda \| \mathbf{w} \|_2^2,
% \end{align}
% \end{small}
%where $h_\mathbf{w}(\mathbf{x}_i) = \text{sigm}(\mathbf{w}^T \mathbf{x}^j) = \frac{1}{1+\exp(-\mathbf{w}^T \mathbf{x}^j)}$.

The derivative of $\mathcal{L}(\mathbf{w})$ with respect to $\mathbf{w}$ is given by
\begin{small}
\begin{align*}
%\label{l2lr_grad}
\begin{split}
& \frac{\partial \mathcal{L}(\mathbf{w})}{\partial \mathbf{w}} = - \sum_{i=1}^n \left[ \frac{y_i}{h_\mathbf{w}(\mathbf{x}_i)} \frac{\partial h_\mathbf{w}(\mathbf{x}_i)}{\partial \mathbf{w}} + \frac{-(1-y_i)}{1-h_\mathbf{w}(\mathbf{x}_i)} \frac{\partial h_\mathbf{w}(\mathbf{x}_i)}{\partial \mathbf{w}}\right] + 2 \lambda \mathbf{w} \\
%& \quad = - \sum_{j=1}^n \left[ \frac{y_j }{h_\mathbf{w}(\mathbf{x}_i)} h_\mathbf{w}(\mathbf{x}_i) (1-h_\mathbf{w}(\mathbf{x}_i)) - \frac{(1-y_j)}{1-h_\mathbf{w}(\mathbf{x}_i)} h_\mathbf{w}(\mathbf{x}_i) (1-h_\mathbf{w}(\mathbf{x}_i)) \right] \frac{\partial \mathbf{w}^T \mathbf{x}^j}{\partial \mathbf{w}} + 2 \lambda \mathbf{w} \\
%& \quad = - \sum_{i=1}^n \left(y_i (1-h_\mathbf{w}(\mathbf{x}_i)) - (1-y_i) h_\mathbf{w}(\mathbf{x}_i) \right) \mathbf{x}_i + 2 \lambda \mathbf{w} \\ 
& \quad = \sum_{i=1}^n (h_\mathbf{w}(\mathbf{x}_i) - y_i) \mathbf{x}_i + 2 \lambda \mathbf{w} = \mathbf{X} (h_\mathbf{w}(\mathbf{X}) - \mathbf{y}) + 2 \lambda \mathbf{w},
\end{split}
\end{align*}
\end{small}
where $\frac{\partial h_\mathbf{w}(\mathbf{x}_i)}{\partial \mathbf{w}} = h_\mathbf{w}(\mathbf{x}_i) (1-h_\mathbf{w}(\mathbf{x}_i))$ in the first equation and $h_\mathbf{w}(\mathbf{X}) = \left[ h_\mathbf{w}(\mathbf{x}_1); h_\mathbf{w}(\mathbf{x}_2); \cdots, h_\mathbf{w}(\mathbf{x}_n) \right]$. 

Setting it to be \textbf{0}, and comparing it with Eqn.~\ref{norm_eqn}, we have
$\mathbf{a} = 2 \mathbf{w}$ and $\mathbf{b} = \mathbf{X} (h_\mathbf{w}(\mathbf{X}) - \mathbf{y})$.

%we can estimate $\lambda$ for as
%\begin{small}
%\begin{align}
%\label{l2lr_soln}
%\hat{\lambda} = - \frac{1}{n} \sum_{i=1}^n \frac{\langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle}{2 w_i}.
%\end{align}
%\end{small}

%where $h_\mathbf{w}(\mathbf{X}) = \left[ h_\mathbf{w}(\mathbf{x}^1_T), h_\mathbf{w}(\mathbf{x}^2_T), \cdots, h_\mathbf{w}(\mathbf{x}^n_T) \right]^T \in \mathbb{R}^n$. %(See Appendix~\ref{app:l2blr}).

%Unlike aforementioned linear model, we cannot write down the closed form for each $w_i$. 

% \paragraph{$L_1$-regularized BLR (L1-BLR)} Its objective function is 
% \begin{align}
% \label{l1lr}
% \mathcal{L}_{L1-BLR}(\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};\mathbf{x}_i,y_j) + \lambda \| \mathbf{w} \|_1.
% %\mathcal{L}_{L1-BLR}(\lambda, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}_i) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}_i)) \right] + \lambda \| \mathbf{w} \|_1.
% \end{align}

% Taking the subgradient of $\mathcal{L}_{L1-BLR}$ with respect to $w$ and setting it to 0, we can estimate $\lambda$ for each $w_i$ as
% \begin{align}
% \label{l1lr_soln}
% \hat{\lambda}^{(i)}_{L1-BLR} = 
% \begin{cases}
% - \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i > 0 \\
%  \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i < 0
% \end{cases}
% \end{align}

% \myparatight{Multi-Class Logistic Regression (MLR)} Now we consider MLR, also known as multinomial logistic regression, softmax regression, and maximum entropy classifier. Given a single sample $\{\mathbf{x},y\}$, the model is defined as
% \begin{align}
% \label{mlr}
% Pr(y=c|\mathbf{x},\mathbf{W}) = \frac{\exp{\langle \mathbf{w}_c, \mathbf{x} \rangle}}{\sum_{c^\prime=1}^C \exp{\langle \mathbf{w}_{c^\prime}, \mathbf{x} \rangle}},
% \end{align}
% where $\mathbf{W}=\left[ \mathbf{w}_1, \cdots, \mathbf{w}_C \right]$, with $c$-th column the coefficients for representing $c$-th class.

% To deal with $C$ classes, we introduce some new notation. Let $y_{j,c} = 1(y_j=c)$ be the one-of-$C$ encoding of $y_j$; thus $\mathbf{y}^j$ is a bit vector, in which $c$-th entry $y_{j,c}=1$ when $y_j=c$. We further denote $\mathbf{Y} = \left[ \mathbf{y}^1; \mathbf{y}^2; \cdots ; \mathbf{y}^n \right] = \left[ \mathbf{y}_1, \mathbf{y}_2, \cdots, \mathbf{y}_C \right] \in \mathbb{R}^{n \times C} $ be the label matrix. Then, the NLL for sample $\mathbf{x}^j$ is written as
% \begin{align*}
% \small
% %\label{mlr_nll}
% \begin{split}
% \text{NLL}_{MLR}(\mathbf{W}; \mathbf{x}_i, \mathbf{y}^j) = - \sum_{c=1}^C y_{j,c} \langle \mathbf{w}_c, \mathbf{x}_i \rangle + \log \big( \sum_{c^\prime=1}^C \exp (\langle \mathbf{w}_{c^\prime}, \mathbf{x}_i ) \big).
% \end{split}
% \end{align*} 

% In practice, MLR is added an $l_2$ regularization, termed $L_2$-regularized MLR (L2-MLR). Its objective function is 
% \begin{align}
% \small
% \label{l2mlr}
% \mathcal{L}_{L_2-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}_i, \mathbf{y}^j) + \lambda \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
% %\mathcal{L}_{L_2-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j, \mathbf{y}_j) + \lambda \sum_
% %{c=1}^C \| \mathbf{w}_c \|_2^2.
% \end{align}

% By setting the derivative of $\mathcal{L}_{L_2-MLR}$ with respect to $c$-th class $\mathbf{w}_c$ to be zero. Then, for each class $c$ and each $\mathbf{x}_i$, we can estimate $\lambda$ as 
% \begin{align}
% \label{l2mlr_soln_2}
% \hat{\lambda}^{(i,c)}_{L_2-MLR} = - \frac{\langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle }{2 w_{i,c}},
% \end{align}
% where $\bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) = \left[ Pr(y_{1,c}=1|\mathbf{x}^1_T, \mathbf{W}), \cdots, Pr(y_{n,c}=1| \mathbf{x}^n_T, \mathbf{W}) \right]^T $  
% and $\mathbf{y}_c = \left[ y_{1,c}, y_{2,c}, \cdots , y_{n,c} \right]^T$. 

% \paragraph{$L_1$-regularized MLR}

% \begin{align}
% \label{l1mlr}
% \mathcal{L}_{L_1-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j,\mathbf{y}^j) + \lambda \| \mathbf{W} \|_1.
% %\mathcal{L}_{L_1-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j,\mathbf{y}_j) + \lambda \sum_{c=1} \| \mathbf{w}_c \|_1.
% \end{align}

% Similarly with $L_2$-regularized MLR, the gradient of $\mathcal{L}_{L_1-MLR}$ with respect to $\mathbf{w}_c$ is given by
% \begin{align}
% \label{l1mlr_soln_1}
% \frac{\partial \mathcal{L}_{L_1-MLR}}{\partial \mathbf{w}_c} = \mathbf{X}^T (\bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c) + \lambda \, \partial_{\mathbf{w}_c} \| \mathbf{w}_c \|_1. 
% \end{align}

% Setting $\partial_{\mathbf{w}_c} \mathcal{L}_{L_1-MLR}=0$ and considering the non-differentiability of $\| \mathbf{w}_c \|_1$, we estimate $\lambda$ for each feature $\mathbf{x}_i$ and nonzero $w_{i,c}$ as 
% \begin{align}
% \label{l1mlr_soln_2}
% \hat{\lambda}^{(i,c)}_8 = 
% \begin{cases}
% - \langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle & \text{if } w_{i,c} > 0 \\
%  \langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle & \text{if } w_{i,c} < 0 \\
% \end{cases}
% \end{align}

% \myparatight{Binary Linear Support Vector Classification (BLSVC)}
% The objective function of BLSVC is defined as
% \begin{align}
% \label{hl_bsvc}
% \mathcal{L}_{BLSVC}(T, \mathbf{w}) = T \sum_{j=1}^n L_{HL}(y_j, \langle \mathbf{w}, \mathbf{x}_i \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2, 
% \end{align}
% where $L_{HL}(y_j, \langle \mathbf{w}, \mathbf{x}_i \rangle)$ is the \textbf{hinge loss} for predicting $\mathbf{x}_i$. 

% There are two common hinge loss functions, i.e., regular hinge loss (RHL) and squared hinge loss (SHL). In correspondence, we denote BLSVC as BLSVC-RHL and BLSVC-SHL, respectively.

% \paragraph{Regular hinge loss (RHL)}
% $L_{RHL}(y_j, \langle \mathbf{w}, \mathbf{x}_i \rangle) = \max(0, 1 - y_j \langle \mathbf{w}, \mathbf{x}_i \rangle)$. 
% %Figure~\ref{XX} shows its function as well as squared hinge loss. 
% Note that RHL is convex, but non-differential when $y_j \langle \mathbf{w}, \mathbf{x}_i \rangle = 1$. Its subgradient with respect to $\mathbf{w}$ is 
% % Once again, it is non-differential because of the \textbf{max} term. However, by introducing slack parameters $\xi_i$, one can show that it is equivalent to solving
% % \begin{align}
% % \begin{split}
% % & \mathcal{L}_{HL-SVM}(T, \mathbf{w}, \bm{\xi}) = T \sum_{j=1}^n \xi_j + \frac{1}{2} \| \mathbf{w} \|^2 \\
% % & \text{s.t. } y_j \langle \mathbf{w}, \mathbf{x}_i \rangle \geq 1 - \xi_i, \xi_i \geq 0, \forall i. 
% % \end{split}
% % \end{align}
% %because of the ``max term". Its subgradient with respect to $\mathbf{w}$ is 
% \begin{align}
% \label{RHL_subg}
% \frac{\partial L_{RHL}}{\partial \mathbf{w}} = 
% \begin{cases}
% -y_j \mathbf{x}_i & \text{if } y_j \langle \mathbf{w}, \mathbf{x}_i \rangle < 1 \\
% [-y_j \mathbf{x}_i, \mathbf{0}] & \text{if } y_j \langle \mathbf{w}, \mathbf{x}_i \rangle = 1 \\
% \mathbf{0} & \text{if } y_j \langle \mathbf{w}, \mathbf{x}_i \rangle > 1
% \end{cases}
% \end{align}

% For non-differential point, its subgradient is set to be 0. Therefore, with Eqn~\ref{RHL_subg}, we can estimate the hyperparamter $T$ using only samples $\mathbf{x}^j$ that satisfy $y_j \langle \mathbf{w}, \mathbf{x}_i \rangle < 1$. Setting the derivative of $\mathcal{L}_{BLSVC}$ with respect to $w_i$ to zero yields
% \begin{align}
% \hat{T}^{(i)}_{BLSVC-RHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, \mathbf{x}_i \rangle < 1} y_j {x}_{j,i}}. 
% %T \sum_{j,y_j \langle \mathbf{w}, \mathbf{x}_i \rangle < 1} -y_j \mathbf{x}^j + \mathbf{w} = 0, \quad \text{if } y_j \langle \mathbf{w}, \mathbf{x}_i \rangle < 1.
% %T \sum_{j=1}^n -y_j \mathbf{x}^j + \mathbf{w} = 0, \quad \text{if } y_j \langle \mathbf{w}, \mathbf{x}_i \rangle < 1.
% \end{align} 

% \paragraph{Squared Hinge Loss (SHL)} 
% $L_{SHL}(y_j, \langle \mathbf{w}, \mathbf{x}_i \rangle) = \max(0, 1 - y_j \langle \mathbf{w}, \mathbf{x}_i \rangle)^2$. SHL is convex, smooth, and differential. Its subgradient with respect to $\mathbf{w}$ is given by
% \begin{align}  
% \label{SHL_subg}
% \frac{\partial L_{SHL}}{\partial \mathbf{w}} =
% \begin{cases}
% -2 y_j \mathbf{x}_i (1 - y_j \langle \mathbf{w}, \mathbf{x}_i \rangle) & \text{if } y_j \langle \mathbf{w}, \mathbf{x}_i \rangle <= 1 \\
% \mathbf{0}  & \text{if } y_j \langle \mathbf{w}, \mathbf{x}_i \rangle > 1
% \end{cases}
% \end{align}

% Therefore, taking the derivative of $\mathcal{L}_{BLSVC}$ with respect to $w_i$ to zero in this case  yields
% \begin{align}
% \hat{T}^{(i)}_{BLSVC-SHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, \mathbf{x}_i \rangle \leq 1} 2y_j {x}_{j,i} (1 - y_j \langle \mathbf{w}, \mathbf{x}_i \rangle) }. 
% \end{align}

% For multi-class LSVC, it can be derivated from binary LSVC in a one-vs-one (or one-vs-rest) fashion~\cite{chang2011libsvm}. In this setting, we can run binary classification Eqn~\ref{hl_bsvc} $K \times (K-1)/2 $ (or $K$) times to estimate the hyperparater.

% \subsubsection{Multi-Class LSVC}

% Normally, binary LSVC is extended to multi-class linear SVC in a one-vs-one or one-vs-rest fashion [2]. In this setting, we can run binary classification Eqn~\ref{hl_bsvc} $K \times (K-1)/2 $ and $K$ times to estimate the hyperparater. However, there exists a ``true" multi-class version hinge loss (MHL) for multi-class SVC, due to Crammer and Singer [3], which optimizes a joint objective over all classes and is defined as
% \begin{align}
% \label{crammer_singer_msvc}
% \begin{split}
% & \min_{\mathbf{W},\epsilon} \quad \mathcal{L}_{MSVC}(T, \mathbf{W}) =  T \sum_{j=1}^n \epsilon_j + \frac{1}{2} \sum_{c=1}^T \| \mathbf{w}_c \|_2^2 \\
% & \text{s.t.} \quad	\langle \mathbf{w}_{y_j}, \mathbf{x}_i  \rangle - \langle \mathbf{w}_c, \mathbf{x}_i  \rangle  \geq e_j^c - \epsilon_j \\
% & \quad \quad \epsilon_j \geq 0, \, j=1,\cdots, n; \, c=1, \cdots, T, 
% \end{split}
% \end{align}
% where $e_j^c = 0$ if $y_j = c$, and $e_j^c = 1$ if $y_j \neq c$ and $\mathbf{W} = \left[ \mathbf{w}_1, \mathbf{w}_2, \cdots, \mathbf{w}_C \right]$. 

% The decision function to predict the label of a new instance $\mathbf{x}$ is $\argmax\nolimits_{c=1,\cdots,C} \langle \mathbf{w}_c, \mathbf{x} \rangle $.

% Directly setting the derivative of $\mathcal{L}_{MSVC}$ for $\mathbf{w}_c$ via Eqn~\ref{crammer_singer_msvc} in a constrainted form is difficult. Therefore, we transform it to the equivalent unconstrained form as follows
% % \begin{align}
% % \mathcal{L}_{MSVC}(T, \mathbf{W}) = T \sum_{j=1}^n \sum_{c \neq y_j} L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2,
% % \end{align}
% \begin{align}
% \mathcal{L}_{MSVC}(T, \mathbf{W}) = T \sum_{j=1}^n L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}_i \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2,
% \end{align}
% where $L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}_i \rangle) = \max(0, 1 + \max\nolimits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}_i \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}_i \rangle)$ is the maximal hinge loss among $C$ classes for predicting $\mathbf{x}^j$. 

% % Similarly, there are also two MHL functions, i.e., regular MHL and squared MHL. 

% % \textbf{Regular multi-class hinge loss (RMHL):} $L_{RMHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j \rangle) = \max(0, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}_j \rangle)$. 

% %Therefore, the objective function in this setting becomes
% In this way, the objective function then becomes
% \begin{align}
% \mathcal{L}_{MSVC}(T, \mathbf{w}) = T \sum_{j=1}^n \max(0, 1 + \max_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}_i \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}_i \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
% \end{align}

% Its subgradient with respect to $\mathbf{w}_c$ is 
% \begin{align}
% \frac{\partial MSVC}{\partial \mathbf{w}_c} =
% \begin{cases}
% T \sum\limits_{j=1}^n \mathbf{x}_i + \mathbf{w}_c & \text{if } 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}_i \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}_i \rangle > 0 \\
% \mathbf{0} & \text{if } 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}_i \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}_i \rangle < 0
% \end{cases}
% \end{align}

% % \begin{align}
% % \mathcal{L}_{MSVC}(T, \mathbf{w}) = T \sum_{j=1}^n \sum_{c \neq y_j} \max(0, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
% % \end{align}

% % Its subgradient with respect to $\mathbf{w}_c$ is 
% % \begin{align}
% % \frac{\partial MSVC}{\partial \mathbf{w}_c} =
% % \begin{cases}
% % T \sum_{j=1}^n \mathbf{x}^j + \mathbf{w}_c & \text{if } 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle > 0 \\
% % \mathbf{0} & \text{if } 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle < 0
% % \end{cases}
% % \end{align}

% Setting it to zero, we have 
% % \begin{align}
% % \hat{T}^{(i,c)} = - \frac{w_{i,c}}{\sum\limits_{j, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle > 0} x_{j,i}}. 
% % \end{align}
% \begin{align}
% \hat{T}^{(i,c)} = - \frac{w_{i,c}}{\sum\limits_{j, 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}_i \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}_i \rangle > 0} x_{j,i}}. 
% \end{align}

\subsubsection{Kernel Classification Models}
\label{cvx_clf_nonlin}

We kernelize linear classification methods to generate corresponding kernel models. We only take $L_2$-regularized Kernel Binary LR(L2-KBLR) as example.

%\myparatight{$L_2$-regularized Kernel Binary  LR (L2-KBLR)~\cite{zhu2001kernel}} 
%Its objective function is 

% Given a single sample $\{\mathbf{x},y\}$, BKLR is to minimize the following NLL
% \begin{small}
% \begin{align*}
% %\label{klr_nll}
% \begin{split}
% & \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}),y) = - \log Pr(y|\phi(\mathbf{x}), \mathbf{w}^\prime) \\
% & \qquad = - \big( y \, \log h_{\mathbf{w}^\prime}(\phi(\mathbf{x})) + (1-y) \log (1- h_{\mathbf{w}^\prime}(\phi(\mathbf{x}))) \big)
% %\text{NLL}(\mathbf{w};\mathbf{x},y) = - \log Pr(y|\mathbf{x}, \mathbf{w}) = - \big( y \, \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) + (1-y) (1- \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) \big). 
% \end{split}
% \end{align*}
% \end{small}
% %where $h_{\mathbf{w}^\prime}(\phi(\mathbf{x}))) = \frac{1}{1+\exp(\langle \bm{\alpha}, \rangle)}$ 

% Again, using dual representer theorem, we have %its dual form 
% \begin{small}
% \begin{align*}
% \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) = - \big( y_j \, \log h_{\bm{\alpha}}(\mathbf{k}_j) + (1 - y_j) (1- h_{\bm{\alpha}}(\mathbf{k}_j)) \big),
% \end{align*}
% \end{small}
% where $h_{\bm{\alpha}}(\mathbf{k}_j) = \frac{1}{1 + \exp{\langle \bm{\alpha}, \mathbf{k}_j \rangle}}$.

% By adding an $L_2$ regularization, 

\myparatight{$L_2$-regularized Kernel Binary  LR (L2-KBLR)~\cite{zhu2001kernel}} 
The objective function of L2-KBLR is
\begin{small}
\begin{align}
\label{l2klr_dual}
\begin{split}
\mathcal{L}(\bm{\alpha}) = \sum_{j=1}^n \text{NLL}(\bm{\alpha}; \mathbf{k}_j,y_j) + 
\lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha},
\end{split}
\end{align} 
\end{small}
where $\text{NLL}(\bm{\alpha}; \mathbf{k}_j,y_j) = - \big( y_j \, \log h_{\bm{\alpha}}(\mathbf{k}_j) + (1 - y_j) (1- h_{\bm{\alpha}}(\mathbf{k}_j)) \big)$ is the cross entropy loss function defined in kernel space and $h_{\bm{\alpha}}(\mathbf{k}_j) = \frac{1}{1 + \exp{(- \langle \bm{\alpha}, \mathbf{k}_j \rangle)}}$. $\bm{\alpha}$ is often solved approximately via coordinate descent.  

% % By adding an $L_2$ regularization, the objective function of L2-BKLR with primal parameters is  
% % % Minimize the following 
% % \begin{align*}
% % %\label{l2klr_primal}
% % \mathcal{L}_{L2-BKLR}(\lambda, \mathbf{w}^\prime) = \sum_{j=1}^n \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}_i),y_j) + 
% \lambda \| \mathbf{w}^\prime \|_2^2.
% % %\mathcal{L}_{L2-BLR}(
% \lambda, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(
% \mathbf{x}_i) + (1-y_j) \log(1-h_\mathbf{w}(
% \mathbf{x}_i)) \right] + 
% \lambda \| \mathbf{w} \|_2^2,
% % \end{align*}
% % %where $h_\mathbf{w}(
% \mathbf{x}_i) = \text{sigm}(\mathbf{w}^T \mathbf{x}^j) = \frac{1}{1+\exp(-\mathbf{w}^T \mathbf{x}^j)}$.

% % Again, using dual representation $\mathbf{w}^\prime = \Phi(\mathbf{X})^T \bm{\alpha}$, we have its dual form
% % \begin{align}
% % \small
% % \label{l2klr_dual}
% % \begin{split}
% % & \mathcal{L}_{L2-BKLR}(
% \lambda, \bm{\alpha}) = \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + 
% \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha} \\
% % & = \sum_{j=1}^n - \big( y_j \, \log h_{\bm{\alpha}}(\mathbf{k}_j) + (1 - y_j) (1- h_{\bm{\alpha}}(\mathbf{k}_j)) \big) + 
% \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha},
% % \end{split}
% \end{align} 
% where $h_{\bm{\alpha}}(\mathbf{k}_j) = \frac{1}{1 + \exp{\langle \bm{\alpha}, \mathbf{k}_j \rangle}}$.

%The derivative of $\mathcal{L}_{L2-BKLR}$ with respect to $\bm{\alpha}$ is given by
Its derivative with respect to $\bm{\alpha}$ is given by
\begin{small}
\begin{align*}
%\label{l2klr_soln_1}
\begin{split}
\frac{\partial \mathcal{L}(\bm{\alpha})}{\partial \bm{\alpha}} 
%& = \sum_{j=1}^n (h_{\bm{\alpha}}(\mathbf{k}_j) - y_j) \mathbf{k}_j + 2 \lambda \mathbf{K} \bm{\alpha} \\
& = \mathbf{K} (h_{\bm{\alpha}}(\mathbf{K}) - \mathbf{y} + 2 \lambda \bm{\alpha}),
\end{split}
\end{align*}
\end{small}
where $h_{\bm{\alpha}}(\mathbf{K}) = \left[ h_{\bm{\alpha}}(\mathbf{k}_1), \cdots, h_{\bm{\alpha}}(\mathbf{k}_n) \right]^T $.
% and $\mathbf{K}^T = \mathbf{K}$.

Setting it to be \textbf{0} and considering that $\mathbf{K}$ is invertible, we have 
$\mathbf{a} = 2 \bm{\alpha}$ and $\mathbf{b} = (h_{\bm{\alpha}}(\mathbf{K}) - \mathbf{y}$.

% for each $\alpha_i$, we estimate $
% \lambda$ as
% \begin{small} 
% \begin{align}
% \label{l2klr_soln}
% \hat{
% \lambda}^{(j)}_{L2-BKLR} = - \frac{h_{\bm{\alpha}}(\mathbf{k}_j) - y_j} {2 \alpha_j}.
% \end{align}
% \end{small}

%\vspace{-5mm}
% \paragraph{$L_1$-regularized BKLR (L1-BKLR)} Its objective function of primal parameters is 
% \begin{align*}
% %\label{l1klr_primal}
% \mathcal{L}_{L1-BKLR}(\lambda, \mathbf{w}^\prime) = \sum_{j=1}^n \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}_i),y_j) + \lambda \| \mathbf{w}^\prime \|_1.
% %\mathcal{L}_{L2-BLR}(\lambda, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}_i) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}_i)) \right] + \lambda \| \mathbf{w} \|_2^2,
% \end{align*}

% Using $\mathbf{w}^\prime = \Phi(\mathbf{X})^T \bm{\alpha}$, we have its dual form
% \begin{align}
% \small
% \begin{split}
% \label{l1klr_dual}
% \mathcal{L}_{L1-BKLR}(\lambda, \bm{\alpha}) & = - \sum_{j=1}^n \big( y_j \, \log h_{\bm{\alpha}}(\mathbf{k}_j) + (1 - y_j) (1- h_{\bm{\alpha}}(\mathbf{k}_j)) \big) \\ 
% & + \lambda \| \mathbf{K} \bm{\alpha} \|_1. 
% \end{split}
% \end{align} 

% By setting the subgradient of $\mathcal{L}_{L1-BKLR}$ with respect to $\bm{\alpha}$ to be zero, we estimate $\lambda$ as 
% \begin{align}
% \label{llklr_soln}
% \hat{\lambda}^{(j)}_{L1-BKLR} = 
% \begin{cases}
%  y_j - h_{\bm{\alpha}}(\mathbf{k}_j)  & \text{if } \mathbf{k}^j \bm{\alpha} > 0 \\
%  h_{\bm{\alpha}}(\mathbf{k}_j) - y_j  & \text{if } \mathbf{k}^j \bm{\alpha} < 0
% \end{cases}
% \end{align} 

% \myparatight{Multi-Class Kernel Logistic Regression (MKLR)}
% Similarly with MLR, MKLR also uses one-of-$C$ code to represent each label $\mathbf{y}$ and dual representation, the NLL of MKLR for $C$-class and $N$ samples is defined as 
% \begin{align*}
% \begin{split}
% & \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) = - \sum_{j=1}^N \sum_{c=1}^C y_{j,c} \log Pr(y_{j,c}=1 | \mathbf{k}_j, \bm{\Omega}) \\ 
% & \qquad = - \sum_{j=1}^N \bigg( \sum_{c=1}^C y_{j,c} \langle \bm{\alpha}_c, \mathbf{k}_j \rangle + \log \big( \sum_{c^\prime=1}^C \exp (\langle \bm{\alpha}_{c^\prime}, \mathbf{k}_j \rangle) \big) \bigg), 
% \end{split}
% \end{align*}
% where $\bm{\Omega} = \left[ \bm{\alpha}_1, \bm{\alpha}_2, \cdots, \bm{\alpha}_C \right]$.

% In practice, MKLR often adds an $l_2$ regularization, termed L2-regularized MKLR (L2-MKLR). Similarly with L2-MLR, its objective function of dual parameters is
% \begin{align}
% \mathcal{L}_{L_2-MKLR}(\lambda, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + \lambda \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c.  
% \end{align}
% and its gradient of $\bm{\alpha}_c$ is given by
% \begin{align}
% \frac{\partial \mathcal{L}_{L_2-MKLR}}{\partial \bm{\alpha}_c} = \mathbf{K} (\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) - \mathbf{y}_c + 2 \lambda \bm{\alpha}_c),
% \end{align}
% where $\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) = \left[ Pr(y_{1,c}=1 | \mathbf{k}_1, \bm{\Omega}), \cdots, Pr(y_{1,c}=n | \mathbf{k}_n, \bm{\Omega}) \right]$.
% % where $\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) = \left[ Pr(y_{1,c}=1 | \mathbf{k}_1, \bm{\Omega}), Pr(y_{2,c}=1 | \mathbf{k}_2, \bm{\Omega}), \cdots, Pr(y_{1,c}=n | \mathbf{k}_n, \bm{\Omega}) \right]$.

% By setting it to \textbf{0}, for each class $c$, we can estimate $\lambda$ as
% \begin{align}
% \hat{\lambda}^{(j,c)}_{L_2-MKLR} = \frac{y_{j,c} - \bm{\mu}_{c, \bm{\Omega}}(\mathbf{k}_j)}{2 \alpha_{j,c}}.
% \end{align}

% \myparatight{Binary Kernel Support Vector Classification (BKSVC)}
% The objective function of BKSVC in the primal form is defined as
% \begin{align*}
% \small
% %\label{kernel_bsvc_prime}
% \mathcal{L}_{BKSVC}(T, \mathbf{w^\prime})  = T \sum_{j=1}^n L_{HL}(y_j, \langle \mathbf{w^\prime}, \phi(\mathbf{x}_i) \rangle) + \frac{1}{2} \| \mathbf{w^\prime} \|_2^2. 
% \end{align*}

% Using dual representation $\mathbf{w}^\prime = \Phi(\mathbf{X})^T \bm{\alpha}$, we have its dual form
% \begin{align}
% \small
% \label{kernel_bsvc_dual}
% \begin{split}
% \mathcal{L}_{BKSVC}(T, \bm{\alpha}) & = T \sum_{j=1}^n L_{HL}(y_j, \langle \Phi(\mathbf{X})^T \bm{\alpha}, \phi(\mathbf{x}_i) \rangle) + \frac{1}{2} \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
% & = T \sum_{j=1}^n L_{HL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha}.
% \end{split}
% \end{align}
% % where $L_{HL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle )$.

% Using RHL and SHL, we denote the associated BKSVC as BKSVC-RHL and BKSVC-SHL, respectively.

% \paragraph{Regular hinge loss (RHL)} $L_{RHL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )$.

% Similarly with BLSVC-RHL, setting the subgradient of $\mathcal{L}_{BKSVC}$ for $\bm{\alpha}$ to be $\mathbf{0}$, we estimate $T$ for each $\alpha_i$ as 
% \begin{align}
% \label{kernel_bsvc_rhl_soln}
% \hat{T}^{(i)}_{BKSVC-RHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j, y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle <1} y_j k_{j,i}}.
% \end{align} 

% \paragraph{Squared Hinge Loss (SHL)} $L_{SHL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )^2$. We take the gradient of $\mathcal{L}_{BKSVC}$ for $\bm{\alpha}$ and set it to $\mathbf{0}$, 
% \begin{align}
% \label{kernel_bsvc_shl_soln}
% \hat{T}^{(i)}_{BKSVC-SHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle \leq 1} 2y_j {k}_{j,i} (1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle)}. 
% \end{align}

% For multi-class KSVC, we leverage one-vs-one (or one-vs-rest) fashion of BKSVC~\cite{chang2011libsvm}, similar as what BLSVC does for multi-class LSVC. 

% \subsubsection{Multi-Class KSVC}

\subsection{Towards Theoretical Analysis}

In real-world implementation, in consideration of different aspects, e.g., accuray, computational complexity, stability, convergence, etc., different ML algorithms adopt different optimization algorithms to solve the objective function. For instance, some algorithms can achieve the accurate analytical solution; some can only seek for approximation solutions; some transfrom the primal problem to its dual problem, and solve for optimal values in the dual. %which often produces a difference between the optimal values of the primal and dual problems.  
%However, for convex objective function, the duality gap is 0 under the KKT conditions~\cite{boyd2004convex}.  
To distinguish these algorithms in terms of hyperparameter stealing performance, we formally define 
\begin{definition}[$\epsilon$-Hyperparameter Learnable]
Given training samples that are drawn independently from a certain distribution, and suppose that the optimal model parameters and hyperparameters of a ML algorithm are learnt via certain optimization algorithm in the training phase. Then, we define that the ML model is $\epsilon$-hyperparameter learnable if the relative difference between optimal hyperparameters and stealed hyperparameters is $\epsilon$.
\end{definition}

Then, summarizing all ML models in Section~\ref{attack_cvx_reg} and~\ref{attack_cvx_clf}, we have the following straightforward theorems related to $\epsilon$-hyperparameter learnable. 

% \myparatight{Observation 1} Suppose that the objective function of a ML model is convex, and its parameters $\mathbf{w}_{\text{primal}}$ (or $\bm{\alpha}_{\text{primal}}$) are learnt in the \emph{primal space} with an \emph{accurate analytic solution}, i.e., $\mathbf{w}_{\text{primal}} = \mathbf{w}^{\star}$ (or $\bm{\alpha}_{\text{primal}} = \bm{\alpha}^{\star}$). Then, the ML model is $0$-error hyperparameter learnable.
% RR and KRR belong to this category. 

% \myparatight{Observation 2} Suppose that the objective function of a ML model is convex, but its parameters $\mathbf{w}_{\text{primal}}$ (or $\bm{\alpha}_{\text{primal}}$) are learnt in the \emph{primal space} with an \emph{approximate solution} against optimal parameters $\mathbf{w}^{\star}$, i.e., $\mathbf{w}_{\text{primal}} \neq \mathbf{w}^{\star}$ (or $\bm{\alpha}_{\text{primal}} = \bm{\alpha}^{\star}$). Suppose further that the corresponding learnt hyperparameters are $h_j(\mathbf{w}_{\text{primal}})$ (or $h_j(\bm{\alpha}_{\text{primal}})$) and $h_j(\mathbf{w}^{\star})$ (or $h_j(\bm{\alpha}^{\star})$).
% Then, the ML model is $\frac{|h_j(\mathbf{w}_{\text{primal}})-h_j(\mathbf{w})^{\star}|}{h_j(\mathbf{w})^{\star}}$ (or) error-hyperparameter learnable. 
% LASSO, ENet, BLR, MLR, BKLR, and MKLR belong to this category.

% \myparatight{Observation 3} Suppose that the objective function of a ML model is convex, but its parameters $\mathbf{w}_{\text{dual}}$ (or $\bm{\alpha}_{\text{dual}}$) are obtained in the \emph{dual space}. Suppose further that the corresponding learnt hyperparameters are $h_j(\mathbf{w}_{\text{dual}})$ (or $h_j(\bm{\alpha}_{\text{dual}})$) and $h_j(\mathbf{w})^{\star}$ (or $h_j(\bm{\alpha}^{\star}$). 
% %We define the duality hyperparameter gap as $h_j(\mathbf{w}_{\text{dual}})-h_j(\mathbf{w})^{\star}$, 
% Then, the ML model is $\frac{|h_j(\mathbf{w}_{\text{dual}})-h_j(\mathbf{w})^{\star}|}{h_j(\mathbf{w})^{\star}}$-hyperparameter learnable. Note that if strong duality holds~\cite{boyd2004convex}, then the ML model is $0$-error hyperparameter learnable.
% SVC and KSVC belong to this category.

\begin{theorem}%[$0$-Hyperparameter Learnable]
\label{obs_1}
Suppose that the objective function of a ML algorithm is convex, and its parameters $\mathbf{w}_{\text{primal}}$ (or $\bm{\alpha}_{\text{primal}}$) are learnt in the \emph{primal space} with an \emph{accurate analytic solution}, i.e., $\mathbf{w}_{\text{primal}} = \mathbf{w}^{\star}$ (or $\bm{\alpha}_{\text{primal}} = \bm{\alpha}^{\star}$). Then, the ML model is $0$-hyperparameter learnable.
\end{theorem}
RR and KRR belong to this category. 

\begin{theorem}
\label{obs_2}
Suppose that the objective function of a ML algorithm is convex, but its parameters $\mathbf{w}_{\text{primal}}$ (or $\bm{\alpha}_{\text{primal}}$) are learnt in the \emph{primal space} with an \emph{approximate solution} to $\mathbf{w}^{\star}$, i.e., $\mathbf{w}_{\text{primal}} \neq \mathbf{w}^{\star}$ (or $\bm{\alpha}_{\text{primal}} \neq \bm{\alpha}^{\star}$). Suppose further that the corresponding learnt hyperparameters are $h_j(\mathbf{w}_{\text{primal}})$ (or $h_j(\bm{\alpha}_{\text{primal}})$) and $h_j(\mathbf{w}^{\star})$ (or $h_j(\bm{\alpha}^{\star})$).
Then, the ML model is $\frac{|h_j(\mathbf{w}_{\text{primal}})-h_j(\mathbf{w}^{\star})|}{h_j(\mathbf{w}^{\star})}$ (or $\frac{|h_j(\bm{\alpha}_{\text{primal}})-h_j(\bm{\alpha}^{\star})|}{h_j(\bm{\alpha}^{\star})}$)-hyperparameter learnable.
\end{theorem}
LASSO, ENet, BLR, MLR, BKLR, and MKLR belong to this category.

\begin{theorem}
\label{obs_3}
Suppose that the objective function of a ML algorithm is convex, but its parameters $\mathbf{w}_{\text{dual}}$ (or $\bm{\alpha}_{\text{dual}}$) are obtained in the \emph{dual space}. Suppose further that the corresponding learnt hyperparameters are $h_j(\mathbf{w}_{\text{dual}})$ (or $h_j(\bm{\alpha}_{\text{dual}})$) and $h_j(\mathbf{w})^{\star}$ (or $h_j(\bm{\alpha}^{\star}$). 
%We define the duality hyperparameter gap as $h_j(\mathbf{w}_{\text{dual}})-h_j(\mathbf{w})^{\star}$, 
Then, the ML model is $\frac{|h_j(\mathbf{w}_{\text{dual}})-h_j(\mathbf{w}^{\star})|}{h_j(\mathbf{w}^{\star})}$ (or $\frac{|h_j(\bm{\alpha}_{\text{dual}})-h_j(\bm{\alpha}^{\star})|}{h_j(\bm{\alpha}^{\star})}$)-hyperparameter learnable. Note that if strong duality holds~\cite{boyd2004convex}, then the ML model is $0$-hyperparameter learnable.
\end{theorem}
SVC and KSVC belong to this category.

We will verify above theorems in the experimental results.



==> attack_v1.tex <==
\section{Hyperparameter Stealing Attack}
\label{hyper_attack}

\subsection{Our Attack Framework}

From ML's perspective, we know that the optimal parameters and optimal hyperparameters are learnt via minimizing the objective function of a ML model. In other words, when we achieve the minimal value of the objective function, the parameters and hyperparameters should be optimal. However, the \emph{global minimal} value can be guaranteed if and only if the objective function is convex, as shown in Definition~\ref{cvx_prop}. 
Therefore, another way to describe is that if the objective function is convex and the optimal parameters are given, then the optimal hyperparameters can be stealed by setting the or subgradient of the objective function with respect to the model parameters to be zero. %if the objective function is \emph{smooth} (or \emph{nonsmooth}). 
With such an intuition, our attack framework in the original space can be defined as  
%More specifically, we can leverage \emph{gradient-based} method if the objective function is \emph{smooth} or \emph{subgradient-based} method if it is \emph{nonsmooth}. 
%Mathematically, if the data samples are drawn from the original space, then 
\begin{align}
\label{attack_frame}
\begin{split}
\frac{\mathcal{L}(\mathbf{w}, \mathbf{h})}{\partial \mathbf{w}} & = \sum_{i=1}^n \frac{ \partial \text{Loss}(\mathbf{w}; \mathbf{x}_i, y_i)}{\partial \mathbf{w}} + \sum_{j} h_j \frac{\partial \text{Reg}_j(\mathbf{w})}{\partial \mathbf{w}}. 
\end{split}
\end{align}
%Note that Eqn~\ref{attack_frame} a $m$-dim vector-based derivative. 
By setting it to \textbf{0}, we have a system of $m$ equations and thus can estimate each hyperparameter $h_j$ (Similarly, we have a system of $n$ equations in the kernel-mapped feature space). 

In practice, for different regression models and classification models, loss functions and regularizations are different. For instance, loss functions can be \emph{cross entropy}, \emph{maximum entropy}, \emph{regular hinge loss (RHL)}, and \emph{square hinge loss (SHL)}, etc. Regularizations can be \emph{sparsity-based $l_1$-norm}, \emph{dense-based $l_2$-norm}, etc. 
%Throughout this paper, we only focus on well-known convex ML models. For regression, we take ridge regression, LASSO, ElasticNet as examples; For classification, we choose LR and SVC. 
In the next two subsections, we will provide the detail as how to steal the hyperparameters of well-known convex regression and classification models, respectively. 

\subsection{Attack on Convex-induced Regression Models} 
\label{attack_cvx_reg}

We consider attacks on both linear and kernel-based nonlinear regression models.

\subsubsection{Linear regression models} 
\label{cvx_reg_lin}

We aim at stealing hyperparameters of ridge regression~\cite{hoerl1970ridge}, LASSO~\cite{tibshirani1996regression}, and Elastic Net~\cite{zou2005regularization}. For simplicity, we only show the objective function and 
the stealed hyperparameter(s) of each model. The derivation details are provided in Appendix~\ref{app:cvx_reg}.

\myparatight{Ridge Regression (RR)} The objective function is 
\begin{align}
\label{ridge_reg}
\mathcal{L}_{RR}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X} \mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_2^2.
\end{align}

Taking the gradient of $\mathcal{L}_{RR}$ with respect to $w_i$ and setting it to 0 yields
\begin{align}
\label{ridge_reg_soln}
\hat{\lambda}^{(i)}_{RR} = \frac{-\langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle}{w_i},
\end{align}
where $\mathbf{r}_i = \mathbf{y}-\mathbf{X}_{:,-i} \mathbf{w}_{-i}$ is the residual that all features are used except the $i$-th feature to approximate $\mathbf{y}$. 

%Eqn~\ref{ridge_reg_soln} implies that if we are provided $\mathbf{w}$ by machine learning service provider (who achieves it using some training dataset and certain model selection (e.g., cross validataion, AIC, BIC) technique). Then, we can ``steal" the true hyperparameter $\lambda$, denoted as $\hat{\lambda}_1$. 

%Theoretically, each estimated $\hat{\lambda}^{(i)}_{RR}$ should be the exact $\lambda$. We demonstrate that our estimates are indeed accurate from the experimental results. 

\myparatight{LASSO} The objective function is 
\begin{align}
\label{lasso}
\mathcal{L}_{LASSO}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_1.
\end{align}

Notice that $\| \mathbf{w} \|_1$ is \emph{not differentiable} when $w_i=0$. To handle such a nonsmooth function, we need to extend the notion of gradient to \emph{subgradient}, as defined above. Setting the \emph{subgradient} of $\mathcal{L}_{LASSO}$ with respect to $w_i$ to be 0 yields 
\begin{align}
\label{lasso_soln}
\hat{\lambda}^{(i)}_{LASSO} =  
\begin{cases}
2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if }  w_i < 0 \\
-2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if } w_i > 0 
\end{cases}
\end{align}
 
% Setting $\frac{\partial \mathcal{L}_{LASSO}}{\partial w_i} = 0$, we have three cases of values of $w_i$, which depends on the value of $\lambda$ and $\left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle$, as follows: 
% \begin{align}
% w_i = 
% \begin{case}
% (2 \left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle + \lambda) / (2 \| \mathbf{x}_i \|_2^2) \quad \text{if} \, c_j < -\lambda \\
% 0 \quad \text{if} \, c_j \in [-\lambda, \lambda] \\
% (2 \left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle - \lambda) / (2 \| \mathbf{x}_i \|_2^2) \quad \text{if} \, c_j > \lambda 
% \end{case}
% \end{align}

Note that if $\lambda \geq \lambda_{\max} = \| \mathbf{X}^T \mathbf{y} \|_{\infty} = \max_i |\langle \mathbf{y}, \mathbf{x}_i \rangle|$, then $\mathbf{w} = \mathbf{0}$. It is because $\mathbf{0}$ is optimal if $(\mathbf{X}^T \mathbf{y})_j \in [-\lambda, \lambda]$, for any $j$. Therefore, $\hat{\lambda}^{(i)}_{LASSO} < \max_i |\langle \mathbf{y}, \mathbf{x}_i \rangle|$.

%The value is obtained by using the fact that $\mathbf{0}$ is optimal if $(\mathbf{X}^T \mathbf{y})_j \in [-\lambda, \lambda]$, for any j. Therefore, we have $\hat{\lambda}^{(i)}_{LASSO} < \max_i |\langle \mathbf{y}, \mathbf{x}_i \rangle|$.

\myparatight{Elastic Net (ENet)} The objective function is 
%\subsubsection{Elastic Net: More general case}
\begin{align}
\label{enet}
\mathcal{L}_{ENet}(\lambda_2, \lambda_1, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda_2 \| \mathbf{w} \|_2^2 + \lambda_1 \| \mathbf{w} \|_1.
\end{align}
Note that the regularization uses both $l_2$-norm and $l_1$-norm. 

By setting the subgradient of $\mathcal{L}_{ENet}$ with respect to $w_i$ to be 0, we have the following equations 
%for each $w_i$, we can estimate $\lambda$ and $\lambda$ using the following equations
\begin{align}
\label{enet_eqn_1}
\begin{cases}
-2 \lambda_2 w_i + \lambda_1 = 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if }  w_i < 0 \\
2 \lambda_2 w_i + \lambda_1 = -2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if } w_i > 0 \\
\end{cases}
\end{align}

%Since there are two hyperparameters to be estimated, we therefore need at least two equations.  
% Here we provide two ways given $\mathbf{w}$. The first way is we randomly choose two equations of Eqn~\ref{enet_eqn_1} with the associated nonzero $w_m$s and $w_n$, and calculate the right hand side values, denoted as $f(w_m, r_m)$ and $f(w_n, r_n)$, respectively. Then, $\lambda$ and $\lambda_1$ can be determined in the following cases:
% \begin{align}
% \small
% \label{enet_soln_1}
% \begin{cases}
% \hat{\lambda}_3 = \frac{f(w_n, r_n)-f(w_m, r_m)}{w_m+w_n}, \, \hat{\lambda}_4 = f(w_m,r_m) + 2\hat{\lambda}_3 w_m & \text{if } w_m < 0 \text{ and } w_n > 0 \\
% \hat{\lambda}_3 = \frac{f(w_m, r_m)-f(w_n, r_n)}{w_m+w_n}, \, \hat{\lambda}_4 = f(w_m,r_m) - 2\hat{\lambda}_3 w_m & \text{if } w_m > 0 \text{ and } w_n < 0 \\
% \hat{\lambda}_3 = \frac{f(w_m, r_m)-f(w_n, r_n)}{-w_m+w_n}, \, \hat{\lambda}_4 = f(w_m,r_m) + 2\hat{\lambda}_3 w_m & \text{if } w_m < 0 \text{ and } w_n < 0 \\
% \hat{\lambda}_3 = \frac{f(w_m, r_m)-f(w_n, r_n)}{w_m-w_n}, \, \hat{\lambda}_4 = f(w_m,r_m) - 2\hat{\lambda}_3 w_m & \text{if } w_m > 0 \text{ and } w_n > 0 \\
% \end{cases}
% \end{align}  

Since there are two hyperparameters to be estimated, we therefore need at least two equations.   
Here, we consider estimating $\lambda_2$ and $\lambda_1$ by leveraging all equations in Eqn~\ref{enet_eqn_1}. In this way, the estimate of $\lambda_2$ and $\lambda_1$ can be cast into ``least square regression". Specifically, we denote $l$-th entry of $\mathbf{w}^+$ and $\mathbf{w}^-$ as $w_l^+$ and $w_l^-$. Furthermore, we construct the following matrices  
\begin{align*}
\mathbf{A} = \left[
\begin{array}{cc}
2 w_1^+ & 1 \\
2 w_2^+ & 1 \\
\vdots & \vdots \\
-2 w_1^- & 1 \\
-2 w_2^- & 1 \\
\vdots & \vdots \\
\end{array}
\right], \quad
\bm{\lambda} = \left[ 
\begin{array}{c}
\lambda_2 \\
\lambda_1 \\
\end{array} 
\right], \\
%\quad
\mathbf{b} = \left[ 
\begin{array}{c}
-2 (\mathbf{x}_1^+)^T \mathbf{x}_1^+ w_1^+ + 2 \left\langle \mathbf{x}_1^+, \mathbf{r}_1^+ \right\rangle \\
-2 (\mathbf{x}_2^+)^T \mathbf{x}_2^+ w_1^+ + 2 \left\langle \mathbf{x}_2^+, \mathbf{r}_2^+ \right\rangle \\
\vdots \\
2 (\mathbf{x}_1^-)^T \mathbf{x}_1^- w_1^- - 2 \left\langle \mathbf{x}_1^-, \mathbf{r}_1^- \right\rangle \\
2 (\mathbf{x}_2^-)^T \mathbf{x}_2^- w_2^- - 2 \left\langle \mathbf{x}_2^-, \mathbf{r}_2^- \right\rangle \\
\vdots
\end{array}
\right]. 
\end{align*}

With above notation, the system of equations of Eqn~\ref{enet_eqn_1} can be rewritten into the well-known 
\emph{normal equation}~\cite{montgomery2015introduction}:
\begin{align}
\label{enet_soln_2}
\mathbf{A}^T \mathbf{A} \bm{\lambda} = \mathbf{A}^T \mathbf{b}.
\end{align}
Hence, $\bm{\lambda}$ can be estimated as 
\begin{align}
\hat{\bm{\lambda}}_{ENet} = \left( \mathbf{A}^T \mathbf{A} \right)^{-1} \mathbf{A}^T \mathbf{b}.
\end{align}

% \subsubsection{Support Vector Regression}

% \begin{align}
% \label{svr}
% \mathcal{L}_{SVR}(T, \mathbf{w}) = T \sum_{j=1}^n L_{\epsilon}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2,
% \end{align}
% where 
% \begin{align}
% L_{\epsilon}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) = 
% \begin{cases}
% 0 & \text{if } |y_j - \langle \mathbf{w}, \mathbf{x}^j_T \rangle| \leq \epsilon \\
% |y_j - \langle \mathbf{w}, \mathbf{x}^j_T \rangle | - \epsilon  & \text{if } |y_j - \langle \mathbf{w}, \mathbf{x}^j_T \rangle| > \epsilon
% \end{cases}
% \end{align}
% is the so called $\epsilon$-\textbf{insensitive loss function}. It indicates that any point lying insider an $\epsilon$-tube around the prediction is not penalized. 
% %$\hat{y}_j = \langle \mathbf{w}, \mathbf{x}^j_T \rangle$ and $T = 1 / \lambda$ is a regularization constant.
% Note that the objective is convex, but is not differentiable at the points $y_j = \langle \mathbf{w}, \mathbf{x}^j_T \rangle + \epsilon$ and $y_j = \langle \mathbf{w}, \mathbf{x}^j_T \rangle - \epsilon$ due to the absolute value function in the loss term. 

% % One popular approach is to formulate the problem as a constrained optimization problem by introducing \textbf{slack parameters} to represent the degree to which each sample lies outside the $\epsilon$-tube. Specifically, we rewrite the objective as 
% % \begin{align}
% % \begin{split}
% % & \mathcal{L}_{SVR}(\mathbf{w},\bm{\xi}_+, \bm{\xi}_+, T) = T \sum_{j=1}^n ( \xi^j_+ + \xi^j_- ) + \frac{1}{2} \| \mathbf{w} \|_2^2 \\
% % & \text{s.t. } \langle \mathbf{w} \mathbf{x}^j \rangle - \epsilon - \xi^j_- \leq y_j \leq \langle \mathbf{w} \mathbf{x}^j \rangle + \epsilon + \xi^j_+, \xi^j_+, \xi^j_- \geq 0, \forall j.
% % \end{split}
% % \end{align}

% The subgradient of $L_{\epsilon}$ with respect to $\mathbf{w}$ is then given by 
% \begin{align}
% \frac{\partial L_{\epsilon}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle)}{\partial \mathbf{w}} = 
% \begin{cases}
% -\mathbf{x}^j_T & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle < y_j - \epsilon \\
% \left[ -\mathbf{x}^j_T, \mathbf{0} \right] & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle = y_j - \epsilon \\
% \mathbf{0} & \text{if } y_j - \epsilon < \langle \mathbf{w}, \mathbf{x}^j_T \rangle < y_j + \epsilon \\
% \left[ \mathbf{0}, \mathbf{x}^j_T \right] & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle = y_j + \epsilon \\
% \mathbf{x}^j_T & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle > y_j + \epsilon
% \end{cases}
% \end{align}


% %Here, we consider the case when $\epsilon=0$.

% In practice, for two non-differential points, the subgradient is set to be 0.
% Finally, setting the derivative of $\mathcal{L}_{SVR}$ with respect to $\mathbf{w}$ to zero, we estimate $T$ as  
% \begin{align}
% \hat{T}^{(i)} = \frac{w_i}{\sum\limits_{j,\langle \mathbf{w}, \mathbf{x}^j_T \rangle < y_j - \epsilon} x_{j,i} - \sum\limits_{j,\langle \mathbf{w}, \mathbf{x}^j_T \rangle > y_j + \epsilon} x_{j,i} }
% \end{align}

% It is critical here, as in any regularization scheme, that a proper value is chosen for $C$, the penalty factor. If it is too large, we have a high penalty for nonseparable points and we may store many support vectors and overfit. If it is too small, we may have underfitting." 
% Alpaydin (2004), page 224
% \begin{align}
% \hat{T}^{(i)} = 
% \begin{cases}
% \frac{w_i}{x_{j,i}} & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle < y_j \\
% -\frac{w_i}{x_{j,i}} & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle > y_j
% \end{cases}
% \end{align}

\subsubsection{Nonlinear regression model}
\label{cvx_reg_nonlin}
%\subsubsection{Nonlinear Model}

So far, we have noticed that above linear models represent each data sample in a \emph{fixed, explicit, and finite dimensional feature space}, i.e., $\mathbf{x}_T^j \in \mathbb{R}^m $. However, for certain types of data samples, it is not clear how they can be best represented using a fixed dimensional feature vector. 
%For instance, how can we represent a text document, which can be of variable length? 
To tackle such problems, one popular way is to leverage a \textbf{nonlinear kernel function} $\kappa$ that measures the similarity between data samples in an implicit, abstract, even infinite dimensional feature space. As aforementioned, $\kappa$ is nonnegative and symmetric. Linear regression that uses the kernel function becomes \emph{nonlinear regression}. 

In this paper, for nonlinear regression, we only focus on kernel ridge regression~\cite{welling2013kernel}, as the kernel version of LASSO and Elastic Net are seldom used in practice. 
Furthermore, for kernel function, we only consider \textbf{Gaussian kernel}, a common Mercer kernel and defined as 
%$\kappa(\mathbf{x}, \mathbf{x}^{\prime}) = \exp ( \| \mathbf{x} - \mathbf{x}^\prime \|_2^2 ／ 2 \sigma^2 )$,
\begin{align}
\label{gaussian_kernel}
%\kappa(\mathbf{x}, \mathbf{x}^\prime) = \exp \big( \| \mathbf{x} - \mathbf{x}^\prime \|_2^2 ／ 2 \sigma^2} \big), 
\kappa(\mathbf{x}, \mathbf{x}^\prime) = \exp \Bigg( \frac{\| \mathbf{x} - \mathbf{x}^\prime \|_2^2}{2 \sigma^2} \Bigg), 
\end{align}
where $\sigma^2$ is the bandwidth. 
% \begin{itemize}
% \item Gaussian kernel: $\kappa(\mathbf{x}, \mathbf{x}^\prime) = \exp \big( \frac{\| \mathbf{x} - \mathbf{x}^\prime \|_2^2}{2 \sigma^2} \big)$, where $\sigma^2$ is the bandwidth.
% \item Polynomial kernel: $\kappa(\mathbf{x}, \mathbf{x}^\prime) = (\langle \mathbf{x}, \mathbf{x}^\prime \rangle)^d$, where $d$ is the degree of the polynomial. 
% \end{itemize}      
%Note that aforementioned linear models use the simplest linear kernel, i.e.,  $\kappa(\mathbf{x}, \mathbf{x}^\prime) = \langle \mathbf{x}, \mathbf{x}^\prime \rangle $.

% In general, if the kernel is Mercer kernel (positive definite kernel), then there exists a function $\phi$ mapping $\mathbf{x} \in \mathbb{R}^m$ to $\phi(\mathbf{x}) \in \mathbb{R}^M $ such that 
% \begin{align}
% \kappa(\mathbf{x}, \mathbf{x}^\prime) = \langle \phi(\mathbf{x}), \phi(\mathbf{x}^\prime) \rangle,
% \end{align}
% is an inner product of some feature vectors that are implicitly defined by $\phi$, which depends on the eigen functions of $\kappa$.  Hence, $M$ can be potentially infinite dimension.     

%For nonlinear regression, we only focus on kernel ridge regression (KLR)~\cite{welling2013kernel}, as the kernel version of LASSO and Elastic Net is seldom used in practice. 

\myparatight{Kernel Ridge Regression (KRR)} Given the kernel mapping $\Phi : \mathbb{R}^m \rightarrow \mathbb{R}^M$, where $M$ is the dimension of the feature space. Then, the objective function of kernel ridge regression is 
%\subsubsection{Kernel Ridge Regression}
\begin{align}
\label{kernel_ridge_primal} 
\mathcal{L}_{KRR}(\lambda, \mathbf{w}^\prime) = \| \mathbf{y}-\Phi(\mathbf{X}) \mathbf{w}^\prime \|_2^2 + \lambda \| \mathbf{w}^\prime \|_2^2,
\end{align}
where $\Phi(\mathbf{X}) = \left[ \phi(\mathbf{x}^1_T); \phi(\mathbf{x}^2_T); \cdots; \phi(\mathbf{x}^n_T) \right] \in \mathbb{R}^{n \times M}$. 

However, we need to emphasize that $\lambda$ cannot be solved using Eqn~\ref{kernel_ridge_primal}, as the exact form of each mapped sample $\phi(\mathbf{x}^j_T)$ is unknown. Fortunately, by leveraging \emph{dual representer theorem}~\cite{scholkopf2001generalized}, we can rewrite $\mathbf{w}^\prime$ as a linear combination of $\phi(\mathbf{x}^j_T)$ with an associated coefficient $\alpha_j$. That is, 
\begin{align}
\mathbf{w}^\prime = \sum_{j=1}^n \alpha_j \phi(\mathbf{x}^j_T) = \Phi(\mathbf{X})^T \bm{\alpha}.
\end{align} 
Note that $\bm{\alpha}$ is an $n$-dim vector, the same size as the number of samples. 
Correspondingly, $\mathbf{w}^\prime$ and $ \bm{\alpha}$ are respectively called \textbf{primal parameters} and \textbf{dual parameters}.

In doing so, we can solve $\lambda$ by using $n$-dim $\bm{\alpha}$ instead of $M$-dim $\mathbf{w}^\prime$. Speficically, substituting $\mathbf{w}^\prime$ with $\Phi(\mathbf{X})^T \bm{\alpha}$, Eqn~\ref{kernel_ridge_primal} becomes 
%For ease of computation, kernalized methods often optimize $\bm{\alpha}$ with size $n$ instead of (infinite) $M$-dim $\mathbf{w}^\prime$. Therefore, by substituting $\mathbf{w}^\prime$ with $\Phi(\mathbf{X})^T \bm{\alpha}$, Eqn~\ref{kernel_ridge_primal} becomes 
\begin{align}
\label{kernel_ridge_dual}
\begin{split}
\mathcal{L}_{KRR}(\lambda, \bm{\alpha}) & = \| \mathbf{y}-\Phi(\mathbf{X}) \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 + \lambda \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
& = \| \mathbf{y} - \mathbf{K} \bm{\alpha} \|_2^2 + \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha},
\end{split}
\end{align}
where $\mathbf{K}=\Phi(\mathbf{X}) \Phi(\mathbf{X})^T=\{ \langle \phi(\mathbf{x}^i_T), \phi(\mathbf{x}^j_T) \rangle_{i,j} \}$ is an $n \times n$ Gram matrix. %inner product matrix, also called \textbf{Gram matrix}, defined in the feature space.

Taking the gradient of $\mathcal{L}_{KRR}$ with respect to $\bm{\alpha}$ and setting it to \textbf{0}, we have
\begin{align}
\mathbf{K}(\lambda \bm{\alpha} + \mathbf{K} \bm{\alpha} - \mathbf{y}) = \mathbf{0}.
\end{align} 

Note that $\mathbf{K}$ is positive definite and thus full rank. Multiplying both sides with $\mathbf{K}^{-1}$ yields $\lambda \bm{\alpha} + \mathbf{K} \bm{\alpha} - \mathbf{y} = \mathbf{0}$. Hence, we can estimate $\lambda$ for each $\alpha_j$ as
\begin{align}
\hat{\lambda}^{(j)}_{KRR} = \frac{y_j - \mathbf{k}^{j} \alpha_j}{\alpha_j}. 
\end{align}

%As the kernel version of LASSO and Elastic Net is seldom used in real-world problems, we thus do not provide the analysis. 
 
% \subsubsection{Kernel Support Vector Regression}

% The problem with kernel ridge regression is that the $\mathbf{w}^\prime$ depends on all the training samples. We now seek a method to produce a sparse estimate of $\mathbf{w}^\prime$.

% Leveraging the similar idea as kernel ridge regression, we rewrite primal parameters $\mathbf{w}^{\prime}$ using its dual $\bm{\alpha}$ and have 
% \begin{align}
% \label{kernel_svr}
% \begin{split}
% \mathcal{L}_{KernelSVR}(T, \bm{\alpha}) & = T \sum_{j=1}^n L_{\epsilon}(y_j, \langle \Phi(\mathbf{X})^T \bm{\alpha}, \phi(\mathbf{x}^j_T) \rangle) + \frac{1}{2} \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
% & = T \sum_{j=1}^n L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha}, 
% \end{split}
% \end{align}
% where 
% \begin{align}
% L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = 
% \begin{cases}
% 0 & \text{if } |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle| \leq \epsilon \\
% |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle | - \epsilon  & \text{if } |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle| > \epsilon
% \end{cases}
% \end{align}
% and $\mathbf{k}_j = \Phi(\mathbf{X}) \phi(\mathbf{x}^j_T)$.

% Note again that the objective function is convex but not differentiable at the points $y_j = \langle \bm{\alpha}, \mathbf{k}_j \rangle \pm \epsilon$. Then, the subgradient of $L_{\epsilon}$ with respect to $\bm{\alpha}$ is 
% \begin{align}
% \frac{\partial L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle)}{\partial \bm{\alpha}} = 
% \begin{cases}
% - \mathbf{k}_j & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j - \epsilon \\
% \left[ -\mathbf{k}_j, \mathbf{0} \right] & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle = y_j - \epsilon \\
% \mathbf{0} & \text{if } y_j - \epsilon < \langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j + \epsilon \\
% \left[ \mathbf{0}, \mathbf{k}_j \right] & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle = y_j + \epsilon \\
% \mathbf{k}_j & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle > y_j + \epsilon
% \end{cases}
% \end{align}

% Finally, we set the subgradient of non-differential points as 0 and the derivative of $\mathcal{L}_{KernelSVR}$ with respect to $\bm{\alpha}$ to zero. With it, $T$ is estimated as  
% \begin{align}
% \hat{T}^{(i)} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,\langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j - \epsilon} k_{j,i} - \sum\limits_{j,\langle \bm{\alpha}, \mathbf{k}_j \rangle > y_j + \epsilon} k_{j,i} }
% \end{align}

\subsection{Attack on Convex-induced Classification Models}
\label{attack_cvx_clf}

We consider attacks on both linear and kernel-based nonlinear classification models.

\subsubsection{Linear classification model}
\label{cvx_clf_lin}

In this part, we focus on stealing hyperparameters of two well-known linear classification models, i.e., logistic regression (LR)~\cite{hosmer2013applied} and linear support vector classification (LSVC)~\cite{cortes1995support}. For LR, we consider both its binary case and multi-class case, and denote them as binary LR (BLR) and multi-class LR (MLR), respectively. 

\myparatight{Binary Logistic Regression (BLR)} Taking a single sample $\{\mathbf{x},y\}$ for example, BLR aims at maximizing the following conditional probability with $y \in \{0,1\}$,
%binary classification model with label $y \in {0,1}$: 
\begin{align}
\label{lr_eqn}
Pr(y|\mathbf{x}, \mathbf{w}) = \text{Ber}(y|h_\mathbf{w}(\mathbf{x})) = h_\mathbf{w}(\mathbf{x})^y (1-h_\mathbf{w}(\mathbf{x}))^{1-y},
%Pr(y|\mathbf{x}, \mathbf{w}) = \text{Ber}(y|\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) = \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)^y (1-\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle))^{1-y},
\end{align}
where \textbf{Ber} is bernoulli distribution with $\text{Ber}(k|p)=p$ if $k=1$, and $\text{Ber}(k|p)=1-p$ if $k=0$; $h_\mathbf{w}(\mathbf{x})=\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) $, where \textbf{sigm} refers to the sigmoid (logistic, or logit) function, defined as $\text{sigm}(z)=\frac{1}{1+\exp{(-z)}}$.

In practice, the maximization of Eqn~\ref{lr_eqn} is often transformed to the minimization of nonnegative log-likelihood (NLL), which is given by
\begin{align}
\label{lr_nll}
\begin{split}
& \text{NLL}_{BLR}(\mathbf{w};\mathbf{x},y) = - \log Pr(y|\mathbf{x}, \mathbf{w}) \\
& \qquad = - \big( y \, \log h_\mathbf{w}(\mathbf{x}) + (1-y) \log (1- h_\mathbf{w}(\mathbf{x})) \big). 
%\text{NLL}(\mathbf{w};\mathbf{x},y) = - \log Pr(y|\mathbf{x}, \mathbf{w}) = - \big( y \, \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) + (1-y) (1- \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) \big). 
\end{split}
\end{align}
This is also called \textbf{cross entropy} error function. 

To tackle real-world problems, BLR is often added an $l_2$ or $l_1$ regularization. We consider these two cases in the following.  

\paragraph{$L_2$-regularized BLR (L2-BLR)} Its objective function  is
\begin{align}
\label{l2lr}
\mathcal{L}_{L_2-BLR}(\tau, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};\mathbf{x}^j_T,y_j) + \tau \| \mathbf{w} \|_2^2.
%\mathcal{L}_{L_2-BLR}(\tau, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}^j_T) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] + \tau \| \mathbf{w} \|_2^2,
\end{align}
%where $h_\mathbf{w}(\mathbf{x}^j_T) = \text{sigm}(\mathbf{w}^T \mathbf{x}^j) = \frac{1}{1+\exp(-\mathbf{w}^T \mathbf{x}^j)}$.

Taking the gradient of $\mathcal{L}_{L_2-BLR}$ with respect to $w$ and setting it to 0, we can estimate $\tau$ for each $w_i$ as
\begin{align}
\label{l2lr_soln}
\hat{\tau}^{(i)}_{L_2-BLR} = - \frac{\langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle}{2 w_i},
\end{align}
where $h_\mathbf{w}(\mathbf{X}) = \left[ h_\mathbf{w}(\mathbf{x}^1_T), h_\mathbf{w}(\mathbf{x}^2_T), \cdots, h_\mathbf{w}(\mathbf{x}^n_T) \right]^T \in \mathbb{R}^n$ (See Appendix~\ref{app:l2blr}).

%Unlike aforementioned linear model, we cannot write down the closed form for each $w_i$. 

\paragraph{$L_1$-regularized BLR (L1-BLR)} Its objective function is 
\begin{align}
\label{l1lr}
\mathcal{L}_{L_1-BLR}(\tau, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};\mathbf{x}^j_T,y_j) + \tau \| \mathbf{w} \|_1.
%\mathcal{L}_{L_1-BLR}(\tau, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}^j_T) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] + \tau \| \mathbf{w} \|_1.
\end{align}

Taking the subgradient of $\mathcal{L}_{L_1-BLR}$ with respect to $w$ and setting it to 0, we can estimate $\tau$ for each $w_i$ as
\begin{align}
\label{l1lr_soln}
\hat{\tau}^{(i)}_{L_1-BLR} = 
\begin{cases}
- \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i > 0 \\
 \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i < 0
\end{cases}
\end{align}

\myparatight{Multi-Class Logistic Regression (MLR)} Now we consider MLR, also known as multinomial logistic regression, softmax regression, and maximum entropy classifier. Given a single sample $\{\mathbf{x},y\}$, the model is defined as
\begin{align}
\label{mlr}
Pr(y=c|\mathbf{x},\mathbf{W}) = \frac{\exp{\langle \mathbf{w}_c, \mathbf{x} \rangle}}{\sum_{c^\prime=1}^C \exp{\langle \mathbf{w}_{c^\prime}, \mathbf{x} \rangle}},
\end{align}
where $\mathbf{W}=\left[ \mathbf{w}_1, \cdots, \mathbf{w}_C \right]$, with $c$-th column the coefficients for representing $c$-th class.

To deal with $C$ classes, we introduce some new notation. Let $y_{j,c} = 1(y_j=c)$ be the one-of-$C$ encoding of $y_j$; thus $\mathbf{y}^j$ is a bit vector, in which $c$-th entry $y_{j,c}=1$ when $y_j=c$. We further denote $\mathbf{Y} = \left[ \mathbf{y}^1; \mathbf{y}^2; \cdots ; \mathbf{y}^n \right] = \left[ \mathbf{y}_1, \mathbf{y}_2, \cdots, \mathbf{y}_C \right] \in \mathbb{R}^{n \times C} $ be the label matrix. Then, the NLL for sample $\mathbf{x}^j$ is written as
\begin{align*}
\small
%\label{mlr_nll}
\begin{split}
\text{NLL}_{MLR}(\mathbf{W}; \mathbf{x}^j_T, \mathbf{y}^j) = - \sum_{c=1}^C y_{j,c} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle + \log \big( \sum_{c^\prime=1}^C \exp (\langle \mathbf{w}_{c^\prime}, \mathbf{x}^j_T ) \big).
\end{split}
\end{align*} 

In practice, MLR is added an $l_2$ regularization, termed $L_2$-regularized MLR (L2-MLR). Its objective function is 
\begin{align}
\small
\label{l2mlr}
\mathcal{L}_{L_2-MLR}(\tau, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j_T, \mathbf{y}^j) + \tau \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
%\mathcal{L}_{L_2-MLR}(\tau, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j, \mathbf{y}_j) + \tau \sum_
%{c=1}^C \| \mathbf{w}_c \|_2^2.
\end{align}

By setting the derivative of $\mathcal{L}_{L_2-MLR}$ with respect to $c$-th class $\mathbf{w}_c$ to be zero. Then, for each class $c$ and each $\mathbf{x}_i$, we can estimate $\tau$ as 
\begin{align}
\label{l2mlr_soln_2}
\hat{\tau}^{(i,c)}_{L_2-MLR} = - \frac{\langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle }{2 w_{i,c}},
\end{align}
where $\bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) = \left[ Pr(y_{1,c}=1|\mathbf{x}^1_T, \mathbf{W}), \cdots, Pr(y_{n,c}=1| \mathbf{x}^n_T, \mathbf{W}) \right]^T $  
and $\mathbf{y}_c = \left[ y_{1,c}, y_{2,c}, \cdots , y_{n,c} \right]^T$. 

% \paragraph{$L_1$-regularized MLR}

% \begin{align}
% \label{l1mlr}
% \mathcal{L}_{L_1-MLR}(\tau, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j,\mathbf{y}^j) + \tau \| \mathbf{W} \|_1.
% %\mathcal{L}_{L_1-MLR}(\tau, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j,\mathbf{y}_j) + \tau \sum_{c=1} \| \mathbf{w}_c \|_1.
% \end{align}

% Similarly with $L_2$-regularized MLR, the gradient of $\mathcal{L}_{L_1-MLR}$ with respect to $\mathbf{w}_c$ is given by
% \begin{align}
% \label{l1mlr_soln_1}
% \frac{\partial \mathcal{L}_{L_1-MLR}}{\partial \mathbf{w}_c} = \mathbf{X}^T (\bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c) + \tau \, \partial_{\mathbf{w}_c} \| \mathbf{w}_c \|_1. 
% \end{align}

% Setting $\partial_{\mathbf{w}_c} \mathcal{L}_{L_1-MLR}=0$ and considering the non-differentiability of $\| \mathbf{w}_c \|_1$, we estimate $\tau$ for each feature $\mathbf{x}_i$ and nonzero $w_{i,c}$ as 
% \begin{align}
% \label{l1mlr_soln_2}
% \hat{\tau}^{(i,c)}_8 = 
% \begin{cases}
% - \langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle & \text{if } w_{i,c} > 0 \\
%  \langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle & \text{if } w_{i,c} < 0 \\
% \end{cases}
% \end{align}

\myparatight{Binary Linear Support Vector Classification (BLSVC)}
The objective function of BLSVC is defined as
\begin{align}
\label{hl_bsvc}
\mathcal{L}_{BLSVC}(T, \mathbf{w}) = T \sum_{j=1}^n L_{HL}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2, 
\end{align}
where $L_{HL}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle)$ is the \textbf{hinge loss} for predicting $\mathbf{x}^j_T$. 

There are two common hinge loss functions, i.e., regular hinge loss (RHL) and squared hinge loss (SHL). In correspondence, we denote BLSVC as BLSVC-RHL and BLSVC-SHL, respectively.

\paragraph{Regular hinge loss (RHL)}
$L_{RHL}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) = \max(0, 1 - y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle)$. 
%Figure~\ref{XX} shows its function as well as squared hinge loss. 
Note that RHL is convex, but non-differential when $y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle = 1$. Its subgradient with respect to $\mathbf{w}$ is 
% Once again, it is non-differential because of the \textbf{max} term. However, by introducing slack parameters $\xi_i$, one can show that it is equivalent to solving
% \begin{align}
% \begin{split}
% & \mathcal{L}_{HL-SVM}(T, \mathbf{w}, \bm{\xi}) = T \sum_{j=1}^n \xi_j + \frac{1}{2} \| \mathbf{w} \|^2 \\
% & \text{s.t. } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle \geq 1 - \xi_i, \xi_i \geq 0, \forall i. 
% \end{split}
% \end{align}
%because of the ``max term". Its subgradient with respect to $\mathbf{w}$ is 
\begin{align}
\label{RHL_subg}
\frac{\partial L_{RHL}}{\partial \mathbf{w}} = 
\begin{cases}
-y_j \mathbf{x}^j_T & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1 \\
[-y_j \mathbf{x}^j_T, \mathbf{0}] & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle = 1 \\
\mathbf{0} & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle > 1
\end{cases}
\end{align}

For non-differential point, its subgradient is set to be 0. Therefore, with Eqn~\ref{RHL_subg}, we can estimate the hyperparamter $T$ using only samples $\mathbf{x}^j$ that satisfy $y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1$. Setting the derivative of $\mathcal{L}_{BLSVC}$ with respect to $w_i$ to zero yields
\begin{align}
\hat{T}^{(i)}_{BLSVC-RHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1} y_j {x}_{j,i}}. 
%T \sum_{j,y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1} -y_j \mathbf{x}^j + \mathbf{w} = 0, \quad \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1.
%T \sum_{j=1}^n -y_j \mathbf{x}^j + \mathbf{w} = 0, \quad \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1.
\end{align} 

\paragraph{Squared Hinge Loss (SHL)} 
$L_{SHL}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) = \max(0, 1 - y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle)^2$. SHL is convex, smooth, and differential. Its subgradient with respect to $\mathbf{w}$ is given by
\begin{align}  
\label{SHL_subg}
\frac{\partial L_{SHL}}{\partial \mathbf{w}} =
\begin{cases}
-2 y_j \mathbf{x}^j_T (1 - y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle) & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle <= 1 \\
\mathbf{0}  & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle > 1
\end{cases}
\end{align}

Therefore, taking the derivative of $\mathcal{L}_{BLSVC}$ with respect to $w_i$ to zero in this case  yields
\begin{align}
\hat{T}^{(i)}_{BLSVC-SHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle \leq 1} 2y_j {x}_{j,i} (1 - y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle) }. 
\end{align}

For multi-class LSVC, it can be derivated from binary LSVC in a one-vs-one (or one-vs-rest) fashion~\cite{chang2011libsvm}. In this setting, we can run binary classification Eqn~\ref{hl_bsvc} $K \times (K-1)/2 $ (or $K$) times to estimate the hyperparater.

% \subsubsection{Multi-Class LSVC}

% Normally, binary LSVC is extended to multi-class linear SVC in a one-vs-one or one-vs-rest fashion [2]. In this setting, we can run binary classification Eqn~\ref{hl_bsvc} $K \times (K-1)/2 $ and $K$ times to estimate the hyperparater. However, there exists a ``true" multi-class version hinge loss (MHL) for multi-class SVC, due to Crammer and Singer [3], which optimizes a joint objective over all classes and is defined as
% \begin{align}
% \label{crammer_singer_msvc}
% \begin{split}
% & \min_{\mathbf{W},\epsilon} \quad \mathcal{L}_{MSVC}(T, \mathbf{W}) =  T \sum_{j=1}^n \epsilon_j + \frac{1}{2} \sum_{c=1}^T \| \mathbf{w}_c \|_2^2 \\
% & \text{s.t.} \quad	\langle \mathbf{w}_{y_j}, \mathbf{x}^j_T  \rangle - \langle \mathbf{w}_c, \mathbf{x}^j_T  \rangle  \geq e_j^c - \epsilon_j \\
% & \quad \quad \epsilon_j \geq 0, \, j=1,\cdots, n; \, c=1, \cdots, T, 
% \end{split}
% \end{align}
% where $e_j^c = 0$ if $y_j = c$, and $e_j^c = 1$ if $y_j \neq c$ and $\mathbf{W} = \left[ \mathbf{w}_1, \mathbf{w}_2, \cdots, \mathbf{w}_C \right]$. 

% The decision function to predict the label of a new instance $\mathbf{x}$ is $\argmax\nolimits_{c=1,\cdots,C} \langle \mathbf{w}_c, \mathbf{x} \rangle $.

% Directly setting the derivative of $\mathcal{L}_{MSVC}$ for $\mathbf{w}_c$ via Eqn~\ref{crammer_singer_msvc} in a constrainted form is difficult. Therefore, we transform it to the equivalent unconstrained form as follows
% % \begin{align}
% % \mathcal{L}_{MSVC}(T, \mathbf{W}) = T \sum_{j=1}^n \sum_{c \neq y_j} L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2,
% % \end{align}
% \begin{align}
% \mathcal{L}_{MSVC}(T, \mathbf{W}) = T \sum_{j=1}^n L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2,
% \end{align}
% where $L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle) = \max(0, 1 + \max\nolimits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle)$ is the maximal hinge loss among $C$ classes for predicting $\mathbf{x}^j$. 

% % Similarly, there are also two MHL functions, i.e., regular MHL and squared MHL. 

% % \textbf{Regular multi-class hinge loss (RMHL):} $L_{RMHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j \rangle) = \max(0, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}_j \rangle)$. 

% %Therefore, the objective function in this setting becomes
% In this way, the objective function then becomes
% \begin{align}
% \mathcal{L}_{MSVC}(T, \mathbf{w}) = T \sum_{j=1}^n \max(0, 1 + \max_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
% \end{align}

% Its subgradient with respect to $\mathbf{w}_c$ is 
% \begin{align}
% \frac{\partial MSVC}{\partial \mathbf{w}_c} =
% \begin{cases}
% T \sum\limits_{j=1}^n \mathbf{x}^j_T + \mathbf{w}_c & \text{if } 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle > 0 \\
% \mathbf{0} & \text{if } 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle < 0
% \end{cases}
% \end{align}

% % \begin{align}
% % \mathcal{L}_{MSVC}(T, \mathbf{w}) = T \sum_{j=1}^n \sum_{c \neq y_j} \max(0, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
% % \end{align}

% % Its subgradient with respect to $\mathbf{w}_c$ is 
% % \begin{align}
% % \frac{\partial MSVC}{\partial \mathbf{w}_c} =
% % \begin{cases}
% % T \sum_{j=1}^n \mathbf{x}^j + \mathbf{w}_c & \text{if } 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle > 0 \\
% % \mathbf{0} & \text{if } 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle < 0
% % \end{cases}
% % \end{align}

% Setting it to zero, we have 
% % \begin{align}
% % \hat{T}^{(i,c)} = - \frac{w_{i,c}}{\sum\limits_{j, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle > 0} x_{j,i}}. 
% % \end{align}
% \begin{align}
% \hat{T}^{(i,c)} = - \frac{w_{i,c}}{\sum\limits_{j, 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle > 0} x_{j,i}}. 
% \end{align}

\subsubsection{Nonlinear classification model}
\label{cvx_clf_nonlin}

We kernelize above linear classification methods to generate corresponding nonlinear models. 

\myparatight{Binary Kernel Logistic Regression (BKLR)~\cite{zhu2001kernel}} Given a single sample $\{\mathbf{x},y\}$, BKLR is to minimize the following NLL
\begin{align*}
%\label{klr_nll}
\begin{split}
& \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}),y) = - \log Pr(y|\phi(\mathbf{x}), \mathbf{w}^\prime) \\
& \qquad = - \big( y \, \log h_{\mathbf{w}^\prime}(\phi(\mathbf{x})) + (1-y) \log (1- h_{\mathbf{w}^\prime}(\phi(\mathbf{x}))) \big)
%\text{NLL}(\mathbf{w};\mathbf{x},y) = - \log Pr(y|\mathbf{x}, \mathbf{w}) = - \big( y \, \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) + (1-y) (1- \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) \big). 
\end{split}
\end{align*}
%where $h_{\mathbf{w}^\prime}(\phi(\mathbf{x}))) = \frac{1}{1+\exp(\langle \bm{\alpha}, \rangle)}$ 

In practice, BKLR is added an $l_2$ or $l_1$ regularization.

\paragraph{$L_2$-regularized BKLR (L2-BKLR)} Its objective function with primal parameters is  
% Minimize the following 
\begin{align*}
%\label{l2klr_primal}
\mathcal{L}_{L_2-BKLR}(\tau, \mathbf{w}^\prime) = \sum_{j=1}^n \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}^j_T),y_j) + \tau \| \mathbf{w}^\prime \|_2^2.
%\mathcal{L}_{L_2-BLR}(\tau, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}^j_T) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] + \tau \| \mathbf{w} \|_2^2,
\end{align*}
%where $h_\mathbf{w}(\mathbf{x}^j_T) = \text{sigm}(\mathbf{w}^T \mathbf{x}^j) = \frac{1}{1+\exp(-\mathbf{w}^T \mathbf{x}^j)}$.

Again, using dual representation $\mathbf{w}^\prime = \Phi(\mathbf{X})^T \bm{\alpha}$, we have its dual form
\begin{align}
\small
\label{l2klr_dual}
\begin{split}
& \mathcal{L}_{L_2-BKLR}(\tau, \bm{\alpha}) = \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + \tau \bm{\alpha}^T \mathbf{K} \bm{\alpha} \\
& = \sum_{j=1}^n - \big( y_j \, \log h_{\bm{\alpha}}(\mathbf{k}_j) + (1 - y_j) (1- h_{\bm{\alpha}}(\mathbf{k}_j)) \big) + \tau \bm{\alpha}^T \mathbf{K} \bm{\alpha},
\end{split}
\end{align} 
where $h_{\bm{\alpha}}(\mathbf{k}_j) = \frac{1}{1 + \exp{\langle \bm{\alpha}, \mathbf{k}_j \rangle}}$

By setting the derivative of $\mathcal{L}_{L_2-BKLR}$ with respect to $\bm{\alpha}$ to be zero, for each $\alpha_i$, we estimate $\tau$ as
\begin{align}
\label{l2klr_soln}
\hat{\tau}^{(j)}_{L_2-BKLR} = - \frac{h_{\bm{\alpha}}(\mathbf{k}_j) - y_j} {2 \alpha_j}.
\end{align}

\paragraph{$L_1$-regularized BKLR (L1-BKLR)} Its objective function of primal parameters is 
\begin{align*}
%\label{l1klr_primal}
\mathcal{L}_{L_1-BKLR}(\tau, \mathbf{w}^\prime) = \sum_{j=1}^n \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}^j_T),y_j) + \tau \| \mathbf{w}^\prime \|_1.
%\mathcal{L}_{L_2-BLR}(\tau, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}^j_T) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] + \tau \| \mathbf{w} \|_2^2,
\end{align*}

Using $\mathbf{w}^\prime = \Phi(\mathbf{X})^T \bm{\alpha}$, we have its dual form
\begin{align}
\small
\begin{split}
\label{l1klr_dual}
\mathcal{L}_{L_1-BKLR}(\tau, \bm{\alpha}) & = - \sum_{j=1}^n \big( y_j \, \log h_{\bm{\alpha}}(\mathbf{k}_j) + (1 - y_j) (1- h_{\bm{\alpha}}(\mathbf{k}_j)) \big) \\ 
& + \tau \| \mathbf{K} \bm{\alpha} \|_1. 
\end{split}
\end{align} 

By setting the subgradient of $\mathcal{L}_{L_1-BKLR}$ with respect to $\bm{\alpha}$ to be zero, we estimate $\tau$ as 
\begin{align}
\label{llklr_soln}
\hat{\tau}^{(j)}_{L_1-BKLR} = 
\begin{cases}
 y_j - h_{\bm{\alpha}}(\mathbf{k}_j)  & \text{if } \mathbf{k}^j \bm{\alpha} > 0 \\
 h_{\bm{\alpha}}(\mathbf{k}_j) - y_j  & \text{if } \mathbf{k}^j \bm{\alpha} < 0
\end{cases}
\end{align} 

\myparatight{Multi-Class Kernel Logistic Regression (MKLR)}
Similarly with MLR, MKLR also uses one-of-$C$ code to represent each label $\mathbf{y}$ and dual representation, the NLL of MKLR for $C$-class and $N$ samples is defined as 
\begin{align*}
\begin{split}
& \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) = - \sum_{j=1}^N \sum_{c=1}^C y_{j,c} \log Pr(y_{j,c}=1 | \mathbf{k}_j, \bm{\Omega}) \\ 
& \qquad = - \sum_{j=1}^N \bigg( \sum_{c=1}^C y_{j,c} \langle \bm{\alpha}_c, \mathbf{k}_j \rangle + \log \big( \sum_{c^\prime=1}^C \exp (\langle \bm{\alpha}_{c^\prime}, \mathbf{k}_j \rangle) \big) \bigg), 
\end{split}
\end{align*}
where $\bm{\Omega} = \left[ \bm{\alpha}_1, \bm{\alpha}_2, \cdots, \bm{\alpha}_C \right]$.

In practice, MKLR often adds an $l_2$ regularization, termed L2-regularized MKLR (L2-MKLR). Similarly with L2-MLR, its objective function of dual parameters is
\begin{align}
\mathcal{L}_{L_2-MKLR}(\tau, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + \tau \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c.  
\end{align}
and its gradient of $\bm{\alpha}_c$ is given by
\begin{align}
\frac{\partial \mathcal{L}_{L_2-MKLR}}{\partial \bm{\alpha}_c} = \mathbf{K} (\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) - \mathbf{y}_c + 2 \tau \bm{\alpha}_c),
\end{align}
where $\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) = \left[ Pr(y_{1,c}=1 | \mathbf{k}_1, \bm{\Omega}), \cdots, Pr(y_{1,c}=n | \mathbf{k}_n, \bm{\Omega}) \right]$.
% where $\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) = \left[ Pr(y_{1,c}=1 | \mathbf{k}_1, \bm{\Omega}), Pr(y_{2,c}=1 | \mathbf{k}_2, \bm{\Omega}), \cdots, Pr(y_{1,c}=n | \mathbf{k}_n, \bm{\Omega}) \right]$.

By setting it to \textbf{0}, for each class $c$, we can estimate $\tau$ as
\begin{align}
\hat{\tau}^{(j,c)}_{L_2-MKLR} = \frac{y_{j,c} - \bm{\mu}_{c, \bm{\Omega}}(\mathbf{k}_j)}{2 \alpha_{j,c}}.
\end{align}

\myparatight{Binary Kernel Support Vector Classification (BKSVC)}
The objective function of BKSVC in the primal form is defined as
\begin{align*}
\small
%\label{kernel_bsvc_prime}
\mathcal{L}_{BKSVC}(T, \mathbf{w^\prime})  = T \sum_{j=1}^n L_{HL}(y_j, \langle \mathbf{w^\prime}, \phi(\mathbf{x}^j_T) \rangle) + \frac{1}{2} \| \mathbf{w^\prime} \|_2^2. 
\end{align*}

Using dual representation $\mathbf{w}^\prime = \Phi(\mathbf{X})^T \bm{\alpha}$, we have its dual form
\begin{align}
\small
\label{kernel_bsvc_dual}
\begin{split}
\mathcal{L}_{BKSVC}(T, \bm{\alpha}) & = T \sum_{j=1}^n L_{HL}(y_j, \langle \Phi(\mathbf{X})^T \bm{\alpha}, \phi(\mathbf{x}^j_T) \rangle) + \frac{1}{2} \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
& = T \sum_{j=1}^n L_{HL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha}.
\end{split}
\end{align}
% where $L_{HL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle )$.

Using RHL and SHL, we denote the associated BKSVC as BKSVC-RHL and BKSVC-SHL, respectively.

\paragraph{Regular hinge loss (RHL)} $L_{RHL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )$.

Similarly with BLSVC-RHL, setting the subgradient of $\mathcal{L}_{BKSVC}$ for $\bm{\alpha}$ to be $\mathbf{0}$, we estimate $T$ for each $\alpha_i$ as 
\begin{align}
\label{kernel_bsvc_rhl_soln}
\hat{T}^{(i)}_{BKSVC-RHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j, y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle <1} y_j k_{j,i}}.
\end{align} 

\paragraph{Squared Hinge Loss (SHL)} $L_{SHL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )^2$. We take the gradient of $\mathcal{L}_{BKSVC}$ for $\bm{\alpha}$ and set it to $\mathbf{0}$, 
\begin{align}
\label{kernel_bsvc_shl_soln}
\hat{T}^{(i)}_{BKSVC-SHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle \leq 1} 2y_j {k}_{j,i} (1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle)}. 
\end{align}

For multi-class KSVC, we leverage one-vs-one (or one-vs-rest) fashion of BKSVC~\cite{chang2011libsvm}, similar as what BLSVC does for multi-class LSVC. 

% \subsubsection{Multi-Class KSVC}

\subsection{Towards Pracitcal Analysis}

In real-world implementation, in consideration of different aspects of a model, e.g., accuray, computational complexity, stability, convergence, etc., different regression and classification models adopt different techniques to solve the objective function. For instance, some models can achieve the accurate analytical solution; some models cannot obtain analytic solution and seek for  approximation methods; some models leverage duality theorem to transfrom the primal problem to its dual problem, which often produces a difference between the optimal values of the primal and dual problems. 
%However, for convex objective function, the duality gap is 0 under the KKT conditions~\cite{boyd2004convex}.  

To summarize all mentioned ML models in Section~\ref{attack_cvx_reg} and~\ref{attack_cvx_clf}, we have the following straightforward theorems in terms of $\epsilon$-error hyperparameter learnable. 

% \myparatight{Observation 1} Suppose that the objective function of a ML model is convex, and its parameters $\mathbf{w}_{\text{primal}}$ (or $\bm{\alpha}_{\text{primal}}$) are learnt in the \emph{primal space} with an \emph{accurate analytic solution}, i.e., $\mathbf{w}_{\text{primal}} = \mathbf{w}^{\star}$ (or $\bm{\alpha}_{\text{primal}} = \bm{\alpha}^{\star}$). Then, the ML model is $0$-error hyperparameter learnable.
% RR and KRR belong to this category. 

% \myparatight{Observation 2} Suppose that the objective function of a ML model is convex, but its parameters $\mathbf{w}_{\text{primal}}$ (or $\bm{\alpha}_{\text{primal}}$) are learnt in the \emph{primal space} with an \emph{approximate solution} against optimal parameters $\mathbf{w}^{\star}$, i.e., $\mathbf{w}_{\text{primal}} \neq \mathbf{w}^{\star}$ (or $\bm{\alpha}_{\text{primal}} = \bm{\alpha}^{\star}$). Suppose further that the corresponding learnt hyperparameters are $h_j(\mathbf{w}_{\text{primal}})$ (or $h_j(\bm{\alpha}_{\text{primal}})$) and $h_j(\mathbf{w}^{\star})$ (or $h_j(\bm{\alpha}^{\star})$).
% Then, the ML model is $\frac{|h_j(\mathbf{w}_{\text{primal}})-h_j(\mathbf{w})^{\star}|}{h_j(\mathbf{w})^{\star}}$ (or) error-hyperparameter learnable. 
% LASSO, ENet, BLR, MLR, BKLR, and MKLR belong to this category.

% \myparatight{Observation 3} Suppose that the objective function of a ML model is convex, but its parameters $\mathbf{w}_{\text{dual}}$ (or $\bm{\alpha}_{\text{dual}}$) are obtained in the \emph{dual space}. Suppose further that the corresponding learnt hyperparameters are $h_j(\mathbf{w}_{\text{dual}})$ (or $h_j(\bm{\alpha}_{\text{dual}})$) and $h_j(\mathbf{w})^{\star}$ (or $h_j(\bm{\alpha}^{\star}$). 
% %We define the duality hyperparameter gap as $h_j(\mathbf{w}_{\text{dual}})-h_j(\mathbf{w})^{\star}$, 
% Then, the ML model is $\frac{|h_j(\mathbf{w}_{\text{dual}})-h_j(\mathbf{w})^{\star}|}{h_j(\mathbf{w})^{\star}}$-hyperparameter learnable. Note that if strong duality holds~\cite{boyd2004convex}, then the ML model is $0$-error hyperparameter learnable.
% SVC and KSVC belong to this category.

\begin{observation}%[$0$-Hyperparameter Learnable]
\label{obs_1}
Suppose that the objective function of a ML model is convex, and its parameters $\mathbf{w}_{\text{primal}}$ (or $\bm{\alpha}_{\text{primal}}$) are learnt in the \emph{primal space} with an \emph{accurate analytic solution}, i.e., $\mathbf{w}_{\text{primal}} = \mathbf{w}^{\star}$ (or $\bm{\alpha}_{\text{primal}} = \bm{\alpha}^{\star}$). Then, the ML model is $0$-error hyperparameter learnable.
\end{observation}
RR and KRR belong to this category. 

\begin{observation}
\label{obs_2}
Suppose that the objective function of a ML model is convex, but its parameters $\mathbf{w}_{\text{primal}}$ (or $\bm{\alpha}_{\text{primal}}$) are learnt in the \emph{primal space} with an \emph{approximate solution} against optimal parameters $\mathbf{w}^{\star}$, i.e., $\mathbf{w}_{\text{primal}} \neq \mathbf{w}^{\star}$ (or $\bm{\alpha}_{\text{primal}} \neq \bm{\alpha}^{\star}$). Suppose further that the corresponding learnt hyperparameters are $h_j(\mathbf{w}_{\text{primal}})$ (or $h_j(\bm{\alpha}_{\text{primal}})$) and $h_j(\mathbf{w}^{\star})$ (or $h_j(\bm{\alpha}^{\star})$).
Then, the ML model is $\frac{|h_j(\mathbf{w}_{\text{primal}})-h_j(\mathbf{w}^{\star})|}{h_j(\mathbf{w}^{\star})}$ (or $\frac{|h_j(\bm{\alpha}_{\text{primal}})-h_j(\bm{\alpha}^{\star})|}{h_j(\bm{\alpha}^{\star})}$)-error hyperparameter learnable.
\end{observation}
LASSO, ENet, BLR, MLR, BKLR, and MKLR belong to this category.

\begin{observation}
\label{obs_3}
Suppose that the objective function of a ML model is convex, but its parameters $\mathbf{w}_{\text{dual}}$ (or $\bm{\alpha}_{\text{dual}}$) are obtained in the \emph{dual space}. Suppose further that the corresponding learnt hyperparameters are $h_j(\mathbf{w}_{\text{dual}})$ (or $h_j(\bm{\alpha}_{\text{dual}})$) and $h_j(\mathbf{w})^{\star}$ (or $h_j(\bm{\alpha}^{\star}$). 
%We define the duality hyperparameter gap as $h_j(\mathbf{w}_{\text{dual}})-h_j(\mathbf{w})^{\star}$, 
Then, the ML model is $\frac{|h_j(\mathbf{w}_{\text{dual}})-h_j(\mathbf{w}^{\star})|}{h_j(\mathbf{w}^{\star})}$ (or $\frac{|h_j(\bm{\alpha}_{\text{dual}})-h_j(\bm{\alpha}^{\star})|}{h_j(\bm{\alpha}^{\star})}$)-error hyperparameter learnable. Note that if strong duality holds~\cite{boyd2004convex}, then the ML model is $0$-error hyperparameter learnable.
\end{observation}
SVC and KSVC belong to this category.

We will demonstrate above observations in the experimental results.



==> clf.tex <==
\subsection{Attack on Convex-induced Classification Models}

\subsubsection{Linear model-based classification}

\textbf{Logistic Regression}

%\subsubsection{Binary LR}

\textbf{Case 1: Binary LR}

Binary logistic regression (BLR) corresponds to maximize the following conditional probability with $y \in \{0,1\}$:
%binary classification model with label $y \in {0,1}$: 
\begin{align}
\label{lr_eqn}
Pr(y|\mathbf{x}, \mathbf{w}) = \text{Ber}(y|h_\mathbf{w}(\mathbf{x})) = h_\mathbf{w}(\mathbf{x})^y (1-h_\mathbf{w}(\mathbf{x}))^{1-y},
%Pr(y|\mathbf{x}, \mathbf{w}) = \text{Ber}(y|\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) = \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)^y (1-\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle))^{1-y},
\end{align}
where \textbf{Ber} is bernoulli distribution with $\text{Ber}(k|p)=p$ if $k=1$, and $\text{Ber}(k|p)=1-p$ if $k=0$. $h_\mathbf{w}(\mathbf{x})=\text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) $, with \textbf{sigm} refering to the sigmoid (logistic, or logit) function, defined as $\text{sigm}(z)=\frac{1}{1+\exp{(-z)}}$.

In practice, we often transform the maximization in Eqn~\ref{lr_eqn} to the minimization of nonnegative log-likelihood (NLL), which is given by
\begin{align}
\label{lr_nll}
\begin{split}
\text{NLL}_{BLR}(\mathbf{w};\mathbf{x},y) & = - \log Pr(y|\mathbf{x}, \mathbf{w}) \\
& = - \big( y \, \log h_\mathbf{w}(\mathbf{x}) + (1-y) \log (1- h_\mathbf{w}(\mathbf{x})) \big). 
%\text{NLL}(\mathbf{w};\mathbf{x},y) = - \log Pr(y|\mathbf{x}, \mathbf{w}) = - \big( y \, \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) + (1-y) (1- \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) \big). 
\end{split}
\end{align}
This is also called \textbf{cross-entropy} error function. 

\paragraph{$L_2$-regularized BLR}

% Minimize the following 
\begin{align}
\label{l2lr}
\mathcal{L}_{L_2-BLR}(\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};\mathbf{x}^j_T,y_j) + \lambda \| \mathbf{w} \|_2^2.
%\mathcal{L}_{L_2-BLR}(\lambda, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}^j_T) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] + \lambda \| \mathbf{w} \|_2^2,
\end{align}
%where $h_\mathbf{w}(\mathbf{x}^j_T) = \text{sigm}(\mathbf{w}^T \mathbf{x}^j) = \frac{1}{1+\exp(-\mathbf{w}^T \mathbf{x}^j)}$.

The gradient of $\mathcal{L}_{L_2-BLR}$ with respect to $\mathbf{w}$ is given by
\begin{align}
\small
\label{l2lr_soln_1}
\begin{split}
& \frac{\partial \mathcal{L}_{L_2-BLR}}{\partial \mathbf{w}} = - \sum_{j=1}^n \left[ y_j \frac{1}{h_\mathbf{w}(\mathbf{x}^j_T)} \frac{\partial h_\mathbf{w}(\mathbf{x}^j_T)}{\partial \mathbf{w}} + (1-y_j) \frac{-1}{1-h_\mathbf{w}(\mathbf{x}^j_T)} \frac{\partial h_\mathbf{w}(\mathbf{x}^j_T)}{\partial \mathbf{w}}\right] + 2 \lambda \mathbf{w} \\
& \quad = - \sum_{j=1}^n \left[ y_j \frac{1}{h_\mathbf{w}(\mathbf{x}^j_T)} h_\mathbf{w}(\mathbf{x}^j_T) (1-h_\mathbf{w}(\mathbf{x}^j_T)) + (1-y_j) \frac{1}{1-h_\mathbf{w}(\mathbf{x}^j_T)} h_\mathbf{w}(\mathbf{x}^j_T) (1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] \frac{\partial \mathbf{w}^T \mathbf{x}^j}{\partial \mathbf{w}} + 2 \lambda \mathbf{w} \\
& \quad = - \sum_{j=1}^n \left(y_j (1-h_\mathbf{w}(\mathbf{x}^j_T)) - (1-y_j) h_\mathbf{w}(\mathbf{x}^j_T) \right) \mathbf{x}^j + 2 \lambda \mathbf{w} \\ 
& \quad = \sum_{j=1}^n (h_\mathbf{w}(\mathbf{x}^j_T) - y_j) \mathbf{x}^j + 2 \lambda \mathbf{w} \\ 
& \quad = \mathbf{X}^T (h_\mathbf{w}(\mathbf{X}) - \mathbf{y}) + 2 \lambda \mathbf{w}
\end{split}
\end{align}
where $h_\mathbf{w}(\mathbf{X}) = \left[ h_\mathbf{w}(\mathbf{x}^1_T), h_\mathbf{w}(\mathbf{x}^2_T), \cdots, h_\mathbf{w}(\mathbf{x}^n_T) \right]^T \in \mathbb{R}^n$.

Given $\mathbf{w}$, we set $\partial_\mathbf{w} \mathcal{L}_{L_2-BLR} = \mathbf{0}$ and rewrite Eqn~\ref{l2lr_soln_1} for each $w_i$. In doing so, $\lambda$ is estimated as
\begin{align}
\label{l2lr_soln_2}
\hat{\lambda}^{(i)}_{L_2-BLR} = - \frac{\langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle}{2 w_i}.
\end{align}

%Unlike aforementioned linear model, we cannot write down the closed form for each $w_i$. 

\paragraph{$L_1$-regularized BLR}

\begin{align}
\label{l1lr}
\mathcal{L}_{L_1-BLR}(\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};\mathbf{x}^j_T,y_j) + \lambda \| \mathbf{w} \|_1.
%\mathcal{L}_{L_1-BLR}(\lambda, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}^j_T) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] + \lambda \| \mathbf{w} \|_1.
\end{align}

Similarly with $L_2$-regularized BLR, the gradient of $\mathcal{L}_{L_1-BLR}$ with respect to $\mathbf{w}$ is given by
\begin{align}
\label{l1lr_soln_1}
\frac{\partial \mathcal{L}_{L_1-BLR}}{\partial \mathbf{w}} = \mathbf{X}^T (h_\mathbf{w}(\mathbf{X}) - \mathbf{y}) + \lambda \partial_\mathbf{w} \| \mathbf{w} \|_1. 
\end{align}

Setting $\partial_\mathbf{w} \mathcal{L}_{L_1-BLR}=0$ and considering the non-differentiability of $\| \mathbf{w} \|_1$, we estimate $\lambda$ for each nonzero $w_i$ as 
\begin{align}
\label{l1lr_soln_2}
\hat{\lambda}^{(i)}_{L_1-BLR} = 
\begin{cases}
- \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i > 0 \\
 \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i < 0 \\
\end{cases}
\end{align}

\textbf{Case 2: Multi-Class LR}

Now we consider multi-class logistic regression (MLR), also known as multinomial logistic regressions, softmax regression, and maximum entropy classifier. The form of the model is defined as
\begin{align}
\label{mlr}
Pr(y=c|\mathbf{x},\mathbf{W}) = \frac{\exp{\langle \mathbf{w}_c, \mathbf{x} \rangle}}{\sum_{c^\prime=1}^C \exp{\langle \mathbf{w}_{c^\prime}, \mathbf{x} \rangle}},
\end{align}
where $\mathbf{W}=\left[ \mathbf{w}_1, \cdots, \mathbf{w}_C \right]$, with $c$-th column the coefficients for representing $c$-th class.

To handle $C$ classes, we introduce some new notation. Let $y_{j,c} = 1(y_j=c)$ be the one-of-$C$ encoding of $y_j$; thus $\mathbf{y}^j$ is a bit vector, in which $c$-th entry $y_{j,c}=1$ when $y_j=c$. We further denote $\mathbf{Y} = \left[ \mathbf{y}^1; \mathbf{y}^2; \cdots ; \mathbf{y}^n \right] = \left[ \mathbf{y}_1, \mathbf{y}_2, \cdots, \mathbf{y}_C \right] \in \mathbb{R}^{n \times C} $ be the label matrix. With this, 
the NLL for sample $\mathbf{x}^j$ can be written as
\begin{align}
\label{mlr_nll}
\begin{split}
& \text{NLL}_{MLR}(\mathbf{W}; \mathbf{x}^j_T, \mathbf{y}^j) = - \log \prod_{c=1}^C Pr(y_{j,c}=1|\mathbf{x}^j_T,\mathbf{W})^{y_{j,c}} \\
& \qquad = - \sum_{c=1}^C y_{j,c} \log  Pr(y_{j,c}=1|\mathbf{x}^j_T,\mathbf{W}) \\
& \qquad = - \sum_{c=1}^C y_{j,c} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle + \sum_{c=1}^C y_{j,c} \log \big( \sum_{c^\prime=1}^C \exp (\langle \mathbf{w}_{c^\prime}, \mathbf{x}^j_T ) \big) \\ 
& \qquad = - \sum_{c=1}^C y_{j,c} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle + \log \big( \sum_{c^\prime=1}^C \exp (\langle \mathbf{w}_{c^\prime}, \mathbf{x}^j_T ) \big),
\end{split}
\end{align} 
where we use the fact that $\sum_{c} y_{j,c} = 1$ in the second equation.

For each class $c$, the derivative of $\text{NLL}_{MLR}$ for $\mathbf{w}_c$ with sample $\mathbf{x}^j$ is given by
\begin{align}
\label{mlr_nll_grad}
\begin{split} 
\frac{\partial \text{NLL}_{MLR}}{\partial \mathbf{w}_c} & = - y_{j,c} \mathbf{x}^j_T + \frac{\exp(\langle \mathbf{w}_{c^\prime}, \mathbf{x}^j_T \rangle)}{\sum_{c^\prime = 1}^C \exp (\langle \mathbf{c^\prime}, \mathbf{x}^j_T \rangle)} \mathbf{x}^j_T \\ 
& = \big( Pr(y_{j,c}=1|\mathbf{x}^j_T, \mathbf{W}) - y_{j,c} \big) \mathbf{x}^j_T.
\end{split} 
\end{align}

\paragraph{$L_2$-regularized MLR}

\begin{align}
\label{l2mlr}
\mathcal{L}_{L_2-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j_T, \mathbf{y}^j) + \lambda \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
%\mathcal{L}_{L_2-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j, \mathbf{y}_j) + \lambda \sum_
%{c=1}^C \| \mathbf{w}_c \|_2^2.
\end{align}

With Eqn~\ref{mlr_nll_grad}, for class $c$, the derivative of $\mathcal{L}_{L_2-MLR}$ with respect to $\mathbf{w}_c$ is
\begin{align}
\label{l2mlr_soln_1}
\begin{split}
\frac{\partial \mathcal{L}_{L_2-MLR}}{\partial \mathbf{w}_c} & = \sum_{j=1}^n \big( Pr(y_{j,c}=1|\mathbf{x}^j_T, \mathbf{W}) - y_{j,c} \big) \mathbf{x}^T_t + 2 \lambda \, \mathbf{w}_c \\
& = \mathbf{X}^T (\bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c) + 2 \lambda \, \mathbf{w}_c,
\end{split}
\end{align}
%where $\bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) = \left[ Pr(y_{1,c}=1|\mathbf{x}^1_T, \mathbf{W}), Pr(y_{2,c}=1|\mathbf{x}^2_T, \mathbf{W}), \cdots, Pr(y_{n,c}=1| \mathbf{x}^n_T, \mathbf{W}) \right]^T $
where $\bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) = \left[ Pr(y_{1,c}=1|\mathbf{x}^1_T, \mathbf{W}), \cdots, Pr(y_{n,c}=1| \mathbf{x}^n_T, \mathbf{W}) \right]^T $  
and $\mathbf{y}_c = \left[ y_{1,c}, y_{2,c}, \cdots , y_{n,c} \right]^T$. 

Note that Eqn~\ref{l2mlr_soln_1} has the similar form as in the binary case in Eqn~\ref{l2lr_soln_1}, i.e., transposed data times an error term. By setting it to zero, for each class $c$ and each feature $\mathbf{x}_i$, we can estimate $\lambda$ as 
\begin{align}
\label{l2mlr_soln_2}
\hat{\lambda}^{(i,c)}_{L_2-MLR} = - \frac{\langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle }{2 w_{i,c}}.
\end{align}

% \paragraph{$L_1$-regularized MLR}

% \begin{align}
% \label{l1mlr}
% \mathcal{L}_{L_1-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j,\mathbf{y}^j) + \lambda \| \mathbf{W} \|_1.
% %\mathcal{L}_{L_1-MLR}(\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};\mathbf{x}^j,\mathbf{y}_j) + \lambda \sum_{c=1} \| \mathbf{w}_c \|_1.
% \end{align}

% Similarly with $L_2$-regularized MLR, the gradient of $\mathcal{L}_{L_1-MLR}$ with respect to $\mathbf{w}_c$ is given by
% \begin{align}
% \label{l1mlr_soln_1}
% \frac{\partial \mathcal{L}_{L_1-MLR}}{\partial \mathbf{w}_c} = \mathbf{X}^T (\bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c) + \lambda \, \partial_{\mathbf{w}_c} \| \mathbf{w}_c \|_1. 
% \end{align}

% Setting $\partial_{\mathbf{w}_c} \mathcal{L}_{L_1-MLR}=0$ and considering the non-differentiability of $\| \mathbf{w}_c \|_1$, we estimate $\lambda$ for each feature $\mathbf{x}_i$ and nonzero $w_{i,c}$ as 
% \begin{align}
% \label{l1mlr_soln_2}
% \hat{\lambda}^{(i,c)}_8 = 
% \begin{cases}
% - \langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle & \text{if } w_{i,c} > 0 \\
%  \langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle & \text{if } w_{i,c} < 0 \\
% \end{cases}
% \end{align}

\textbf{Linear Support Vector Classification}

We define the objective function of binary linear support vector classification (BLSVC) as follows:
\begin{align}
\label{hl_bsvc}
\mathcal{L}_{BLSVC}(C, \mathbf{w}) = C \sum_{j=1}^n L_{HL}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2, 
\end{align}
where $L_{HL}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle)$ is the \textbf{hinge loss} for predicting $\mathbf{x}^j_T$. 

In practice, there are two commonly used hinge loss functions, i.e., regular hinge loss (RHL) and squared hinge loss (SHL).  

\textbf{Regular hinge loss (RHL):} $L_{RHL}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) = \max(0, 1 - y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle)$. Figure~\ref{XX} shows its function as well as squared hinge loss. Note that RHL is convex, but non-differential when $y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle = 1$. Its subgradient with respect to $\mathbf{w}$ is 
% Once again, it is non-differential because of the \textbf{max} term. However, by introducing slack variables $\xi_i$, one can show that it is equivalent to solving
% \begin{align}
% \begin{split}
% & \mathcal{L}_{HL-SVM}(C, \mathbf{w}, \bm{\xi}) = C \sum_{j=1}^n \xi_j + \frac{1}{2} \| \mathbf{w} \|^2 \\
% & \text{s.t. } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle \geq 1 - \xi_i, \xi_i \geq 0, \forall i. 
% \end{split}
% \end{align}
%because of the ``max term". Its subgradient with respect to $\mathbf{w}$ is 
\begin{align}
\label{RHL_subg}
\frac{\partial L_{RHL}}{\partial \mathbf{w}} = 
\begin{cases}
-y_j \mathbf{x}^j_T & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1 \\
[-y_j \mathbf{x}^j_T, \mathbf{0}] & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle = 1 \\
\mathbf{0} & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle > 1
\end{cases}
\end{align}

In practice, for non-differential point, its subgradient is set to be 0. Therefore, with Eqn~\ref{RHL_subg}, we can estimate the hyperparamter $C$ using only samples $\mathbf{x}^j$ that satisfy $y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1$. Setting the derivative of $\mathcal{L}_{BLSVC}$ with respect to $w_i$ to zero yields
\begin{align}
\hat{C}^{(i)}_{BLSVC-RHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1} y_j {x}_{j,i}}. 
%C \sum_{j,y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1} -y_j \mathbf{x}^j + \mathbf{w} = 0, \quad \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1.
%C \sum_{j=1}^n -y_j \mathbf{x}^j + \mathbf{w} = 0, \quad \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle < 1.
\end{align} 

\textbf{Squared Hinge Loss (SHL):} $L_{SHL}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) = \max(0, 1 - y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle)^2$. SHL is convex, smooth, and differential. Its subgradient with respect to $\mathbf{w}$ is given by
\begin{align}  
\label{SHL_subg}
\frac{\partial L_{SHL}}{\partial \mathbf{w}} =
\begin{cases}
-2 y_j \mathbf{x}^j_T (1 - y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle) & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle <= 1 \\
\mathbf{0}  & \text{if } y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle > 1
\end{cases}
\end{align}

Therefore, taking the derivative of $\mathcal{L}_{BLSVC}$ with respect to $w_i$ to zero in this case  yields
\begin{align}
\hat{C}^{(i)}_{BLSVC-SHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle \leq 1} 2y_j {x}_{j,i} (1 - y_j \langle \mathbf{w}, \mathbf{x}^j_T \rangle) }. 
\end{align}

For multi-class LSVC, it can be derivated from binary LSVC in a one-vs-one or one-vs-rest fashion [2]. In this setting, we can run binary classification Eqn~\ref{hl_bsvc} $K \times (K-1)/2 $ and $K$ times to estimate the hyperparater.


% \subsubsection{Multi-Class LSVC}

% Normally, binary LSVC is extended to multi-class linear SVC in a one-vs-one or one-vs-rest fashion [2]. In this setting, we can run binary classification Eqn~\ref{hl_bsvc} $K \times (K-1)/2 $ and $K$ times to estimate the hyperparater. However, there exists a ``true" multi-class version hinge loss (MHL) for multi-class SVC, due to Crammer and Singer [3], which optimizes a joint objective over all classes and is defined as
% \begin{align}
% \label{crammer_singer_msvc}
% \begin{split}
% & \min_{\mathbf{W},\epsilon} \quad \mathcal{L}_{MSVC}(C, \mathbf{W}) =  C \sum_{j=1}^n \epsilon_j + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2 \\
% & \text{s.t.} \quad	\langle \mathbf{w}_{y_j}, \mathbf{x}^j_T  \rangle - \langle \mathbf{w}_c, \mathbf{x}^j_T  \rangle  \geq e_j^c - \epsilon_j \\
% & \quad \quad \epsilon_j \geq 0, \, j=1,\cdots, n; \, c=1, \cdots, C, 
% \end{split}
% \end{align}
% where $e_j^c = 0$ if $y_j = c$, and $e_j^c = 1$ if $y_j \neq c$ and $\mathbf{W} = \left[ \mathbf{w}_1, \mathbf{w}_2, \cdots, \mathbf{w}_C \right]$. 

% The decision function to predict the label of a new instance $\mathbf{x}$ is $\argmax\nolimits_{c=1,\cdots,C} \langle \mathbf{w}_c, \mathbf{x} \rangle $.

% Directly setting the derivative of $\mathcal{L}_{MSVC}$ for $\mathbf{w}_c$ via Eqn~\ref{crammer_singer_msvc} in a constrainted form is difficult. Therefore, we transform it to the equivalent unconstrained form as follows
% % \begin{align}
% % \mathcal{L}_{MSVC}(C, \mathbf{W}) = C \sum_{j=1}^n \sum_{c \neq y_j} L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2,
% % \end{align}
% \begin{align}
% \mathcal{L}_{MSVC}(C, \mathbf{W}) = C \sum_{j=1}^n L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2,
% \end{align}
% where $L_{MHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle) = \max(0, 1 + \max\nolimits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle)$ is the maximal hinge loss among $C$ classes for predicting $\mathbf{x}^j$. 

% % Similarly, there are also two MHL functions, i.e., regular MHL and squared MHL. 

% % \textbf{Regular multi-class hinge loss (RMHL):} $L_{RMHL}(y_j, \langle \mathbf{w}_c, \mathbf{x}^j \rangle) = \max(0, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}_j \rangle)$. 

% %Therefore, the objective function in this setting becomes
% In this way, the objective function then becomes
% \begin{align}
% \mathcal{L}_{MSVC}(C, \mathbf{w}) = C \sum_{j=1}^n \max(0, 1 + \max_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
% \end{align}

% Its subgradient with respect to $\mathbf{w}_c$ is 
% \begin{align}
% \frac{\partial MSVC}{\partial \mathbf{w}_c} =
% \begin{cases}
% C \sum\limits_{j=1}^n \mathbf{x}^j_T + \mathbf{w}_c & \text{if } 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle > 0 \\
% \mathbf{0} & \text{if } 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle < 0
% \end{cases}
% \end{align}

% % \begin{align}
% % \mathcal{L}_{MSVC}(C, \mathbf{w}) = C \sum_{j=1}^n \sum_{c \neq y_j} \max(0, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle) + \frac{1}{2} \sum_{c=1}^C \| \mathbf{w}_c \|_2^2.
% % \end{align}

% % Its subgradient with respect to $\mathbf{w}_c$ is 
% % \begin{align}
% % \frac{\partial MSVC}{\partial \mathbf{w}_c} =
% % \begin{cases}
% % C \sum_{j=1}^n \mathbf{x}^j + \mathbf{w}_c & \text{if } 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle > 0 \\
% % \mathbf{0} & \text{if } 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle < 0
% % \end{cases}
% % \end{align}

% Setting it to zero, we have 
% % \begin{align}
% % \hat{C}^{(i,c)} = - \frac{w_{i,c}}{\sum\limits_{j, 1 + \langle \mathbf{w}_c, \mathbf{x}^j \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j \rangle > 0} x_{j,i}}. 
% % \end{align}
% \begin{align}
% \hat{C}^{(i,c)} = - \frac{w_{i,c}}{\sum\limits_{j, 1 + \max\limits_{c \neq y_j} \langle \mathbf{w}_c, \mathbf{x}^j_T \rangle - \langle \mathbf{w}_{y_j}, \mathbf{x}^j_T \rangle > 0} x_{j,i}}. 
% \end{align}


\subsubsection{Nonlinear model-based classification}

\textbf{Kernel Logistic Regression}

\textbf{Case 1: Binary KLR}

Binary kernel logistic regression (BKLR) is to minimize the following nonegative log-likelihood
\begin{align}
\label{klr_nll}
\begin{split}
& \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}),y) = - \log Pr(y|\phi(\mathbf{x}), \mathbf{w}^\prime) \\
& \qquad = - \big( y \, \log h_{\mathbf{w}^\prime}(\phi(\mathbf{x})) + (1-y) \log (1- h_{\mathbf{w}^\prime}(\phi(\mathbf{x}))) \big)
%\text{NLL}(\mathbf{w};\mathbf{x},y) = - \log Pr(y|\mathbf{x}, \mathbf{w}) = - \big( y \, \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle) + (1-y) (1- \text{sigm}(\langle \mathbf{w}, \mathbf{x} \rangle)) \big). 
\end{split}
\end{align}
%where $h_{\mathbf{w}^\prime}(\phi(\mathbf{x}))) = \frac{1}{1+\exp(\langle \bm{\alpha}, \rangle)}$ 

\paragraph{$L_2$-regularized BKLR}

% Minimize the following 
\begin{align}
\label{l2klr_primal}
\mathcal{L}_{L_2-BKLR}(\lambda, \mathbf{w}^\prime) = \sum_{j=1}^n \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}^j_T),y_j) + \lambda \| \mathbf{w}^\prime \|_2^2.
%\mathcal{L}_{L_2-BLR}(\lambda, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}^j_T) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] + \lambda \| \mathbf{w} \|_2^2,
\end{align}
%where $h_\mathbf{w}(\mathbf{x}^j_T) = \text{sigm}(\mathbf{w}^T \mathbf{x}^j) = \frac{1}{1+\exp(-\mathbf{w}^T \mathbf{x}^j)}$.

Using $\mathbf{w}^\prime = \Phi(\mathbf{X})^T \bm{\alpha}$, we have
\begin{align}
\label{l2klr_dual}
\begin{split}
& \mathcal{L}_{L_2-BKLR}(\lambda, \bm{\alpha}) 
= \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha} \\
& = \sum_{j=1}^n - \big( y_j \, \log h_{\bm{\alpha}}(\mathbf{k}_j) + (1 - y_j) (1- h_{\bm{\alpha}}(\mathbf{k}_j)) \big) + \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha},
\end{split}
\end{align} 
where $h_{\bm{\alpha}}(\mathbf{k}_j) = \frac{1}{1 + \exp{\langle \bm{\alpha}, \mathbf{k}_j \rangle}}$

Similarly with binary logistic regression, the gradient of $\mathcal{L}_{L_2-BKLR}$ with respect to $\bm{\alpha}$ is given by
\begin{align}
\label{l2klr_soln_1}
\begin{split}
\frac{\partial \mathcal{L}_{L_2-BKLR}}{\partial \bm{\alpha}}
& = \sum_{j=1}^n (h_{\bm{\alpha}}(\mathbf{k}_j) - y_j) \mathbf{k}_j + 2 \lambda \mathbf{K} \bm{\alpha} \\
& = \mathbf{K} (h_{\bm{\alpha}}(\mathbf{K}) - \mathbf{y}) + 2 \lambda \mathbf{K} \bm{\alpha} \\
& = \mathbf{K} (h_{\bm{\alpha}}(\mathbf{K}) - \mathbf{y} + 2 \lambda \bm{\alpha})
\end{split}
\end{align}
where we use $\mathbf{K}^T = \mathbf{K}$ and $h_{\bm{\alpha}}(\mathbf{K}) = \left[ h_{\bm{\alpha}}(\mathbf{k}_1), \cdots, h_{\bm{\alpha}}(\mathbf{k}_n) \right]^T \in \mathbb{R}^n$.

Given $\bm{\alpha}$, we set $\partial_{\bm{\alpha}} \mathcal{L}_{L_2-BKLR} = \mathbf{0}$ and consider that $\mathbf{K}$ is full rank, we thus have $h_{\bm{\alpha}}(\mathbf{K}) - \mathbf{y} + 2 \lambda \bm{\alpha} = \mathbf{0}$. For each $\alpha_i$, we then estimate $\lambda$ as
\begin{align}
\label{l2klr_soln_2}
\hat{\lambda}^{(j)}_{L_2-BKLR} = - \frac{h_{\bm{\alpha}}(\mathbf{k}_j) - y_j} {2 \alpha_j}.
\end{align}

\paragraph{$L_1$-regularized BKLR}

\begin{align}
\label{l1klr_primal}
\mathcal{L}_{L_1-BKLR}(\lambda, \mathbf{w}^\prime) = \sum_{j=1}^n \text{NLL}_{BKLR}(\mathbf{w^\prime};\phi(\mathbf{x}^j_T),y_j) + \lambda \| \mathbf{w}^\prime \|_1.
%\mathcal{L}_{L_2-BLR}(\lambda, \mathbf{w}) = - \sum_{j=1}^n \left[ y_j \log h_\mathbf{w}(\mathbf{x}^j_T) + (1-y_j) \log(1-h_\mathbf{w}(\mathbf{x}^j_T)) \right] + \lambda \| \mathbf{w} \|_2^2,
\end{align}

Using $\mathbf{w}^\prime = \Phi(\mathbf{X})^T \bm{\alpha}$, we have
\begin{align}
\begin{split}
\label{l1klr_dual}
\mathcal{L}_{L_1-BKLR}(\lambda, \bm{\alpha}) & = - \sum_{j=1}^n \big( y_j \, \log h_{\bm{\alpha}}(\mathbf{k}_j) + (1 - y_j) (1- h_{\bm{\alpha}}(\mathbf{k}_j)) \big) \\ 
& + \lambda \| \mathbf{K} \bm{\alpha} \|_1. 
\end{split}
\end{align} 

The subderivative of the second term for $\bm{\alpha}$ is
\begin{align}
\begin{split}
\frac{\partial \| \mathbf{K} \bm{\alpha} \|_1 }{\partial \bm{\alpha}} & = \frac{\partial \| \mathbf{K} \bm{\alpha} \|_1 }{\partial \mathbf{K} \bm{\alpha}} \frac{\partial \mathbf{K} \bm{\alpha}}{\partial \bm{\alpha}} = \frac{\bm{\alpha}^T \mathbf{K}^T }{\bm{\alpha}} \textbf{sign}(\mathbf{K} \bm{\alpha}) \\ 
& =  \mathbf{K}^T \textbf{sign}(\mathbf{K} \bm{\alpha}) = \mathbf{K} \textbf{sign}(\mathbf{K} \bm{\alpha}),
\end{split}
\end{align} 
where $\textbf{sign}(\mathbf{K} \bm{\alpha}) = \left[ \text{sign}(\mathbf{k}^1\bm{\alpha});  \text{sign}(\mathbf{k}^2\bm{\alpha}); \cdots; \text{sign}(\mathbf{k}^n\bm{\alpha}) \right]$ is the sign vector of $\mathbf{K} \bm{\alpha}$. 

Therefore, the subderivative of $\mathcal{L}_{L_1-BKLR}$ for $\bm{\alpha}$ is given by
\begin{align}
\frac{\partial \mathcal{L}_{L_1-BKLR}}{\partial \bm{\alpha}} = \mathbf{K} (h_{\bm{\alpha}}(\mathbf{K}) - \mathbf{y} + \lambda \textbf{sign}(\mathbf{K} \bm{\alpha})).
\end{align}

By setting it to $\mathbf{0}$, we estimate $\lambda$ as 
\begin{align}
\hat{\lambda}^{(j)}_{L_1-BKLR} = 
\begin{cases}
 y_j - h_{\bm{\alpha}}(\mathbf{k}_j)  & \text{if } \mathbf{k}^j \bm{\alpha} > 0 \\
 h_{\bm{\alpha}}(\mathbf{k}_j) - y_j  & \text{if } \mathbf{k}^j \bm{\alpha} < 0
\end{cases}
\end{align} 


\textbf{Case 2: Multi-Class KLR}

We now consider multi-class kernel logistic regression (MKLR). Using one-of-$C$ code to represent each label $\mathbf{y}$ and Mercer's Theorem, the nonnegative log-likelihood of MKLR for $C$-class is defined as 
\begin{align}
\begin{split}
& \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) = - \sum_{j=1}^N \sum_{c=1}^C y_{j,c} \log Pr(y_{j,c}=1 | \mathbf{k}_j, \bm{\Omega}) \\ 
& \qquad = - \sum_{j=1}^N \bigg( \sum_{c=1}^C y_{j,c} \langle \bm{\alpha}_c, \mathbf{k}_j \rangle + \log \big( \sum_{c^\prime=1}^C \exp (\langle \bm{\alpha}_{c^\prime}, \mathbf{k}_j \rangle) \big) \bigg), 
\end{split}
\end{align}
where $\bm{\Omega} = \left[ \bm{\alpha}_1, \bm{\alpha}_2, \cdots, \bm{\alpha}_C \right]$.

The objective function of $L_2$-regularized MKLR is 
\begin{align}
\mathbf{L}_{L_2-MKLR}(\lambda, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + \lambda \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c.  
\end{align}
and its derivative of $\bm{\alpha}_c$ is given by
\begin{align}
\frac{\partial \mathbf{L}_{L_2-MKLR}}{\partial \bm{\alpha}_c} = \mathbf{K} (\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) - \mathbf{y}_c + 2 \lambda \bm{\alpha}_c),
\end{align}
where $\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) = \left[ Pr(y_{1,c}=1 | \mathbf{k}_1, \bm{\Omega}), \cdots, Pr(y_{1,c}=n | \mathbf{k}_n, \bm{\Omega}) \right]$.
% where $\bm{\mu}_{c, \bm{\Omega}}(\mathbf{K}) = \left[ Pr(y_{1,c}=1 | \mathbf{k}_1, \bm{\Omega}), Pr(y_{2,c}=1 | \mathbf{k}_2, \bm{\Omega}), \cdots, Pr(y_{1,c}=n | \mathbf{k}_n, \bm{\Omega}) \right]$.

By setting it to zero, for each class $c$ we can estimate $\lambda$ as
\begin{align}
\hat{\lambda}^{(j,c)}_{L_2-MKLR} = \frac{y_{j,c} - \bm{\mu}_{c, \bm{\Omega}}(\mathbf{k}_j)}{2 \alpha_{j,c}}.
\end{align}




\subsection{Kernel Support Vector Classification}

\subsubsection{Binary KSVC}

\begin{align}
\label{kernel_bsvc_prime}
\mathcal{L}_{BKSVC}(C, \mathbf{w^\prime})  = C \sum_{j=1}^n L_{HL}(y_j, \langle \mathbf{w^\prime}, \phi(\mathbf{x}^j_T) \rangle) + \frac{1}{2} \| \mathbf{w^\prime} \|_2^2 
\end{align}

Again using Mercer’s Theorem, we adopt dual variables $\bm{\alpha}$ to represent primal variables $\mathbf{w}^\prime$, and transform Eqn~\ref{kernel_bsvc_prime} as follows
\begin{align}
\label{kernel_bsvc_dual}
\begin{split}
\mathcal{L}_{BKSVC}(C, \bm{\alpha}) & = C \sum_{j=1}^n L_{HL}(y_j, \langle \Phi(\mathbf{X})^T \bm{\alpha}, \phi(\mathbf{x}^j_T) \rangle) + \frac{1}{2} \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
& = C \sum_{j=1}^n L_{HL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha}.
\end{split}
\end{align}
% where $L_{HL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle )$.

\textbf{Regular hinge loss (RHL):} $L_{RHL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )$.

Similarly with binary linear SVC, taking the subderivative of $\mathcal{L}_{BKSVC}$ for $\bm{\alpha}$, and setting it to $\mathbf{0}$, we estimate $C$ for each $\alpha_i$ as 
\begin{align}
\label{kernel_bsvc_rhl_soln}
\hat{C}^{(i)}_{BKSVC-RHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j, y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle <1} y_j k_{j,i}}.
\end{align} 

\textbf{Squared Hinge Loss (SHL):} $L_{SHL}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )^2$. We take the derivative of $\mathcal{L}_{BKSVC}$ for $\bm{\alpha}$, and set it to $\mathbf{0}$, 
\begin{align}
\label{kernel_bsvc_shl_soln}
\hat{C}^{(i)}_{BKSVC-SHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle \leq 1} 2y_j {k}_{j,i} (1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle)}. 
\end{align}

% \subsubsection{Multi-Class KSVC}

==> defense_res.tex <==
\subsection{Experimental Results}

\subsubsection{Experimental Setup} 

We evaluate hyperparameter defense capability by leveraging the rounding technique and analyze hyperparameter sensitivity of all above ML methods on several datasets. 

First, we randomly split each dataset into the training set with proportion $2/3$ and testing set with proportion $1/3$. 
Then, we use default optimization algorithms in Table~\ref{opt_alg} and 5-fold CV to learn the optimal model parameters and hyperparameters of each model using the training set. After that, we steal each model's hyperparameter as done in previous Section.

To globally perform defense against hyperparameter stealing, we round decimals and keep its number from 1 to 5, respectively. We take the metric average relative $\gamma$-hyperparameter error measured on the training set and relative $\delta$-MSE (or relative $\delta$-ACC error) measured on the testing set to quantify defense capability. Furthermore, to locally analyze the sensitivity of each hyperparameter estimated by the respective parameter, we adopt the metric $\theta$-hyperparameter sensitivity. Our defense strategy and sensitive analysis are implemented using Python. 

%To defense hyperparameter stealing, we round decimals and keep its number from 1 to 5. Specifically, we use the default optimization algorithm in Table~\ref{opt_alg} and 5-fold CV to learn the optimal model parameters and hyperparameters. 
%We use the metric average relative $\gamma$-hyperparameter error and relative $\delta$-MSE (or relative $\delta$-ACC error) to quantify defense capability. 

\subsubsection{Hyperparameter Defense Results}

% \begin{figure*}
% \center
% \subfigure[Diabetes]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/reg/result-reg-diabetes-new.pdf}\label{diabetes_defense}} 
% \subfigure[GeoOrigin]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/reg/result-reg-geo-origin-new.pdf}\label{geoorigin_defense}}
% \subfigure[UJIIndoor]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/reg/result-reg-indoorLoc-new.pdf}\label{ujiindoor_defense}}
% \caption{Hyperparameter defense results of regression models.}
% \label{reg_res_defense}
% \end{figure*}

% \begin{figure*}
% \center
% \subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-lr-madelon-new-new.pdf}\label{clf_lr_madelon_defense}} 
% \subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-svc-madelon-new-new.pdf}\label{clf_svc_madelon_defense}}
% \subfigure[Digits]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-mlr-digits-new-new.pdf}\label{clf_mlr_digits_defense}} 
% \caption{Hyperparameter defense results of classification models on Madelon and Digits.}
% \label{clf_res_defense}
% \end{figure*}

\begin{figure}
\center
\label{clf_lr_res_defense}
\subfigure[Iris]{\includegraphics[width=0.23\textwidth]{../src_defense/figs/clf/result-clf-lr-iris-new-new.pdf}\label{lr_iris_defense}} 
\subfigure[Ionosphere]{\includegraphics[width=0.23\textwidth]{../src_defense/figs/clf/result-clf-lr-ionosphere-new-new.pdf}\label{lr_ionosphere_defense}}
%\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-lr-madelon-new-new.pdf}\label{lr_madelon_defense}} 
\caption{Hyperparameter defense results of BLR-based methods.}
\end{figure}

% \begin{figure*}
% \center
% \label{clf_mlr_res_defense}
% \subfigure[Iris]{\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-mlr-iris-new-new.pdf}\label{mlr_iris_defense}} 
% \subfigure[Digits]{\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-mlr-digits-new-new.pdf}\label{mlr_digits_defense}}
% \caption{Hyperparameter defense results of multi-class LR-based classification models.}
% \end{figure*}


\begin{figure}
\center
\label{clf_svc_res_defense}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-svc-iris-new-new.pdf}\label{svc_iris_defense}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-svc-ionosphere-new-new.pdf}\label{svc_ionosphere_defense}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-svc-madelon-new-new.pdf}\label{svc_ionosphere_defense}} 
\caption{Hyperparameter defense results of SVC-based methods.}
\end{figure}


The defense results of regression methods on Diabetes, GeoOrigin, and UJIndoorLoc, are shown in Fig.~\ref{reg_res_defense}. As can be seen, by rounding decimals, all methods can still maintain performance with relative MSE less than 1\% on all datasets. However, as a whole, RR has the largest average relative $\gamma$-hyperparameter error, and is followed by KRR and $L_2$ regularization of ENet. LASSO and $L_1$ regularization of ENet are very stable. Therefore, we can conclude that RR, KRR, and $L_2$ regularization of ENet are more secure than LASSO and $L_1$ regularization of ENet.  

The results of binary LR-based and SVC-based classification models on Madelon and multiple LR-based models on Digits are shown in Fig.~\ref{clf_res_defense} (Due to space limitation, we leave results on the other datasets in Appendix). 
Similarly, all methods can achieve relative ACC error less than 1\%. However, we observe that the average relative $\gamma$-hyperparameter error of L2-BLR and L2-BKLR is larger than that of L1-BLR and L1-BKLR; BLSVC-SHL and BKSVC-SHL is larger than that of BLSVC-RHL and BKSVC-RHL, which indicates that the former two methods are more secure than the latter two. In addition, L2-MLR and L2-MKLR have an approximate 5\%- and 23\%-hyperparameter error when only 1 decimal is kept.  

% \subsubsection{Hyperparameter Sensitivity Results}

% % \begin{figure*}
% % \center
% % \subfigure[Diabetes]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/reg/result-reg-diabetes.pdf}\label{diabetes_defense}} 
% % \subfigure[GeoOrigin]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/reg/result-reg-geo-origin.pdf}\label{geoorigin_defense}}
% % \subfigure[UJIIndoor]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/reg/result-reg-indoorLoc.pdf}\label{ujiindoor_defense}}
% % \label{reg_res_sensi}
% % \caption{Hyperparameter sensitivity results of regression models.}
% % \end{figure*}

% \begin{figure}
% \center
% \subfigure[Iris]{\includegraphics[width=0.23\textwidth]{../src_sensitivity/figs/clf/result-clf-lr-iris.pdf}\label{lr_iris_sensi}} 
% \subfigure[Ionosphere]{\includegraphics[width=0.23\textwidth]{../src_sensitivity/figs/clf/result-clf-lr-ionosphere.pdf}\label{lr_ionosphere_sensi}}
% %\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-lr-madelon.pdf}\label{lr_madelon_sensi}} 
% \label{clf_lr_res_sensi}
% \caption{Hyperparameter sensitivity results of BLR methods.}
% \end{figure}


% \begin{figure}
% \center
% \subfigure[Iris]{\includegraphics[width=0.23\textwidth]{../src_sensitivity/figs/clf/result-clf-klr-iris.pdf}\label{klr_iris_sensi}} 
% \subfigure[Ionosphere]{\includegraphics[width=0.23\textwidth]{../src_sensitivity/figs/clf/result-clf-klr-ionosphere.pdf}\label{klr_ionosphere_sensi}}
% %\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-klr-madelon.pdf}\label{klr_madelon_sensi}} 
% \label{clf_klr_res_sensi}
% \caption{Hyperparameter sensitivity results of BKLR methods.}
% \end{figure}


% \begin{figure}
% \center
% \subfigure[Iris]{\includegraphics[width=0.23\textwidth]{../src_sensitivity/figs/clf/result-clf-svc-iris.pdf}\label{svc_iris_sensi}} 
% \subfigure[Ionosphere]{\includegraphics[width=0.23\textwidth]{../src_sensitivity/figs/clf/result-clf-svc-ionosphere.pdf}\label{svc_ionosphere_sensi}}
% %\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-svc-madelon.pdf}\label{svc_madelon_sensi}} 
% \label{clf_svc_res_sensi}
% \caption{Hyperparameter sensitivity results of BLSVC methods.}
% \end{figure}

% \begin{figure}
% \center
% \subfigure[Iris]{\includegraphics[width=0.23\textwidth]{../src_sensitivity/figs/clf/result-clf-ksvc-iris.pdf}\label{ksvc_iris_sensi}} 
% \subfigure[Ionosphere]{\includegraphics[width=0.23\textwidth]{../src_sensitivity/figs/clf/result-clf-ksvc-ionosphere.pdf}\label{ksvc_ionosphere_sensi}}
% %\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-ksvc-madelon.pdf}\label{ksvc_madelon_sensi}} 
% \label{clf_ksvc_res_sensi}
% \caption{Sensitivity analysis results of BKSVC methods.}
% \end{figure}


% The sensitive results of regression methods on Diabetes, GeoOrigin, and UJIndoorLoc, are shown in Fig.~\ref{reg_res_sensi}.

% \subsection{Real-world Deployment}

% Due to space limitation, we only show results of XXX.
  
% Regression results for cloud-based services:

% \begin{figure}
% \center
% \label{real_defense}
% \includegraphics[width=0.45\textwidth]{../src_time/figs/result-UJIndoorLoc-ridge-defense-m1-m3.pdf}\label{ridge_defense_m1_m3} 
% %\subfigure[LASSO]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-UJIndoorLoc-Lasso-defense-m1-m3.pdf}\label{lasso_defense_m1_m3}}
% \caption{Relative MSE of RR under defense on UJIndoorLoc dataset.}
% \end{figure}

% Classification results for cloud-based services:

% \begin{figure*}
% \center
% \label{real_defense}
% \subfigure[L2-BLR]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-bank-lr-defense-m1-m3.pdf}\label{lr_defense_m1_m3}} 
% \subfigure[BLSVC-SHL]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-bank-svc-defense-m1-m3.pdf}\label{svc_defense_m1_m3}}
% \caption{Relative ACC error of L2-BLR and BLSVC-SHL under defense on Bank dataset.}
% \end{figure*}


==> discussion.tex <==
\section{Discussions and Limitations}
\label{discussion}

%\subsection{Discussion}


% \begin{figure}[!t]
% %\vspace{-4mm}
% \center
% {\includegraphics[width=0.35\textwidth]{./src_attack/figs/reg/result-reg-diabetes-final.pdf}\label{reg_diabetes}} 
% \caption{Effectiveness of our hyperparameter stealing attacks when model parameters are unknown but stolen by model parameter stealing attacks. %(Change y-axis to be``Relative estimation error (log10)")
% }
% \label{modelparameterunknown}
% \vspace{-2mm}
% \end{figure}

\alan{
\noindent
{\bf Assumptions for our Train-Steal-Retrain strategy:} A user of an MLaaS platform can benefit from our Train-Steal-Retrain strategy when the following assumptions hold:  1) the hyperparameters can be accurately learnt using a small fraction of the training dataset; 2) the user does not have enough computational resource or ML expertise to learn the hyperparameters locally; and 3) training both the hyperparameters and model parameters using a small fraction of the training dataset does not lead to an accurate model. The validity of the first and third assumptions is data-dependent. % i.e., a user can benefit from our Train-Steal-Retrain strategy when the user's dataset satisfies the two assumptions. 
We note that  Train-Steal-Retrain requires ML expertise, but an attacker can develop it as a service for non-ML-expert users to use. 
}

\noindent
{\bf ML algorithm is unknown:} When the ML algorithm is unknown, 
 the problem becomes jointly stealing the ML algorithm and the hyperparameters. Our current attack is defeated in this scenario. In fact, jointly stealing the ML algorithm and the hyperparameters may be impossible in some cases. For instance, logistic regression with a hyperparameter $A$ produces a model $M_A$. On the same training dataset, SVM with a hyperparameter $B$ produces a model $M_B$. If the model parameters $M_A$ and $M_B$ are the same, we cannot distinguish between the logistic regression with hyperparameter $A$ and the SVM with a hyperparameter $B$. It is an interesting future work to study jointly stealing ML algorithm and hyperparameters, e.g., show when it is possible and impossible to do so. %However, as shown in~\cite{tramer2016stealing}, the ML algorithms of several MLasS platforms are known. For instance, LR is employed by Microsoft, Google, BigML, and PredictionIO; SVM is employed by Microsoft, Google, and PredictionIO. 


\alan{
\noindent
{\bf Other types of hyperparameters:} As a first step towards stealing hyperparameters in machine learning, our work is limited to stealing the hyperparameters that are used to balance between the loss function and the regularization terms in an objective function. Many ML algorithms (please refer to Table~\ref{sum_ml}) rely on such hyperparameters. We note that some ML algorithms use other types of hyperparameters. For instance, $K$ is a hyperparameter for $K$ Nearest Neighbor; the number of trees is a hyperparameter for random forest; and architecture, dropout rate, learning rate, and mini-batch size are important hyperparameters for deep convolutional neural networks.  Modern deep convolutional neural networks use dropout~\cite{dropout} instead of conventional $L_1$/$L_2$ norm to perform regularization. 
%in the objective functions of ML algorithms and ML algorithms that are almost everywhere differentiable.  We note that some ML algorithms have non-differentiable objective functions, e.g., decision tree, $k$ nearest neighbor, and random forest. Moreover, some ML algorithms have other types of hyperparameters, e.g., dropout rate, learning rate, and mini-batch size when training neural networks. 
We believe it is an interesting future work to study hyperparameter stealing for these hyperparameters. 
}

\noindent
{\bf Other countermeasures:} It is an interesting future work to explore defenses other than rounding model parameters. For instance, like differentially private ML algorithms~\cite{chaudhuri2011differentially}, we could add noise to the objective function. %Moreover, we can add noise to the model parameters instead of rounding them. 

%In this work, our major goal is to show the feasibility of stealing hyperparameters in machine learning. For completeness, we also evaluated rounding as a defense technique. We found that rounding has negligible impact on testing performance of the model parameters, but it is not effective enough to defend against our hyperparameter stealing attacks for certain ML algorithms. It is an interesting future work to explore other defenses. For instance, like differentially private ML algorithms~\cite{chaudhuri2011differentially}, we can add noise to the objective function. Moreover, we can add noise to the model parameters instead of rounding them. 


%we use rounding as a countermeasure against our stealing hyperparameter attack, and show it is not effective enough for certain ML algorithms. Some other countermeasures, e.g., adding noise to the model parameters or adding noise to the objective function~\cite{chaudhuri2011differentially}, will be investigated in future work. 

%\subsection{Limitations}
%
%\myparatight{Not suitable for non-differentiable objective functions} This work focuses on stealing hyperparameters in ML algorithms whose objective functions are almost everywhere differentiable. Actually, there exists another type of ML algorithms whose objective functions are non-differentiable, e.g., decision tree, random forest, etc.. We acknowledge that our attack is not suitable for this type of ML algorithms. 
%
%\myparatight{Perhaps not suitable for deep neural network} Due to the highly nonlinear and nonconvex objective function,  deep neural network often exists a large amount of (even infinite) local minimums. In practice, training a general neural network model is NP-hard~\cite{blum1989training}. A surrogate is to leverage (stochastic) gradient descent to approximate the miminum. However, it has been empirically observed that this way of training a deep neural network often cannot reach a minimum~\cite{lecun1998gradient}. Note that our attack in this paper assumes that the model parameters learnt by a ML algorithm are often a minima of the respective objective function. In this sense, it may be not suitable for deep neural network.





==> exp.tex <==
\section{Experimental Results}

\subsection{Experimental Setups}

\begin{table}[!htp]
\centering
\caption{Selected UCI datasets for regression}
\label{data_reg}
\begin{tabular}{|c|c|c|c|}
\hline
 \textbf{Dataset} & \textbf{Instance} & \textbf{Feature} & \textbf{Year} \\ \hline
 \textbf{Diabetes} &  442 & 10 &  \\ \hline
% \textbf{Parkinson Speech} & 1040 & 26 & 2014 \\ \hline
% \textbf{Breast Cancer} &  568 & 32 & 1995 \\ \hline
 \textbf{GeoOrig} & 1059 & 68 & 2014 \\ \hline
% \textbf{TomHardWare} &  28197 & 96 &  2013 \\ \hline
% \textbf{Community \& Crime} & 1993 & 121 & 2009 \\ \hline
 \textbf{UJIIndoor} & 19937 & 529 & 2014 \\ \hline
\end{tabular}
\end{table}

% \begin{table*}[!htb]
% \centering
% \caption{Linear-based regression results on selected UCI datasets}
% \label{lin_reg_res}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{Ridge} & \multicolumn{2}{c|}{\textbf{LASSO}} & \multicolumn{2}{c|}{\textbf{ENet}} & \multicolumn{2}{c|}{\textbf{SVR}} \\ \cline{2-9} 
%                &    True  &       Est  &   True  &       Est &   True  &       Est  &   True   &   Est    \\ \hline
%   \textbf{Diabetes}                &    0.1       &   0.1$\pm$7e-14        &    0.001       &   0.001$\pm$6e-6        &  (1.326, 6.188)         &  (1.326, 6.186)         &   0.01        &    0.01$\pm$9e-5       \\ \hline
%   \textbf{Parkinson Speech}         &    0.1       &    0.1$\pm$8e-9       &    0.001       &    0.001$\pm$3e-6       &    (1029.600, 20.800)       &    (1029.595, 20.793)       &    0.01       &     0.01$\pm$2e-17      \\ \hline
%    \textbf{Breast Cancer}           &     0.1      &    0.1$\pm$2e-7       &   0.001        &   0.001$\pm$3e-5        &   (56.232, 1.136)        &   (56.159, 1.136)        &    0.01       &  0.01$\pm$8e-5         \\ \hline
%    \textbf{GeoOrig of Music}      &     0.1      &   0.1$\pm$1e-5        &     0.001      &    0.001$\pm$9e-6      &    (942.678, 19.044)       &   (942.677, 19.004)        &     0.01      &   0.01$\pm$3e-17        \\ \hline
%    %\textbf{TomHardWare}          &           &           &           &           &           &           &          0.001      &   0.001$\pm$3e-9           \\ \hline
%    \textbf{Community \& Crime}      &    0.1       &   0.1$\pm$1e-12        &     0.001      &     0.001$\pm$2e-7      &   (0.179, 0.0398)        &   (0.179, 0.0399)        &   0.01        &   0.01$\pm$2e-4        \\ \hline
%    \textbf{UJIIndoor}    &    0.1       &    0.1$\pm$7e-5       &    0.001       &   0.001$\pm$2e-5        &    (990.0, 20.0)       &  (991.328, 19.998)         &    0.01       &    0.01$\pm$5e-4       \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table}[!htb]
% \centering
% \caption{Kernel-based regression results on selected UCI datasets}
% \label{ker_reg_res}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{KernelRidge}} & \multicolumn{2}{c|}{\textbf{KernelSVR}} \\ \cline{2-5}
%  		&    						\textrm{True}         &   \textrm{Est}      &    \textrm{True}       &    \textrm{Est}       \\ \hline 
%   \textbf{Diabetes}         &      0.05     &   0.05$\pm$1e-13       &    0.001       &   0.001$\pm$1e-14        \\ \hline
%   \textbf{Parkinson Speech}   &     0.05      &  0.05$\pm$4e-13         &   0.001        &   0.001$\pm$2e-19        \\ \hline
%   \textbf{Breast Cancer}       &    0.05       & 0.05$\pm$7e-14          &  0.001         & 0.00099$\pm$4e-5         \\ \hline
%    \textbf{GeoOrig of Music}    &   0.05        &  0.05$\pm$3e-12         &  0.001         &  0.001$\pm$4e-19         \\ \hline
% %  \textbf{TomHardWare}           &  0.05         & 0.05$\pm$4e-9           &  0.001         & 0.00096$\pm$1e-4          \\ \hline
%   \textbf{Community \& Crime}     & 0.05          &  0.05$\pm$3e-12          &  0.001         & 0.001$\pm$4e-5          \\ \hline
%    \textbf{UJIIndoor}               &  0.05        &  0.05$\pm$4e-14          & 0.001          & 0.00098$\pm$1e-4          \\ \hline
                 
% \end{tabular}
% \end{table}


\begin{table}[!htp]
\centering
\caption{Selected UCI datasets for classification}
\label{data_clf}
\begin{tabular}{|c|c|c|c|}
\hline
 \textbf{Dataset} & \textbf{Instance} & \textbf{Feature} & \textbf{Type} \\ \hline
 \textbf{Iris} & 100 & 4 &  \textrm{Binary \& Multi-Class} \\ \hline
 \textbf{Ionosphere} & 351 & 34 & \textrm{Binary} \\ \hline
% \textbf{Sonar} & 208 & 60 &  \textrm{Binary}\\ \hline
% \textbf{Breast Cancer}& 569 & 30 & \textrm{Binary} \\ \hline
% \textbf{LSVT} & 125 & 310 & \textrm{Binary} \\ \hline
 \textbf{Madelon} & 4400 & 500 & \textrm{Binary} \\ \hline
 \textbf{Bank} & 45210 & 16 & \textrm{Binary} \\ \hline
 \textbf{Digit} & 1797 & 64 & \textrm{Multi-Class} \\ \hline
 \textbf{CovType} & 581012 & 54 & \textrm{Multi-Class} \\ \hline

\end{tabular}
\end{table}

% \begin{table*}[!htb]
% \centering
% \caption{Linear-based binary classification results on selected UCI datasets}
% \label{clf_res}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% 	\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{L$_2$-BLR}} & \multicolumn{2}{c|}{\textbf{L$_1$-LR}} & 
% 	\multicolumn{2}{c|}{\textbf{BLSVC-RHL}} & \multicolumn{2}{c|}{\textbf{BLSVC-SHL}}  \\ \cline{2-9} 
%            &    \textrm{True}       &   \textrm{Est}        &           \textrm{True}       &   \textrm{Est}     &          \textrm{True}       &   \textrm{Est}      &     \textrm{True}       &   \textrm{Est}           \\ \hline
%   \textbf{Iris}          &     1.0      &   1.0$\pm$6e-6        &   1.0        &   1.0$\pm$8e-5        &    0.01       &  0.01$\pm$3e-18         &    0.01       &  0.01$\pm$4e-9         \\ \hline
%   \textbf{Ionosphere}    &    100       &   100$\pm$0.2        &   10.0        &   10.0$\pm$2e-4        & 0.01           &    0.01$\pm$2e-3       &    0.01      &    0.01$\pm$1e-7        \\ \hline
%   \textbf{Sonar}         &    100       &    100$\pm$1e-1       &  2.0         &    2.00$\pm$3e-3       &           &           &     0.01      &   0.01$\pm$2e-7        \\ \hline
%   % \textbf{Breast Cancer}  &   10.0        &  9.98$\pm$8e-2         &       5.0    &  5.0$\pm$3e-2          &           &           &     0.0001      &   0.0001$\pm$3e-7        \\ \hline
%   % \textbf{LSVT}     &   50.0        &   49.66$\pm$06e-1        &     2.0      &   1.93$\pm$1e-2        &           &           &     0.001      &  0.001$\pm$1e-9         \\ \hline
%    \textbf{Madelon}   &   5.0        &   5.0$\pm$4e-4        &    2.0       &  2.0$\pm$3e-5          &    0.01       &   0.01$\pm$1e-3        &    0.001       &   0.001$\pm$8e-9        \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[!htb]
% \centering
% \caption{Kernel-based binary classification results on selected UCI datasets}
% \label{my-label}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{L$_2$-BKLR}} & \multicolumn{2}{c|}{\textbf{L$_1$-BKLR}} & \multicolumn{2}{c|}{\textbf{BKSVC-RHL}} & \multicolumn{2}{c|}{\textbf{BKSVC-SHL}} \\ \cline{2-9} 
% 		&    \textrm{True}       &   \textrm{Est}        &           \textrm{True}       &   \textrm{Est}          &  \textrm{True}       &   \textrm{Est}      &     \textrm{True}       &   \textrm{Est}           \\ \hline
%  \textbf{Iris}                 &    0.001       &    0.001$\pm$8e-6       &    0.001       &   0.001$\pm$1e-5        &     0.1      &  0.1$\pm$1e-17     &     0.01      &  0.01$\pm$3e-3         \\ \hline
%  \textbf{Ionosphere}         &     0.01      &  0.01$\pm$7e-4         &    0.001       &   0.001$\pm$6e-6        &   0.1        &   0.1$\pm$1e-17        &    0.01       &   0.01$\pm$1e-4        \\ \hline
%   \textbf{Sonar}      &    0.01       &   0.01$\pm$2e-4        &  0.0001         &  0.0001$\pm$2e-6         & 0.1           &   0.1$\pm$1e-17        &  0.01         &  0.01$\pm$5e-4         \\ \hline
%   \textbf{Madelon}      &  0.01         &  0.01$\pm$2e-5         &   0.001        &   0.001$\pm$9e-7        &    0.1       &    0.1$\pm$2e-4       &   0.01        &  0.01$\pm$5e-6         \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[!htb]
% \centering
% \caption{Multi-class classification results on selected UCI datasets}
% \label{my-label}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{L$_2$-MLR}} & \multicolumn{2}{c|}{\textbf{MLSVC-RHL}} & \multicolumn{2}{c|}{\textbf{L$_2$-MKLR}} & \multicolumn{2}{c|}{\textbf{MKSVC-RHL}} \\ \cline{2-9} 
% 	&    \textrm{True}       &   \textrm{Est}        &           \textrm{True}       &   \textrm{Est}          &  \textrm{True}       &   \textrm{Est}      &     \textrm{True}       &   \textrm{Est}           \\ \hline	
%  \textbf{Iris}                 &   50.0        &   50.0$\pm$9e-6        &           &           &     50.0      &   50.0$\pm$3e-3        &           &           \\ \hline
%  \textbf{Digits}                 &  5000.0         &  5000.0$\pm$9.3         &           &           &    50.0       &  50.0$\pm$0.69         &           &           \\ \hline
%                   &           &           &           &           &           &           &           &           \\ \hline
%                   &           &           &           &           &           &           &           &           \\ \hline
%                   &           &           &           &           &           &           &           &           \\ \hline
%                   &           &           &           &           &           &           &           &           \\ \hline
% \end{tabular}
% \end{table*}
\subsection{Attack Results}

% \begin{figure*}
% \center
% \subfigure[Diabetes]{\includegraphics[width=0.24\textwidth]{../src_attack/figs/reg/result-reg-diabetes-final.pdf}\label{reg_diabetes}} 
% \subfigure[Parkinson]{\includegraphics[width=0.24\textwidth]{../src_attack/figs/reg/result-reg-parkinson-final.pdf}\label{reg_parkinson}}
% \subfigure[GeoOrigin]{\includegraphics[width=0.24\textwidth]{../src_attack/figs/reg/result-reg-geo-origin-final.pdf}\label{reg_geoorigin}}
% \subfigure[UJIIndoor]{\includegraphics[width=0.24\textwidth]{../src_attack/figs/reg/result-reg-indoorLoc-final.pdf}\label{ujiindoor}}
% \caption{Hyperparameter stealing results of regression methods}
% \label{reg_res}
% \end{figure*}


\begin{figure*}
\center
\subfigure[Diabetes]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/reg/result-reg-diabetes-final.pdf}\label{reg_diabetes}} 
\subfigure[GeoOrigin]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/reg/result-reg-geo-origin-final.pdf}\label{reg_geoorigin}}
\subfigure[UJIIndoor]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/reg/result-reg-indoorLoc-final.pdf}\label{ujiindoor}}
\caption{Hyperparameter stealing results of regression methods}
\label{reg_res}
\end{figure*}


\begin{figure*}
\center
\label{clf_lr_res}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/clf/result-clf-lr-iris-new-final.pdf}\label{clf_lr_iris}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/clf/result-clf-lr-ionosphere-new-final.pdf}\label{clf_lr_ionosphere}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/clf/result-clf-lr-madelon-new-final.pdf}\label{clf_lr_madelon}} 
\caption{Hyperparameter stealing results of LR classification methods}
\end{figure*}

\begin{figure*}
\center
\label{clf_svc_res}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/clf/result-clf-svc-iris-new-final.pdf}\label{clf_svc_iris}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/clf/result-clf-svc-ionosphere-new-final.pdf}\label{clf_svc_ionosphere}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_attack/figs/clf/result-clf-svc-madelon-new-final.pdf}\label{clf_svc_madelon}} 
\caption{Hyperparameter stealing results of SVC classification methods}
\end{figure*}

\subsection{Defense Results}

% \begin{figure*}
% \center
% \subfigure[Diabetes]{\includegraphics[width=0.24\textwidth]{../src_defense/figs/reg/result-reg-diabetes-new.pdf}\label{diabetes_defense}} 
% \subfigure[Parkinson]{\includegraphics[width=0.24\textwidth]{../src_defense/figs/reg/result-reg-parkinson-new.pdf}\label{parkinson_defense}}
% \subfigure[GeoOrigin]{\includegraphics[width=0.24\textwidth]{../src_defense/figs/reg/result-reg-geo-origin-new.pdf}\label{geoorigin_defense}}
% \subfigure[UJIIndoor]{\includegraphics[width=0.24\textwidth]{../src_defense/figs/reg/result-reg-indoorLoc-new.pdf}\label{ujiindoor_defense}}
% \caption{Hyperparameter defense results of regression methods}
% \label{reg_res_defense}
% \end{figure*}

\begin{figure*}
\center
\subfigure[Diabetes]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/reg/result-reg-diabetes-new.pdf}\label{diabetes_defense}} 
\subfigure[GeoOrigin]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/reg/result-reg-geo-origin-new.pdf}\label{geoorigin_defense}}
\subfigure[UJIIndoor]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/reg/result-reg-indoorLoc-new.pdf}\label{ujiindoor_defense}}
\caption{Hyperparameter defense results of regression methods}
\label{reg_res_defense}
\end{figure*}


% \begin{figure}
% \center
% \label{reg_diabetes_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/reg/result-reg-diabetes-new.pdf}\label{diabetes_defense}}
% \caption{Hyperparameter defense results  of regression methods on Diabetes }
% \end{figure}

% \begin{figure}
% \center
% \label{reg_parkinson_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/reg/result-reg-parkinson-new.pdf}\label{parkinson_defense}}
% \caption{Hyperparameter defense results of regression methods on Parkinson }
% \end{figure}

% \begin{figure}
% \center
% \label{reg_geoorigin_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/reg/result-reg-geo-origin-new.pdf}\label{geoorigin_defense}}
% \caption{Hyperparameter defense results of regression methods on Geoorigin }
% \end{figure}

% \begin{figure}
% \center
% \label{reg_ujiindoor_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/reg/result-reg-indoorLoc-new.pdf}\label{ujiindoor_defense}}
% \caption{Hyperparameter defense results of regression methods on UJIIndoor}
% \end{figure}


\begin{figure*}
\center
\label{clf_lr_res_defense}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-lr-iris-new-new.pdf}\label{lr_iris_defense}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-lr-ionosphere-new-new.pdf}\label{lr_ionosphere_defense}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-lr-madelon-new-new.pdf}\label{lr_madelon_defense}} 
\caption{Hyperparameter defense results of LR classification methods}
\end{figure*}

% \begin{figure}
% \center
% \label{clf_lr_iris_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-lr-iris-new-new.pdf}\label{lr_iris_defense}}
% \caption{Hyperparameter defense results  of LR methods on Iris }
% \end{figure}

% \begin{figure}
% \center
% \label{clf_lr_ionosphere_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-lr-ionosphere-new-new.pdf}\label{lr_ionosphere_defense}}
% \caption{Hyperparameter defense results  of LR methods on Ionosphere }
% \end{figure}

% \begin{figure}
% \center
% \label{clf_lr_madelon_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-lr-madelon-new-new.pdf}\label{lr_madelon_defense}}
% \caption{Hyperparameter defense results  of LR methods on Madelon }
% \end{figure}


\begin{figure*}
\center
\label{clf_svc_res_defense}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-svc-iris-new-new.pdf}\label{svc_iris_defense}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-svc-ionosphere-new-new.pdf}\label{svc_ionosphere_defense}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_defense/figs/clf/result-clf-svc-madelon-new-new.pdf}\label{svc_ionosphere_defense}} 
\caption{Hyperparameter defense results of SVC classification methods}
\end{figure*}

% \begin{figure}
% \center
% \label{clf_svc_iris_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-svc-iris-new-new.pdf}\label{svc_iris_defense}}
% \caption{Hyperparameter defense results  of SVC methods on Iris }
% \end{figure}

% \begin{figure}
% \center
% \label{clf_svc_ionosphere_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-svc-ionosphere-new-new.pdf}\label{svc_ionosphere_defense}}
% \caption{Hyperparameter defense results  of SVC methods on Ionosphere }
% \end{figure}

% \begin{figure}
% \center
% \label{clf_svc_ionosphere_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-svc-ionosphere-new-new.pdf}\label{svc_ionosphere_defense}}
% \caption{Hyperparameter defense results  of SVC methods on Ionosphere }
% \end{figure}

\subsection{Sensitivity Results}

\begin{figure*}
\center
\subfigure[Diabetes]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/reg/result-reg-diabetes.pdf}\label{diabetes_defense}} 
\subfigure[GeoOrigin]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/reg/result-reg-geo-origin.pdf}\label{geoorigin_defense}}
\subfigure[UJIIndoor]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/reg/result-reg-indoorLoc.pdf}\label{ujiindoor_defense}}
\caption{Sensitivity analysis results of regression methods}
\label{reg_res_sensi}
\end{figure*}


\begin{figure*}
\center
\label{clf_lr_res_sensi}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-lr-iris.pdf}\label{lr_iris_sensi}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-lr-ionosphere.pdf}\label{lr_ionosphere_sensi}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-lr-madelon.pdf}\label{lr_ionosphere_sensi}} 
\caption{Sensitivity analysis results of LR classification methods}
\end{figure*}


\begin{figure*}
\center
\label{clf_klr_res_sensi}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-klr-iris.pdf}\label{klr_iris_sensi}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-klr-ionosphere.pdf}\label{klr_ionosphere_sensi}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-klr-madelon.pdf}\label{klr_ionosphere_sensi}} 
\caption{Sensitivity analysis results of KLR classification methods}
\end{figure*}


\begin{figure*}
\center
\label{clf_svc_res_sensi}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-svc-iris.pdf}\label{svc_iris_sensi}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-svc-ionosphere.pdf}\label{svc_ionosphere_sensi}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-svc-madelon.pdf}\label{svc_ionosphere_sensi}} 
\caption{Sensitivity analysis results of BLSVC classification methods}
\end{figure*}

\begin{figure*}
\center
\label{clf_ksvc_res_sensi}
\subfigure[Iris]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-ksvc-iris.pdf}\label{ksvc_iris_sensi}} 
\subfigure[Ionosphere]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-ksvc-ionosphere.pdf}\label{ksvc_ionosphere_sensi}}
\subfigure[Madelon]{\includegraphics[width=0.32\textwidth]{../src_sensitivity/figs/clf/result-clf-ksvc-madelon.pdf}\label{ksvc_ionosphere_sensi}} 
\caption{Sensitivity analysis results of BKSVC classification methods}
\end{figure*}


\begin{figure*}
\center
\label{clf_mlr_res}
\subfigure[Iris]{\includegraphics[width=0.48\textwidth]{../src_attack/figs/clf/result-clf-mlr-iris-new-final.pdf}\label{clf_mlr_iris}} 
\subfigure[Digits]{\includegraphics[width=0.48\textwidth]{../src_attack/figs/clf/result-clf-mlr-digits-new-final.pdf}\label{clf_mlr_digits}}
\caption{Hyperparameter stealing results of MLR classification methods}
\end{figure*}



\begin{figure*}
\center
\label{clf_mlr_res_defense}
\subfigure[Iris]{\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-mlr-iris-new-new.pdf}\label{mlr_iris_defense}} 
\subfigure[Digits]{\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-mlr-digits-new-new.pdf}\label{mlr_digits_defense}}
\caption{Hyperparameter defense results of MLR classification methods}
\end{figure*}


% \begin{figure}
% \center
% \label{clf_mlr_iris_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-lr-iris-multi-new-new.pdf}\label{mlr_iris_defense}}
% \caption{Hyperparameter defense results  of MLR methods on Iris }
% \end{figure}

% \begin{figure}
% \center
% \label{clf_mlr_digits_defense}
% {\includegraphics[width=0.48\textwidth]{../src_defense/figs/clf/result-clf-lr-digit-multi-new-new.pdf}\label{mlr_digits_defense}}
% \caption{Hyperparameter defense results of MLR methods on Digits }
% \end{figure}

\subsection{Real-world Simulation and Deployment}

Machine learning system: 

Training set + Validation set + Test Set 

From machine learning theory's perspective, the training set and test set are under the assumption that they are drawn from the same distribution. 

For instance, given a sample set, we split it into two parts, i.e., training set and validation set, and leverage cross validation to learn the hyperparameter as well as the model parameter. Then, we use the learnt hyperparameter to evaluate testing samples. Now, if we have acquired new data samples and send them to machine learning service provider. The service provide will adopt \emph{all} our provided samples and leverage cross validation to learn a new hyperparameter. As a result, each time we provide new samples, the ML service provide should update the hyperparameter using cross validation. One should note that cross-validation
occupies the majority of computing source when we train a model and is very time-consuming if the training set is large enough. 

However, we can reconsider the learning problem from a new perspective. Specifically, we can steal the hyperparameter learnt from the machine learning service on a representative training dataset. Then, we can reuse the hyperparameter instead of re-learning it to learn new model parameter when we are given new data samples (We call it one-shot training). %predict new unseen data which are also drawn from the same distribution. 

Questions: 

1. Whether there exist theoretical guarantees: if we choose different training sets with different sample sizes that are drawn from the same data distribution, whether the leant optimal hyperparameter is the same.

2. Accuracy should be almost the same. 


Synthetic dataset: Two Gaussian distributions + Poisson noise

%N = 1,000; 10,000; 100,000, 1,000,000
%mu1=[-1,-1], sigma1=[5, 0; 0, 5]
%X1 = np.random.multivariate_normal(mu1,sigma1,N)  # shape sample * dim
%vals = 2 ** np.ceil(np.log2(N))
%X1 = X1 + 2* np.random.poisson(abs(X1) * vals) / float(vals)
%
%mu2=[1,1], sigma2 = [5, 0; 0, 5]
%X2 = np.random.multivariate_normal(mu2,sigma2,N)
%vals = 2 ** np.ceil(np.log2(N))
%X2 = X2 + 2* np.random.poisson(abs(X2) * vals) / float(vals)

Real world dataset: UJInddoorLoc, Bank dataset, CovType dataset 

% \begin{figure*}
% \center
% \label{lr_gaussian}
% \subfigure[N=1,000]{\includegraphics[width=0.32\textwidth]{../src_time/figs/result-Gaussian-1000-lr-acc-time.pdf}\label{lr_gaussian_1000}} 
% \subfigure[N=10,000]{\includegraphics[width=0.32\textwidth]{../src_time/figs/result-Gaussian-10000-lr-acc-time.pdf}\label{lr_gaussian_10000}}
% \subfigure[N=100,000]{\includegraphics[width=0.32\textwidth]{../src_time/figs/result-Gaussian-100000-lr-acc-time.pdf}\label{lr_gaussian_100000}}
% \caption{Estimated relative error and speedup of LR on different synthetic Gaussian distributions with Poisson noise.}
% \end{figure*}

% \begin{figure*}
% \center
% \label{svc_gaussian}
% \subfigure[N=1,000]{\includegraphics[width=0.32\textwidth]{../src_time/figs/result-Gaussian-1000-svc-acc-time.pdf}\label{svc_gaussian_1000}} 
% \subfigure[N=10,000]{\includegraphics[width=0.32\textwidth]{../src_time/figs/result-Gaussian-10000-svc-acc-time.pdf}\label{svc_gaussian_10000}}
% \subfigure[N=100,000]{\includegraphics[width=0.32\textwidth]{../src_time/figs/result-Gaussian-100000-svc-acc-time.pdf}\label{svc_gaussian_100000}}
% \caption{Estimated relative error and speedup of BLSVC on different synthetic Gaussian distributions with Poisson noise.}
% \end{figure*}

% \begin{figure*}
% \center
% \label{lr_svc_bank}
% \subfigure[LR]{\includegraphics[width=0.48\textwidth]{../src_time/figs/result-bank-lr-acc-time.pdf}\label{lr_bank}} 
% \subfigure[BLSVC]{\includegraphics[width=0.48\textwidth]{../src_time/figs/result-bank-svc-acc-time.pdf}\label{svc_bank}}
% \caption{Estimated relative error and speedup of LR and BLSVC on the real-world Bank dataset.}
% \end{figure*}

\begin{figure*}
\center
\label{ridge_UJIndoorLoc}
\subfigure[M1 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-UJIndoorLoc-ridge-acc-time-m1-m3.pdf}\label{ridge_UJIndoorLoc_m1_m3}} 
\subfigure[M2 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-UJIndoorLoc-ridge-acc-time-m2-m3.pdf}\label{ridge_UJIndoorLoc_m2_m3}}
\caption{Estimated relative error and speedup of Ridge regression on UJIndoorLoc dataset.}
\end{figure*}

\begin{figure*}
\center
\label{lasso_UJIndoorLoc}
\subfigure[M1 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-UJIndoorLoc-Lasso-acc-time-m1-m3.pdf}\label{lasso_UJIndoorLoc_m1_m3}} 
\subfigure[M2 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-UJIndoorLoc-Lasso-acc-time-m2-m3.pdf}\label{lasso_UJIndoorLoc_m2_m3}}
\caption{Estimated relative error and speedup of LASSO regression on UJIndoorLoc dataset.}
\end{figure*}

\begin{figure}
\center
\label{real_defense}
\subfigure[Ridge]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-UJIndoorLoc-ridge-defense-m1-m3.pdf}\label{ridge_defense_m1_m3}} 
%\subfigure[LASSO]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-UJIndoorLoc-Lasso-defense-m1-m3.pdf}\label{lasso_defense_m1_m3}}
\caption{Estimated relative error of Ridge regression under defense on UJIndoorLoc dataset.}
\end{figure}

\begin{figure*}
\center
\label{lr_bank}
\subfigure[M1 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-bank-lr-acc-time-m1-m3.pdf}\label{lr_bank_m1_m3}} 
\subfigure[M2 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-bank-lr-acc-time-m2-m3.pdf}\label{lr_bank_m2_m3}}
\caption{Estimated relative error and speedup of L2-BLR on Bank dataset.}
\end{figure*}

\begin{figure*}
\center
\label{svc_bank}
\subfigure[M1 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-bank-svc-acc-time-m1-m3.pdf}\label{svc_bank_m1_m3}}
\subfigure[M2 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-bank-svc-acc-time-m2-m3.pdf}\label{svc_bank_m2_m3}}
\caption{Estimated relative error and speedup of BLSVC-SHL on Bank dataset.}
\end{figure*}

\begin{figure*}
\center
\label{lr_covtype}
\subfigure[M1 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-CovType-lr-acc-time-m1-m3.pdf}\label{lr_covtype_m1_m3}} 
\subfigure[M2 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-CovType-lr-acc-time-m2-m3.pdf}\label{lr_covtype_m2_m3}}
\caption{Estimated relative error and speedup of L2-BLR on CovType dataset.}
\end{figure*}

\begin{figure*}
\center
\label{svc_covtype}
\subfigure[M1 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-CovType-svc-acc-time-m1-m3.pdf}\label{svc_covtype_m1_m3}} 
\subfigure[M2 vs. M3]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-CovType-svc-acc-time-m2-m3.pdf}\label{svc_covtype_m2_m3}}
\caption{Estimated relative error and speedup of BLSVC-SHL on CovType dataset.}
\end{figure*}

\begin{figure*}
\center
\label{real_defense}
\subfigure[L2-BLR]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-bank-lr-defense-m1-m3.pdf}\label{lr_defense_m1_m3}} 
\subfigure[BLSVC-SHL]{\includegraphics[width=0.45\textwidth]{../src_time/figs/result-bank-svc-defense-m1-m3.pdf}\label{svc_defense_m1_m3}}
\caption{Estimated relative error of L2-BLR and BLSVC-SHL under defense on Data dataset.}
\end{figure*}





==> notation.tex <==
\subsection{Notation and Definition}

\subsubsection{Notation} 

In this paper, vectors and matrices are written as bold lowercase and uppercase symbols. The $i$-th entry of vector $\mathbf{u}$ is $u_i$, and $\mathbf{u}_{-i}$ is $\mathbf{u}$ without $i$-th entry. We denote $\mathbf{u}^+$ and $\mathbf{u}^{-}$ as positive entries and negative entries of $\mathbf{u}$; and their $l$-th entry as $u_l^+$ and $u_l^-$ respectively.
For matrix $\mathbf{W}$, its $(i,j)$-th entry, $i$-th column, and $j$-th row are denoted as $w_{i,j}$, $\mathbf{w}_i$, and $\mathbf{w}^j$ respectively. For $\mathbf{w}_i$ and $\mathbf{w}^j$, their transpose are denoted as $\mathbf{w}_i^T$ and $\mathbf{w}^j_T$. $\mathbf{W}_{:,-i}$ and $\mathbf{W}_{-j,:}$ are $\mathbf{W}$ without $i$-th column and $j$-th row.  

For vector $\mathbf{u} \in \mathbb{R}^m$, its $l_p$-norm is $\left\| \mathbf{u} \right\|_p = {(\sum_{i=1}^m |u_i|^p)}^\frac{1}{p}$ and $l_\infty$-norm is $\left\| \mathbf{u} \right\|_\infty = \max_i |u_i|$. The inner product between two vectors $\mathbf{u}, \mathbf{v} \in \mathbb{R}^m$ is $\langle \mathbf{u}, \mathbf{v} \rangle = \mathbf{u}^T \mathbf{v} = \sum_{i}^m u_i v_i$. 

%For matrix $\mathbf{W} \in \mathbb{R}^{m \times n}$, its $l_1$ norm is $\| \mathbf{W}\|_1 = \sum_{i=1}^m |\mathbf{w}^i|_1 = \sum_{j=1}^n |\mathbf{w}_j|_1 = \sum_{i=1}^m \sum_{j=1}^n |w_{ij}|$. %and Frobenius norm $\| \mathbf{W} \|_F = \sqrt{\sum_{i=1}^m \sum_{j=1}^n w_{i,j}^2}$. 
%The inner product between two matrices $\mathbf{W}$, $\mathbf{U}$ is $\langle \mathbf{W}, \mathbf{U} \rangle = \textbf{tr}(\mathbf{W}^C \mathbf{U})$, where $\textbf{tr}$ is the trace operator defined on a square matrix.

In this paper, we assume that each data sample $\mathbf{x}_i$ is drawn from the $m$-dim Euclidean space $\Re$^{m}, and denote $n$ data samples row by row as $\mathbf{X} = \{ \mathbf{x}_1^T; \mathbf{x}_2^T; \cdots; \mathbf{x}_n^T  \} \in \Re^{n \times m}$. For regression methods, we assume that data samples are centered to the origin; for classification methods, we further assume that data samples are normalized to have unit length, so as to eliminate the effect of magnitute of different features. 

Moreover, consider that all methods involve the hyperparameter(s) estimate, we use the same notation for the same type of algorithm for simplicity. For instance, for LR-based methods, we adopt $\lambda$; for SVC-based methods, we adopt $C$. 

%Moreover, for regression methods, we assume that data samples are centered to the origin; for classification methods, we further assume that data samples are normalized to have unit length, so as to eliminate the effect of magnitute of different features. 

\subsection{Terminology}

\begin{definition}[Convex Set and Convex Function~\cite{boyd2004convex}]

A set $\mathbb{C}$ is \emph{\textbf{convex}} if the line segment between any two points in $\mathbb{C}$ lies in $\mathbb{C}$, i.e., $\forall p_1, p_2 \in \mathbb{C}$ and $\forall \theta$ with $0 \leq \theta \leq 1$,
\begin{align*}
\theta p_1 + (1-\theta) p_2 \in \mathbb{C}.
\end{align*}

A function $f: \mathbb{R} \rightarrow \mathbb{R}$ is \emph{\textbf{convex}} if the domain of $f$, \textbf{dom} f, is a \emph{convex set} and for all $p, q \in \textbf{dom} f$, and $\forall \theta$ with $0 \leq \theta \leq 1$, we have 
\begin{align*}
f(\theta p + (1-\theta) q) \leq \theta f(p) + (1-\theta) f(q).
\end{align*}
\end{definition}

\begin{definition}[Subgradient and Subdifferential~\cite{boyd2004convex}]
The \emph{\textbf{subgradient}} of a convex function $f: \mathbb{I} \rightarrow \mathbb{R}$ at a point $p_0$ in the open interval $\mathbb{I}$ is a real number $g$ such that the
\begin{align*}
f(p)-f(p_0) \geq g (p-p_0), \, \forall p \in \mathbb{I}.
%$f(\mathbf{\theta}-f(\mathbf{\theta}_0) \geq \mathbf{\theta-\theta_0}^C \mathbf{g}$.
\end{align*}
The set of subgradients are defined as the interval $[a, b]$, where $a$ and $b$ are the one-sided limits
\begin{align*}
a = \lim_{p \to p_0^-} \frac{f(p)-f(p_0)}{p-p_0}, \, 
b = \lim_{p \to p_0^+} \frac{f(p)-f(p_0)}{p-p_0}. 
\end{align*} 
The set $[a, b]$ of all subgradients is called the \emph{\textbf{subdifferential}} of the function $f$ at $p_0$ and is denoted as $\partial f(p)|_{p_0}$. 
\end{definition}

\begin{definition}[Kernel Function and Mercer Kernel~\cite{murphy2012machine}] A kernel function $\kappa$ is a real-valued function of two parameters $\mathbf{x}, \mathbf{x}^{\prime} \in \Delta$, where $\Delta$ is some abstract, even infinite dimensional, space, such that $\kappa(\mathbf{x}, \mathbf{x}^{\prime})$ is nonnegative, i.e., $\kappa(\mathbf{x}, \mathbf{x}^{\prime}) \geq 0$, and symmetric, i.e., $\kappa(\mathbf{x}, \mathbf{x}^{\prime}) = \kappa(\mathbf{x}^{\prime}, \mathbf{x})$. Therefore, it can be treated as a measure of similarity. 

Mercer kernel (or positive definite kernel) is the kernel which requires the \textbf{Gram matrix}
\begin{equation}
\mathbf{K} = 
\begin{bmatrix}
& \kappa(\mathbf{x}_1, \mathbf{x}_1) & \cdots & \kappa(\mathbf{x}_1, \mathbf{x}_n) \\
&  & \vdots & \\
& \kappa(\mathbf{x}_n, \mathbf{x}_1) & \cdots & \kappa(\mathbf{x}_n, \mathbf{x}_n) \\
\end{bmatrix}
\end{equation}
be positive definite for any set of inputs $\{ \mathbf{x}_i \}_{i=1}^n$. In general, if the kernel is Mercer kernel, then there exists a function $\phi$ mapping $\mathbf{x} \in \Delta$ to $\phi(\mathbf{x}) \in \mathbb{R}^M $ such that the kernel function
\begin{align}
\kappa(\mathbf{x}, \mathbf{x}^\prime) = \langle \phi(\mathbf{x}), \phi(\mathbf{x}^\prime) \rangle,
\end{align}
is represented as an \emph{inner product} of mapped feature vectors in an implicit feature space defined by $\phi$, which in essence depends on the eigenfunction of $\kappa$. Hence, $M$ can be potentially infinite dimension.     

\end{definition}



==> reg.tex <==
\section{Hyperparameter Stealing Attack}

\subsection{Attack on Convex-induced Regression Models} 

We classify regression models into linear and nonlinear cases.

\subsubsection{Linear model-based regression} In this category, we aim at stealing hyperparameters of well-known ridge regression~\cite{hoerl1970ridge}, LASSO~\cite{tibshirani1996regression}, and Elastic Net~\cite{zou2005regularization}. 

% \begin{align}
% \mathcal{L}_{OLS}(\mathbf{w}) = \| \mathbf{y-X\beta} \|_2^2.
% \end{align}

\textbf{Ridge Regression}
%\subsubsection{Ridge Regression}

\begin{align}
\label{ridge_reg}
\begin{split}
& \mathcal{L}_{Ridge}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X} \mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_2^2 \\
& = \mathbf{y}^T \mathbf{y} - 2 \mathbf{w}^T \mathbf{X}^T \mathbf{y} + \mathbf{w}^T \mathbf{X}^T \mathbf{X} \mathbf{w} + \lambda \mathbf{w}^T \mathbf{w} \\
& = \mathbf{y}^T \mathbf{y} - 2 w_i \mathbf{x}_i^T \mathbf{y} - 2 \mathbf{w}_{-i}^T \mathbf{X}^T_{:,-i} \mathbf{y} + w_i \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 w_i \mathbf{x}_i^T \mathbf{X}_{:,-i} \mathbf{w}_{-i} \\
& \quad \quad + \mathbf{w}_{-i}^T \mathbf{X}^T_{:,-i} \mathbf{X}_{:,-i} \mathbf{w}_{-i} + \lambda (w_i^2 + \mathbf{w}_{-i}^T \mathbf{w}_{-i} )   
\end{split}
\end{align}

Taking the gradient of $\mathcal{L}_{Ridge}$ with respect to $w_i$ yields
\begin{align*}
%\label{ridge_reg_grad}
\begin{split}
\frac{\partial \mathcal{L}_{Ridge}}{\partial w_i} & = -2 \mathbf{x}_i^T \mathbf{y} + 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \mathbf{x}_i^T \mathbf{X}_{:,-i} \mathbf{w}_{-i} + 2 \lambda w_i \\ 
& = 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right \rangle + 2 \lambda w_i, 
\end{split}
\end{align*}
where $\mathbf{r}_i = \mathbf{y}-\mathbf{X}_{:,-i} \mathbf{w}_{-i}$ is the residual that all features are used except the $i$-th feature to approximate $\mathbf{y}$. 

Setting $\partial_{w_i} \mathcal{L}_{Ridge} = 0$, we can estimate $\lambda$  for each $w_i$  as
\begin{align}
\label{ridge_reg_soln}
\hat{\lambda}^{(i)}_{Ridge} = \frac{-\langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle}{w_i}.
\end{align}

Eqn~\ref{ridge_reg_soln} implies that if we are provided $\mathbf{w}$ by machine learning service provider (who achieves it using some training dataset and certain model selection (e.g., cross validataion, AIC, BIC) technique). Then, we can ``steal" the true hyperparameter $\lambda$, denoted as $\hat{\lambda}_1$. 

Theoretically, each estimated $\hat{\lambda}^{(i)}_{Ridge}$ should be the exact $\lambda$. We demonstrate that our estimates are indeed accurate from the experimental results. 

\textbf{LASSO}
%\subsubsection{LASSO}

\begin{align}
\label{lasso}
\mathcal{L}_{LASSO}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_1.
\end{align}

Notice that the $\| \mathbf{w} \|_1$ term is not differentiable when $w_i=0$. To handle such a nonsmooth function, we need to extend the notion of gradient to \emph{subgradient}. As defined above, the subderivative of $\mathcal{L}_{LASSO}$ with respect to $w_i$ is given by  
\begin{align*}
%\label{lasso_grad}
\frac{\partial \mathcal{L}_{LASSO}}{\partial w_i} = 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle + \lambda \partial \|\mathbf{w}\|_1 |_{w_i},
\end{align*}
where 
\begin{align*}
\partial \| \mathbf{w} \|_1 |_{w_i} = 
\begin{cases}
-1 & \text{if } w_i < 0 \\
[-1, 1] & \text{if } w_i = 0 \\
1  & \text{if } w_i > 0.
\end{cases}
\end{align*}
 
%where $\mathbf{r}_i = \mathbf{y}-\mathbf{X}_{:,-i} \mathbf{\theta}_{-i}$. $\mathbf{\theta}_{-i}$ is $\mathbf{\theta}$ without entry $\theta_i$, $\mathbf{X}_{:,-i}$ is $\mathbf{X}$ without $i$-th feature $\mathbf{x}_i$. $\mathbf{r}_i$ is the residual that uses all features except $i$-th feature. 

In doing so, we have the following subgradient 
%anlaytic solution of subgradient as follows
\begin{align*}
%\label{lasso_subgrad}
\frac{\partial \mathcal{L}_{LASSO}}{\partial w_i} =  
\begin{cases}
2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle - \lambda & \text{if } w_i < 0 \\
\left[ - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right \rangle - \lambda, - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle + \lambda \right] & \text{if } \, w_i = 0 \\
2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle + \lambda & \text{if } w_i > 0
\end{cases}
\end{align*}

% Setting $\frac{\partial \mathcal{L}_{LASSO}}{\partial w_i} = 0$, we have three cases of values of $w_i$, which depends on the value of $\lambda$ and $\left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle$, as follows: 
% \begin{align}
% w_i = 
% \begin{case}
% (2 \left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle + \lambda) / (2 \| \mathbf{x}_i \|_2^2) \quad \text{if} \, c_j < -\lambda \\
% 0 \quad \text{if} \, c_j \in [-\lambda, \lambda] \\
% (2 \left\langle \mathbf{x}_i, \mathbf{r}_i) \right \rangle - \lambda) / (2 \| \mathbf{x}_i \|_2^2) \quad \text{if} \, c_j > \lambda 
% \end{case}
% \end{align}

%Suppose that one have obtained $\mathbf{w}$ and the associated $\lambda$ using the training dataset and certain model selection (e.g., cross validataion, AIC, BIC) technique. 
Then for each $w_i$, we can estimate $\lambda$ as
\begin{align}
\label{lasso_soln}
\hat{\lambda}^{(i)}_{LASSO} =  
\begin{cases}
2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if }  w_i < 0 \\
-2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if } w_i > 0 
\end{cases}
\end{align}

Note that, if $\lambda \geq \lambda_{\max}$, we get $\mathbf{w} = 0$, where 
\begin{align}
\lambda_{\max} = \| \mathbf{X}^T \mathbf{y} \|_{\infty} = \max_i |\langle \mathbf{y}, \mathbf{x}_i \rangle|.
\end{align} 
The value is obtained by using the fact that $\mathbf{0}$ is optimal if $(\mathbf{X}^T \mathbf{y})_j \in [-\lambda, \lambda], \forall j$. Therefore, we have $\hat{\lambda}^{(i)}_{LASSO} < \max_i |\langle \mathbf{y}, \mathbf{x}_i \rangle|$.


\textbf{Elastic Net}
%\subsubsection{Elastic Net: More general case}

\begin{align}
\label{enet}
\mathcal{L}_{ElasticNet}(\lambda_2, \lambda_1, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda_2 \| \mathbf{w} \|_2^2 + \lambda_1 \| \mathbf{w} \|_1.
\end{align}

Similarly with Ridge regression and LASSO, we take the gradient of $\mathcal{L}_{ElasticNet}$ with respect to $w_i$ as 
\begin{align*}
\frac{\partial \mathcal{L}_{ElasticNet}}{\partial w_i} = 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle + \lambda_2 \partial_{w_i} \mathbf{w}^T \mathbf{w} + \lambda_1 \partial \| \mathbf{w} \|_1 |_{w_i}.
\end{align*}

Incorporating into the subgraident $\partial \| \mathbf{w} \|_1 |_{w_i}$, we have 
\begin{align*}
\small
%\label{enet_subgrad}
\frac{\partial \mathcal{L}_{ElasticNet}}{\partial w_i} =  
\begin{cases}
2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle + 2 \lambda_2 w_i - \lambda_1 & \text{if } w_i < 0 \\
\left[ - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right \rangle + 2 \lambda_2 w_i - \lambda_1, - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle + 2 \lambda_2 w_i + \lambda_1 \right] & \text{if }  w_i = 0 \\
2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle + 2 \lambda_2 w_i + \lambda_1 & \text{if } w_i > 0
\end{cases}
\end{align*}

Setting $\partial_{w_i} \mathcal{L}_{ElasticNet} = 0$, we have the following equations 
%for each $w_i$, we can estimate $\lambda$ and $\lambda$ using the following equations
\begin{align}
\label{enet_eqn_1}
\begin{cases}
-2 \lambda_2 w_i + \lambda_1 = 2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if }  w_i < 0 \\
2 \lambda_2 w_i + \lambda_1 = -2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if } w_i > 0 \\
\end{cases}
\end{align}

Since there are two hyperparameters to be estimated, we therefore need at least two equations.  

% Here we provide two ways given $\mathbf{w}$. The first way is we randomly choose two equations of Eqn~\ref{enet_eqn_1} with the associated nonzero $w_m$s and $w_n$, and calculate the right hand side values, denoted as $f(w_m, r_m)$ and $f(w_n, r_n)$, respectively. Then, $\lambda$ and $\lambda_1$ can be determined in the following cases:
% \begin{align}
% \small
% \label{enet_soln_1}
% \begin{cases}
% \hat{\lambda}_3 = \frac{f(w_n, r_n)-f(w_m, r_m)}{w_m+w_n}, \, \hat{\lambda}_4 = f(w_m,r_m) + 2\hat{\lambda}_3 w_m & \text{if } w_m < 0 \text{ and } w_n > 0 \\
% \hat{\lambda}_3 = \frac{f(w_m, r_m)-f(w_n, r_n)}{w_m+w_n}, \, \hat{\lambda}_4 = f(w_m,r_m) - 2\hat{\lambda}_3 w_m & \text{if } w_m > 0 \text{ and } w_n < 0 \\
% \hat{\lambda}_3 = \frac{f(w_m, r_m)-f(w_n, r_n)}{-w_m+w_n}, \, \hat{\lambda}_4 = f(w_m,r_m) + 2\hat{\lambda}_3 w_m & \text{if } w_m < 0 \text{ and } w_n < 0 \\
% \hat{\lambda}_3 = \frac{f(w_m, r_m)-f(w_n, r_n)}{w_m-w_n}, \, \hat{\lambda}_4 = f(w_m,r_m) - 2\hat{\lambda}_3 w_m & \text{if } w_m > 0 \text{ and } w_n > 0 \\
% \end{cases}
% \end{align}  

%Another way that 
Here, we consider estimating $\lambda_2$ and $\lambda_1$ by leveraging all equations in Eqn~\ref{enet_eqn_1}. In this way, the estimate of $\lambda_2$ and $\lambda_1$ can be cast into ``least square regression". Specifically, we denote $l$-th entry of $\mathbf{w}^+$ and $\mathbf{w}^-$ as $w_l^+$ and $w_l^-$. Furthermore, we construct the following matrices  
\begin{align*}
\mathbf{A} = \left[
\begin{array}{cc}
2 w_1^+ & 1 \\
2 w_2^+ & 1 \\
\vdots & \vdots \\
-2 w_1^- & 1 \\
-2 w_2^- & 1 \\
\vdots & \vdots \\
\end{array}
\right], \quad
\bm{\lambda} = \left[ 
\begin{array}{c}
\lambda_2 \\
\lambda_1 \\
\end{array} 
\right], \\
%\quad
\mathbf{b} = \left[ 
\begin{array}{c}
-2 (\mathbf{x}_1^+)^T \mathbf{x}_1^+ w_1^+ + 2 \left\langle \mathbf{x}_1^+, \mathbf{r}_1^+ \right\rangle \\
-2 (\mathbf{x}_2^+)^T \mathbf{x}_2^+ w_1^+ + 2 \left\langle \mathbf{x}_2^+, \mathbf{r}_2^+ \right\rangle \\
\vdots \\
2 (\mathbf{x}_1^-)^T \mathbf{x}_1^- w_1^- - 2 \left\langle \mathbf{x}_1^-, \mathbf{r}_1^- \right\rangle \\
2 (\mathbf{x}_2^-)^T \mathbf{x}_2^- w_2^- - 2 \left\langle \mathbf{x}_2^-, \mathbf{r}_2^- \right\rangle \\
\vdots
\end{array}
\right]. 
\end{align*}

With above notation, the system of equations in Eqn~\ref{enet_eqn_1} can be rewritten into the \textbf{normal equation}
\begin{align}
\label{enet_soln_2}
\mathbf{A}^T \mathbf{A} \bm{\lambda} = \mathbf{A}^T \mathbf{b}.
\end{align}
and thus $\bm{\lambda}$ can be estimated as 
\begin{align}
\hat{\bm{\lambda}}_{ElasticNet} = \left( \mathbf{A}^T \mathbf{A} \right)^{-1} \mathbf{A}^T \mathbf{b}.
\end{align}

% \subsubsection{Support Vector Regression}

% \begin{align}
% \label{svr}
% \mathcal{L}_{SVR}(C, \mathbf{w}) = C \sum_{j=1}^n L_{\epsilon}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2,
% \end{align}
% where 
% \begin{align}
% L_{\epsilon}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle) = 
% \begin{cases}
% 0 & \text{if } |y_j - \langle \mathbf{w}, \mathbf{x}^j_T \rangle| \leq \epsilon \\
% |y_j - \langle \mathbf{w}, \mathbf{x}^j_T \rangle | - \epsilon  & \text{if } |y_j - \langle \mathbf{w}, \mathbf{x}^j_T \rangle| > \epsilon
% \end{cases}
% \end{align}
% is the so called $\epsilon$-\textbf{insensitive loss function}. It indicates that any point lying insider an $\epsilon$-tube around the prediction is not penalized. 
% %$\hat{y}_j = \langle \mathbf{w}, \mathbf{x}^j_T \rangle$ and $C = 1 / \lambda$ is a regularization constant.
% Note that the objective is convex, but is not differentiable at the points $y_j = \langle \mathbf{w}, \mathbf{x}^j_T \rangle + \epsilon$ and $y_j = \langle \mathbf{w}, \mathbf{x}^j_T \rangle - \epsilon$ due to the absolute value function in the loss term. 

% % One popular approach is to formulate the problem as a constrained optimization problem by introducing \textbf{slack variables} to represent the degree to which each sample lies outside the $\epsilon$-tube. Specifically, we rewrite the objective as 
% % \begin{align}
% % \begin{split}
% % & \mathcal{L}_{SVR}(\mathbf{w},\bm{\xi}_+, \bm{\xi}_+, C) = C \sum_{j=1}^n ( \xi^j_+ + \xi^j_- ) + \frac{1}{2} \| \mathbf{w} \|_2^2 \\
% % & \text{s.t. } \langle \mathbf{w} \mathbf{x}^j \rangle - \epsilon - \xi^j_- \leq y_j \leq \langle \mathbf{w} \mathbf{x}^j \rangle + \epsilon + \xi^j_+, \xi^j_+, \xi^j_- \geq 0, \forall j.
% % \end{split}
% % \end{align}

% The subgradient of $L_{\epsilon}$ with respect to $\mathbf{w}$ is then given by 
% \begin{align}
% \frac{\partial L_{\epsilon}(y_j, \langle \mathbf{w}, \mathbf{x}^j_T \rangle)}{\partial \mathbf{w}} = 
% \begin{cases}
% -\mathbf{x}^j_T & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle < y_j - \epsilon \\
% \left[ -\mathbf{x}^j_T, \mathbf{0} \right] & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle = y_j - \epsilon \\
% \mathbf{0} & \text{if } y_j - \epsilon < \langle \mathbf{w}, \mathbf{x}^j_T \rangle < y_j + \epsilon \\
% \left[ \mathbf{0}, \mathbf{x}^j_T \right] & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle = y_j + \epsilon \\
% \mathbf{x}^j_T & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle > y_j + \epsilon
% \end{cases}
% \end{align}


% %Here, we consider the case when $\epsilon=0$.

% In practice, for two non-differential points, the subgradient is set to be 0.
% Finally, setting the derivative of $\mathcal{L}_{SVR}$ with respect to $\mathbf{w}$ to zero, we estimate $C$ as  
% \begin{align}
% \hat{C}^{(i)} = \frac{w_i}{\sum\limits_{j,\langle \mathbf{w}, \mathbf{x}^j_T \rangle < y_j - \epsilon} x_{j,i} - \sum\limits_{j,\langle \mathbf{w}, \mathbf{x}^j_T \rangle > y_j + \epsilon} x_{j,i} }
% \end{align}

% It is critical here, as in any regularization scheme, that a proper value is chosen for $C$, the penalty factor. If it is too large, we have a high penalty for nonseparable points and we may store many support vectors and overfit. If it is too small, we may have underfitting." 
% Alpaydin (2004), page 224
% \begin{align}
% \hat{C}^{(i)} = 
% \begin{cases}
% \frac{w_i}{x_{j,i}} & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle < y_j \\
% -\frac{w_i}{x_{j,i}} & \text{if } \langle \mathbf{w}, \mathbf{x}^j_T \rangle > y_j
% \end{cases}
% \end{align}

\subsubsection{Nonlinear model-based regression}
%\subsubsection{Nonlinear Model}

So far, we have noticed that we regress each data sample using a fixed finite dimensional feature vector, i.e., $\mathbf{x}^j \in \mathbb{R}^m $. However, for certain types of data, it is not clear how they can be best represented using fixed-dimension feature vector. For instance, how can we represent a text document, which can be of variable length? One well-known approach to handle such problem is to leverage a \textbf{nonlinear kernel function} $\kappa$ that measures the similarity between data samples in an implicit, abstract, even infinite dimensional feature space. As aforementioned, $\kappa$ is nonnegative and symmetric.

In this paper, we consider the following kernels
\begin{itemize}
\item Gaussian kernel: $\kappa(\mathbf{x}, \mathbf{x}^\prime) = \exp \big( \frac{\| \mathbf{x} - \mathbf{x}^\prime \|_2^2}{2 \sigma^2} \big)$, where $\sigma^2$ is the bandwidth.
\item Polynomial kernel: $\kappa(\mathbf{x}, \mathbf{x}^\prime) = (\langle \mathbf{x}, \mathbf{x}^\prime \rangle)^d$, where $d$ is the degree of the polynomial. 
\end{itemize}      
Note that aforementioned linear models use the simplest linear kernel, i.e.,  $\kappa(\mathbf{x}, \mathbf{x}^\prime) = \langle \mathbf{x}, \mathbf{x}^\prime \rangle $.

In general, if the kernel is Mercer kernel (positive definite kernel), then there exists a function $\phi$ mapping $\mathbf{x} \in \mathbb{R}^m$ to $\phi(\mathbf{x}) \in \mathbb{R}^M $ such that 
\begin{align}
\kappa(\mathbf{x}, \mathbf{x}^\prime) = \langle \phi(\mathbf{x}), \phi(\mathbf{x}^\prime) \rangle,
\end{align}
is an inner product of some feature vectors that are implicitly defined by $\phi$, which depends on the eigen functions of $\kappa$.  Hence, $M$ can be potentially infinite dimension.     

In this part, we only focus on kernel-based ridge regression (KLR)~\cite{welling2013kernel}, as the kernel version of LASSO and Elastic Net is soldem used in practice. 

\textbf{Kernel Ridge Regression}
%\subsubsection{Kernel Ridge Regression}

%Define the kernel mapping function $\Phi : \mathbb{R}^m -> \mathbb{R}^M$. 

\begin{align}
\label{kernel_ridge_primal}
\mathcal{L}_{KernelRidge}(\lambda, \mathbf{w}^\prime) = \| \mathbf{y}-\Phi(\mathbf{X}) \mathbf{w}^\prime \|_2^2 + \lambda \| \mathbf{w}^\prime \|_2^2,
\end{align}
where $\Phi(\mathbf{X}) = \left[ \phi(\mathbf{x}^1_T); \phi(\mathbf{x}^2_T); \cdots; \phi(\mathbf{x}^n_T) \right] \in \mathbb{R}^{n \times M}$. 

Using Mercer's Theorem~\cite{XX}, $\mathbf{w}^\prime$ can be rewritten as a linear combination of samples mapped into the feature space, i.e., 
\begin{align*}
\mathbf{w}^\prime = \sum_{j=1}^n \alpha_j \phi(\mathbf{x}^j_T) = \Phi(\mathbf{X})^T \bm{\alpha}.
\end{align*} 
Correspondingly, $\mathbf{w}^\prime$ and $ \bm{\alpha}$ are respectively called \textbf{primal variables} and \textbf{dual variables}.

For ease of computation, kernalized methods often optimize $\bm{\alpha}$ with size $n$ instead of (infinite) $M$-dimensional $\mathbf{w}^\prime$. Therefore, by substituting $\mathbf{w}^\prime$ with $\Phi(\mathbf{X})^T \bm{\alpha}$, Eqn~\ref{kernel_ridge_primal} becomes 
\begin{align}
\label{kernel_ridge_dual}
\begin{split}
\mathcal{L}_{KernelRidge}(\lambda, \bm{\alpha}) & = \| \mathbf{y}-\Phi(\mathbf{X}) \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 + \lambda \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
& = \| \mathbf{y} - \mathbf{K} \bm{\alpha} \|_2^2 + \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha},
\end{split}
\end{align}
where $\mathbf{K}=\Phi(\mathbf{X}) \Phi(\mathbf{X})^T=\{ \langle \phi(\mathbf{x}^i_T), \phi(\mathbf{x}^j_T) \rangle_{i,j} \}$ is an $n \times n$ inner product matrix, also called \textbf{Gram matrix}, defined in the feature space.

Taking the gradient of $\mathcal{L}_{KernelRidge}$ with respect to $\bm{\alpha}$ and setting it to zero, we have
\begin{align}
\mathbf{K}(\lambda \bm{\alpha} + \mathbf{K} \bm{\alpha} - \mathbf{y}) = \mathbf{0}.
\end{align} 

Note that $\mathbf{K}$ is positive definite and full rank. Therefore, $\lambda \bm{\alpha} + \mathbf{K} \bm{\alpha} - \mathbf{y} = \mathbf{0}$ and we can estimate $\lambda$ for each $\alpha_j$ as
\begin{align}
\hat{\lambda}^{(j)}_{KernelRidge} = \frac{y_j - \mathbf{k}^{j} \alpha_j}{\alpha_j}. 
\end{align}

As the kernel version of LASSO and Elastic Net is seldom used in real-world problems, we thus do not provide the analysis. 
 
% \subsubsection{Kernel Support Vector Regression}

% The problem with kernel ridge regression is that the $\mathbf{w}^\prime$ depends on all the training samples. We now seek a method to produce a sparse estimate of $\mathbf{w}^\prime$.

% Leveraging the similar idea as kernel ridge regression, we rewrite primal variables $\mathbf{w}^{\prime}$ using its dual $\bm{\alpha}$ and have 
% \begin{align}
% \label{kernel_svr}
% \begin{split}
% \mathcal{L}_{KernelSVR}(C, \bm{\alpha}) & = C \sum_{j=1}^n L_{\epsilon}(y_j, \langle \Phi(\mathbf{X})^T \bm{\alpha}, \phi(\mathbf{x}^j_T) \rangle) + \frac{1}{2} \| \Phi(\mathbf{X})^T \bm{\alpha} \|_2^2 \\
% & = C \sum_{j=1}^n L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha}, 
% \end{split}
% \end{align}
% where 
% \begin{align}
% L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle) = 
% \begin{cases}
% 0 & \text{if } |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle| \leq \epsilon \\
% |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle | - \epsilon  & \text{if } |y_j - \langle \bm{\alpha}, \mathbf{k}_j \rangle| > \epsilon
% \end{cases}
% \end{align}
% and $\mathbf{k}_j = \Phi(\mathbf{X}) \phi(\mathbf{x}^j_T)$.

% Note again that the objective function is convex but not differentiable at the points $y_j = \langle \bm{\alpha}, \mathbf{k}_j \rangle \pm \epsilon$. Then, the subgradient of $L_{\epsilon}$ with respect to $\bm{\alpha}$ is 
% \begin{align}
% \frac{\partial L_{\epsilon}(y_j, \langle \bm{\alpha}, \mathbf{k}_j \rangle)}{\partial \bm{\alpha}} = 
% \begin{cases}
% - \mathbf{k}_j & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j - \epsilon \\
% \left[ -\mathbf{k}_j, \mathbf{0} \right] & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle = y_j - \epsilon \\
% \mathbf{0} & \text{if } y_j - \epsilon < \langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j + \epsilon \\
% \left[ \mathbf{0}, \mathbf{k}_j \right] & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle = y_j + \epsilon \\
% \mathbf{k}_j & \text{if } \langle \bm{\alpha}, \mathbf{k}_j \rangle > y_j + \epsilon
% \end{cases}
% \end{align}

% Finally, we set the subgradient of non-differential points as 0 and the derivative of $\mathcal{L}_{KernelSVR}$ with respect to $\bm{\alpha}$ to zero. With it, $C$ is estimated as  
% \begin{align}
% \hat{C}^{(i)} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,\langle \bm{\alpha}, \mathbf{k}_j \rangle < y_j - \epsilon} k_{j,i} - \sum\limits_{j,\langle \bm{\alpha}, \mathbf{k}_j \rangle > y_j + \epsilon} k_{j,i} }
% \end{align}


==> table.tex <==


\begin{sidewaystable*}
\small
\centering
\caption{Summarization of all ML models.}
\label{sum_ml}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
  Category                &       \multicolumn{2}{c|}{ML Model}       & Objective Function & Loss Function & Regularization \\ \hline
\multirow{4}{*}{Regression} & \multirow{3}{*}{Linear} & RR & $\mathcal{L}_{RR}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X} \mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_2^2 $	& Least Square & $L_2$ \\ \cline{3-6} 
                  &                   &  LASSO & $\mathcal{L}_{LASSO}(\lambda, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda \| \mathbf{w} \|_1. $ & Least Square & $L_1$ \\ \cline{3-6} 
                  &                   & ENet & $ \mathcal{L}_{ENet}(\lambda_2, \lambda_1, \mathbf{w}) = \| \mathbf{y}-\mathbf{X}\mathbf{w} \|_2^2 + \lambda_2 \| \mathbf{w} \|_2^2 + \lambda_1 \| \mathbf{w} \|_1 $ & Least Square & $L_2 + L_1$ \\ \cline{2-6} 
                  &     Nonlinear       & KRR       & $\mathcal{L}_{KRR}(\lambda, \bm{\alpha}) = \| \mathbf{y} - \mathbf{K} \bm{\alpha} \|_2^2 + \lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha}$ &  Least Square & $L_2$ \\ \hline

           
\multirow{4}{*}{BLR Classification} & \multirow{2}{*}{Linear}  & L2-BLR & $\mathcal{L}_{L2-BLR}(
\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};
\mathbf{x}_i,y_j) + 
\lambda \| \mathbf{w} \|_2^2 $
 & Cross Ent. & $L_2$ \\ \cline{3-6} 
                  &                    & L1-BLR & $\mathcal{L}_{L1-BLR}(
\lambda, \mathbf{w}) = \sum_{j=1}^n \text{NLL}_{BLR}(\mathbf{w};
\mathbf{x}_i,y_j) + 
\lambda \| \mathbf{w} \|_1 $ & Cross Ent. & $L_1$ \\ \cline{2-6} 
                  
                  & \multirow{2}{*}{Nonlinear}  & L2-BKLR & $\mathcal{L}_{L2-BKLR}(
\lambda, \bm{\alpha}) = \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + 
\lambda \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & Cross Ent. & $L_2$ \\ \cline{3-6} 
                  
                  &                    &  L1-BKLR & $\mathcal{L}_{L1-BKLR}(
\lambda, \bm{\alpha}) = \sum_{j=1}^n \text{NLL}_{BKLR}(\bm{\alpha}; \mathbf{k}_j,y_j) + 
\lambda \| \mathbf{K} \bm{\alpha} \|_1 $ & Cross Ent. & $L_1$ \\ \hline

\multirow{2}{*}{MLR Classification} & Linear & L2-MLR & $\mathcal{L}_{L2-MLR}(
\lambda, \mathbf{W}) = \sum_{j=1}^n \text{NLL}_{MLR}(\mathbf{W};
\mathbf{x}_i, \mathbf{y}^j) + 
\lambda \sum_{c=1}^C \| \mathbf{w}_c \|_2^2 $  & Max. Ent. & $L_2$ \\ \cline{2-3} 
						  & Nonlinear & L1-MLR & $\mathcal{L}_{L2-MKLR}(
\lambda, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + 
\lambda \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c $ & Max. Ent. & $L_1$ \\ \hline

\multirow{4}{*}{SVC Classification} & \multirow{2}{*}{Linear}  & BLSVC-RHL & $\mathcal{L}_{BLSVC-RHL}(T, \mathbf{w}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle) + \frac{1}{2} \| \mathbf{w} \|_2^2 $  & RHL & $L_2$ \\ \cline{3-6} 
                  &                    & BLSVC-SHL & $\mathcal{L}_{BLSVC-SHL}(T, \mathbf{w}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle)^2 + \frac{1}{2} \| \mathbf{w} \|_2^2 $ & SHL & $L_2$ \\ \cline{2-6} 
                  & \multirow{2}{*}{Nonlinear}  & BKSVC-RHL & $\mathcal{L}_{BKSVC-RHL}(T, \bm{\alpha}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle ) + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & RHL & $L_2$ \\ \cline{3-6} 
                  &                    & BKSVC-SHL & $\mathcal{L}_{BKSVC-SHL}(T, \bm{\alpha}) = T \sum_{j=1}^n \max(0, 1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle )^2 + \frac{1}{2} \bm{\alpha}^T \mathbf{K} \bm{\alpha} $ & SHL & $L_2$ \\ \hline

\hline
  Category                &       \multicolumn{2}{c|}{ML Model}            & Stealed Hyperparameter & Optimization Algorithm & Solution Type \\ \hline
            
\multirow{4}{*}{Regression} & \multirow{3}{*}{Linear} & RR & $\hat{\lambda}^{(i)}_{RR} = \frac{-\langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle}{w_i}$ & SVD~\cite{weisstein2002singular} & I \\ \cline{3-6}

                  &                   &  LASSO & $\hat{\lambda}^{(i)}_{LASSO} =  \begin{cases}
2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i - 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if }  w_i < 0 \\
-2 \langle \mathbf{x}_i, \mathbf{x}_i \rangle w_i + 2 \left\langle \mathbf{x}_i, \mathbf{r}_i \right\rangle & \text{if } w_i > 0 
\end{cases} $ & CD~\cite{friedman2010regularization} & II \\ \cline{3-6} 
                  &                   & ENet & $\hat{\bm{\lambda}}_{ENet} = \left( \mathbf{A}^T \mathbf{A} \right)^{-1} \mathbf{A}^T \mathbf{b} $ & CD & II \\ \cline{2-6} 
                  &     Nonlinear       & KRR       & $\hat{\lambda}^{(j)}_{KRR} = \frac{y_j - \mathbf{k}^{j} \alpha_j}{\alpha_j} $ & SVD & I \\ \hline

\multirow{4}{*}{BLR Classification} & \multirow{2}{*}{Linear}  & L2-BLR & $\hat{
\lambda}^{(i)}_{L2-BLR} = - \frac{\langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle}{2 w_i} $  & \multirow{4}*{LBFGS~\cite{liu1989limited}}  & \multirow{4}*{II} \\ \cline{3-4}

                  &                    & L1-BLR & $\hat{
\lambda}^{(i)}_{L1-BLR} = \begin{cases}
- \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i > 0 \\
 \langle \mathbf{x}_i, h_\mathbf{w}(\mathbf{X}) - \mathbf{y} \rangle & \text{if } w_i < 0 \end{cases} $  & & \\ \cline{2-4} 
                  
                  & \multirow{2}{*}{Nonlinear}  & L2-BKLR & $\hat{
\lambda}^{(j)}_{L2-BKLR} = - \frac{h_{\bm{\alpha}}(\mathbf{k}_j) - y_j} {2 \alpha_j}$ &  & \\ \cline{3-4} 
                  
                  &                    &  L1-BKLR & $\hat{
\lambda}^{(j)}_{L1-BKLR} = \begin{cases} y_j - h_{\bm{\alpha}}(\mathbf{k}_j)  & \text{if } \mathbf{k}^j \bm{\alpha} > 0 \\ h_{\bm{\alpha}}(\mathbf{k}_j) - y_j  & \text{if } \mathbf{k}^j \bm{\alpha} < 0 \end{cases} $ &  & \\ \hline

\multirow{2}{*}{MLR Classification} & Linear & L2-MLR & $\hat{
\lambda}^{(i,c)}_{L2-MLR} = - \frac{\langle \mathbf{x}_i, \bm{\mu}_{c,\mathbf{W}}(\mathbf{X}) - \mathbf{y}_c \rangle }{2 w_{i,c}} $ & \multirow{2}{*}{Newton-CG~\cite{wright1999numerical}} & \multirow{2}{*}{II} \\ \cline{2-4} 
						  & Nonlinear & L1-MLR & $\mathcal{L}_{L2-MKLR}(
\lambda, \bm{\Omega}) = \text{NLL}_{MKLR}(\bm{\Omega}; \mathbf{K}, \mathbf{Y}) + 
\lambda \sum_{c=1}^C \bm{\alpha}_c^T \mathbf{K} \bm{\alpha}_c $ & & \\ \hline

\multirow{4}{*}{SVC Classification} & \multirow{2}{*}{Linear}  & BLSVC-RHL & $\hat{T}^{(i)}_{BLSVC-RHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle < 1} y_j {x}_{j,i}}$ & SMO~\cite{platt1998sequential} & \multirow{4}*{III} \\ \cline{3-5} 
                  &                    & BLSVC-SHL & $\hat{T}^{(i)}_{BLSVC-SHL} = \frac{w_i}{\sum\limits_{j,y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle \leq 1} 2y_j {x}_{j,i} (1 - y_j \langle \mathbf{w}, 
\mathbf{x}_i \rangle) }$ & SGD~\cite{bottou2010large} & \\ \cline{2-5} 
                  & \multirow{2}{*}{Nonlinear}  & BKSVC-RHL & $\hat{T}^{(i)}_{BKSVC-RHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j, y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle <1} y_j k_{j,i}}$ & SMO & \\ \cline{3-5} 
                  &                    & BKSVC-SHL & $\hat{T}^{(i)}_{BKSVC-SHL} = \frac{\mathbf{k}^i \bm{\alpha}}{\sum\limits_{j,y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle \leq 1} 2y_j {k}_{j,i} (1 - y_j \langle \bm{\alpha}, \mathbf{k}_j \rangle)}$ & SGD & \\ \hline

\end{tabular} \\
\small
%Note: Obj. Func. is short for ``Objective Function". Similarly, Loss Func., Regu., Regression, Classification, Linear, Nonlinear, Est. Hyper., Opt. Alg., and Sol. Type are short for ``Loss Function", ``Regularization", ``Regression", ``Classification", ``Linear", ``Nonlinear", ``Estimated Hyperparameter", ``Optimization Algorithm", and ``Solution Type"; 
Note: SVD is Singular Value Decomposition; CD is Coordinate Descent; CG is Conjugate Gradient; SMO is Sequential Minimal Optimization; SGD is Stochastic Gradient Descent.
\end{sidewaystable*}



